Training-Free Restoration of Pruned Neural Networks

Although network pruning has been highly popularized to compress deep neural networks, its resulting accuracy heavily depends on a fine-tuning process that is often computationally expensive and requires the original data. However, this may not be the case in real-world scenarios, and hence a few recent works attempt to restore pruned networks without any expensive retraining process. Their strong assumption is that every neuron being pruned can be replaced with another one quite similar to it, but unfortunately this does not hold in many neural networks, where the similarity between neurons is extremely low in some layers. In this article, we propose a more rigorous and robust method of restoring pruned networks in a fine-tuning free and data-free manner, called LBYL (Leave Before You Leave). LBYL significantly relaxes the aforementioned assumption in a way that each pruned neuron leaves its pieces of information to as many preserved neurons as possible and thereby multiple neurons together obtain a more robust approximation to the original output of the neuron who just left. Our method is based on a theoretical analysis on how to formulate the reconstruction error between the original network and its approximation, which nicely leads to a closed form solution for our derived loss function. Through the extensive experiments, LBYL is confirmed to be indeed more effective to approximate the original network and consequently able to achieve higher accuracy for restored networks, compared to the recent approaches exploiting the similarity between two neurons. The very first version of this work, which contains major technical and theoretical components, was submitted to NeurIPS 2021 and ICML 2022.

==> backup/ICML22_bak/abstract.tex <==
\begin{abstract}
Although network pruning has been highly popularized to compress deep neural networks, its resulting accuracy heavily depends on a fine-tuning process that is often computationally expensive and requires the original data. However, this may not be the case in real-world scenarios, and hence a few recent works attempt to restore pruned networks without any expensive retraining process. Their strong assumption is that every neuron being pruned can be replaced with another one quite similar to it, but unfortunately this does not hold in many neural networks, where the similarity between neurons is extremely low in some layers. In this paper, we propose a more rigorous and robust method of restoring pruned networks in a fine-tuning free and data-free manner, called \textit{LBYL} (\textit{Leave Before You Leave}). LBYL significantly relaxes the aforementioned assumption in a way that each pruned neuron \textit{leaves} its pieces of information to as many preserved neurons as possible and thereby multiple neurons together obtain a more robust approximation to the original output of the neuron who just \textit{left}. Our method is based on a theoretical analysis on how to formulate the reconstruction error between the original network and its approximation, which nicely leads to a closed form solution for our derived loss function. Through the extensive experiments, LBYL is confirmed to be indeed more effective to approximate the original network and consequently able to achieve higher accuracy for restored networks, compared to the recent approaches exploiting the similarity between two neurons.
\end{abstract}



==> backup/ICML22_bak/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
This paper proposed the problem of restoring a pruned CNN in a way free of training data and fine-tuning. We mathematically formulated how filter pruning can make a damage to the output of the pruned network, and focused on how to model the information carried by each pruned filter to be delivered to the other remaining filters. Our proposed assumption is inspired by the fact that the more the remaining filters participate in the recovery process, the better the approximation we can obtain for the original output. With this assumption, we successfully decomposed the reconstruction error into the three different components, and thereby designed a data-free loss function along with its closed form solution. Our future work would be to extend the proposed loss function so as to cover different activation functions other than ReLU.

==> backup/ICML22_bak/experiments.tex <==
\section{Experiments} \label{sec:experiments}
In this section, we empirically validate the performance and effectiveness of our proposed LBYL method, compared to a one-to-one compensation method, called \textit{Neuron Merging} (\textit{NM})  \cite{NM} as well as a baseline called \textit{Prune} that does not perform any recovery process after pruning. For a fair comparison, we exploit the code provided by the authors of \cite{NM} and then implement our proposed method using PyTorch \cite{PyTorch}. LBYL uses two hyperparameters, namely $\lambda_1$ and $\lambda_2$, that adjust the weights of loss terms BE and AE, respectively. The details of hyperparameter settings are presented in Appendix. Also, our implementation is available at our anonymized github.\footnote{https://github.com/anonymous}

\smalltitle{Pruning criteria and ratio}
We evaluate LBYL using the following four data-independent pruning criteria: L1-norm \cite{PFEC}, L2-norm \cite{Soft}, L2-GM \cite{FPGM}, and lastly even random. We prune only convolution filters in CNNs, and hence the pruning ratio is the ratio of pruned filters for each convolution layer.
% Random pruning is intended to show the robustness of each method when a norm-based criterion is not used.

\subsection{Experiments using CIFAR-10 and CIFAR-100}
\smalltitle{Dataset and pretrained model} 
The CIFAR-10 dataset \cite{krizhevsky2009learning} consists 60K images of 10 different classes, where each class includes 5K training images along with 1K validation images and the size of every image is 32 × 32. CIFAR-100 \cite{krizhevsky2009learning} also include 60K images for 100 different classes, where 500 training images along with 100 validation images are included for each class. We test VGG-16 \cite{VGG} for CIFAR-10 and ResNet-50 \cite{ResNet} for CIFAR-100, and present the result of CIFAR-100 only in Appendix as 
their experimental results of CIFAR-10 and CIFAR-100 show the similar trend.


% In case of CIFAR-100, we evaluate the our proposed method using the ResNet-50 \cite{ResNet}. To train the ResNet-50, we exploit SGD with Nesterov momentum of 0.9. the initial learning rate is 0.1 and it is divided by 5 at 60, 120, 160 epochs. the weight decay is set to 5e-4, the train epochs is 200 with batch size 128. 

\smalltitle{Results}
We first prune VGG-16 on CIFAR-10, which is a representative single-branched CNN, using the layer-by-layer pruning scheme with four different criteria, and then update the remaining filters in each layer to restore the pruned VGG-16. As shown in Table \ref{tab:VGG16-CIFAR10}, our LBYL method achieves up to 6.16\% higher average accuracy than NM \cite{NM}. In particular, LBYL outperforms NM with clear margins when the pruning ratio increases. This is probably because NM might have trouble finding a filter sufficiently close to each pruned filter with less remaining filters due to a higher pruning ratio.

\subsection{Experiments using ImageNet (ILSVRC2012)}

\smalltitle{Dataset and pre-trained model} 
The ImageNet dataset \cite{deng2009imagenet} contains 1,000 classes and consist of 1.28M training images and 50K validation images of size 256 $\times$ 256. For ImageNet, we use pretrained ResNet-34 and ResNet-101, both of which are released by PyTorch\footnote{https://pytorch.org/vision/stable/models.html}. ResNet-34 and ResNet-101 respectively represent two different types of the ResNet architecture, namely the one consisting of basic blocks and the other one consisting of bottleneck blocks.

\smalltitle{Results}
To prune a ResNet architecture, we exploit the common strategy to remove each residual block, that is, pruning the first two convolutional layers and not changing the output dimension of the block. Tables \ref{tab:ResNet34-ImageNet} and \ref{tab:ResNet101-ImageNet} present the experimental results using ResNet-34 and ResNet-101 on ImageNet. Through the results, LBYL can still recover the damaged filters to a satisfactory extent.

\begin{figure}[t]
	\centering 
	% vanilla WA
	\includegraphics[height=2mm]{./figure/error_key.pdf} \\
    \subfigure[\label{fig:expcos_:a}{RE} ]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/LBYL_figure_3_RE.pdf}\hspace{0mm}}
    %CTL + WA
    \subfigure[\label{fig:expcos_:b}{BE} ]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/LBYL_figure_3_BE.pdf}\hspace{0mm}}
    % ART+WA
    \subfigure[\label{fig:expcos_:c}{WARE} ]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/LBYL_figure_3_WARE.pdf}\hspace{0mm}}
    \caption{Comparison on the three error components with NM \cite{NM}, where each $m$\_$n\_k$ in the x-axis represents the $k$-th conv module in the $n$-th block at the $m$-th layer in ResNet-50}
	\label{fig:error_components}
	\vspace{-2mm}
\end{figure}


\subsection{Effectiveness in terms of Reconstruction}
In order to see the effectiveness of our loss function on minimizing the reconstruction error, we compute the values of three error components, namely RE, BE, and AE, using ResNet-50 \cite{ResNet} on CIFAR-100 \cite{krizhevsky2009learning}. Both RE and BE can be measured without any inference with sample data, but AE is not easy to obtain. Therefore, we adopt the \textit{weighted average reconstruction error} (\textit{WARE}) introduced in \cite{NISP}, which shows the difference between the layer-wise output of the original model and that of the pruned model.

Figure \ref{fig:error_components} shows layer-wise values for each of RE, BE and WARE. It is clearly observed that NM returns a very rough approximation in terms of RE, compared to our LBYL method. This is due to the fact that NM uses only a single remaining filter to receive the missing information of a pruned filter, and consequently the final output can be quite far from the original.
In both BE and WARE, there is not much difference between LBYL and NM in early layers, but we can observe that the error values of NM become higher in the end. Thus, even though NM might be effective to reconstruct the original output in some layers, it shows unstable performance depending on the existence of similar filters and finally ends up with less accurate approximation. On the other hand, our LBYL method is less varied across layers and managed to keep the error values lower in the end for all three metrics.

\begin{table}[t]
\centering
\tiny
\begin{tabular}{c||c|c|c|c|c} \Xhline{2\arrayrulewidth}
Pruning Ratio& Ours & NM& Coreset&Prune & From Scratch (80 epochs) \\ \Xhline{2\arrayrulewidth}
10 \% & \textbf{78.3}   & 77.57  &76.55 & 77.67  & 48.22 (72.07)\\\hline
20 \% & \textbf{77.22}  &  75.62  &74.39&  75.4   & 47.85 (72.01)\\\hline 
30 \% & \textbf{75.99}  & 73.03  &71.88&  73.18  & 46.7 (72.24)\\\hline
40 \% & \textbf{74.13}  & 69.71  &68.14&  70.12  & 46.53 (72.88)\\\hline
50 \% & \textbf{71.15}  & 65.03  &62.88&  65.72  & 44 (69.33)\\\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Fine-tuned or trained accuracies of ResNet-50 on CIFAR-100 using L2-norm criterion, where we fine-tune each model for 20 epochs and train the same-sized small architecture for 20 epochs (80 epochs)}
\label{tab:finetune_scratch}
\vspace{-3mm}
\end{table}

\begin{figure}[t]
	\centering 
	\includegraphics[height=2mm]{./figure/f4_KEY.pdf} \\
    \subfigure[\label{fig:expcos:a}{10 \%} ]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/f4_10.pdf}\hspace{0mm}}
    \subfigure[\label{fig:expcos:b}{30 \%} ]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/f4_30.pdf}\hspace{0mm}}
    \subfigure[\label{fig:expcos:c}{50 \%} ��]{\hspace{0mm}\includegraphics[width=0.32\columnwidth]{./figure/f4_50.pdf}\hspace{0mm}}
    \caption{Comparison on learning curves of fine-tuning restored networks for 20 epochs and that of training the same-sized small architecture from scratch for 80 epochs at different pruning ratios}
	\label{fig:Fine tuning and From Scratch}
 	\vspace{-2mm}
\end{figure}

\smalltitle{Performance estimation}
��) can also be utilized in such a case. As shown in Figure \ref{fig:error_components}, we can roughly estimate WARE, which is also highly relevant to the final performance, by combining RE and BE.

\subsection{Practical Test with Data and Fine-Tuning}
Although this paper focuses on the problem of restoring pruned networks without data, we additionally test whether our method is also effective when the data becomes available later on. Table \ref{tab:finetune_scratch} shows the experimental results on the final accuracy of each pruned or restored model after fine-tuning along with that of the same-sized architecture trained from scratch. In this experiment, we take the data-independent pruning method based on coreset \cite{CoreSet_ICLR} as another competitor, which also introduces a training-free recovery method as an intermediate process. We fine-tune and train each model for 20 epochs, and also show the resulting accuracy of the model trained from scratch after 80 epochs. In all cases, our LBYL method outperforms its competitors particularly when the pruning ratio increases. Our best guess on why NM becomes eventually worse than just pruned model is that NM can choose a dissimilar filter to recover each pruned one in some layers, which makes it hard for fine-tuning to improve the performance.
\textit{Coreset} \cite{CoreSet_ICLR} shows the lowest accuracy probably because it does not focus on training-free recovery and hence 20 epochs of fine-tuning is not sufficient. As shown in Figure \ref{fig:Fine tuning and From Scratch}, LBYL shows the fastest convergence speed during the fine-tuning process. Both of these observations justify the fact that our LBYL method is practically useful when the data is available. 

% \TODO{Add Coreset method in Table 4 and Figure 4. Change Table 4 to have arrows}
% We also compare the Coreset\cite{CoreSet_ICLR} from the standpoint that update the weights of pruned model as shown in the Figure 4. \ref{fig:Fine tuning and From Scratch},where we present average accuracy of the Coreset \cite{CoreSet_ICLR}. The reason why Coreset \cite{CoreSet_ICLR} shows the lowest accuracy is that Coreset \cite{CoreSet_ICLR} do not focus on directly minimizing the output between pruned model and pre-trained model but concentrate on proving the error bound for output between pruned model and pre-trained model, which results in insignificant compensation.


% We measure the reconstruction errors (RE) generated by pruned filter and preserved filter and batch normalization error, which can minimize the reconstruction error, where both RE and BE are taken l2-norm to show magnitude. LBLY optimize the scale parameter to minimize the both RE and BE. Therefore, Our method has a lower error compared to NM \cite{NM} as shown in Figure \ref{fig:error_components}.Moreover we also calculate the Weighted Average Reconstruction Error (WARE) used in \cite{NISP} to measure the difference between original model and recovered model. From Figure \ref{fig:error_components}, LBLY tends to increase more gently in last layer because our method is based on the number of filters,leads to small reconstruction error than NM with considering relationship between pruned filter and only one remained filter.\cite{NM} 




% \begin{figure*}[t]
% 	\centering
% 	{
%     \includegraphics[height=2.5mm]{./figure/key.pdf}	\vspace{1mm}

% 		\begin{tabular}{cccc}
% 			\subfigure[\label{fig:cifar:a}2 tasks] {\includegraphics[height=32mm]{./figure/LBYL_figure_2}}  & 
% 		\end{tabular}
% 		\vspace{-3mm}
% 		\caption{Comparison on the accuracy for each incremental task using CIFAR-100}
% 		\label{fig:cifar}
% 	}

% \end{figure*}



% \begin{table}[]
% {\scriptsize

% \begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
% \multicolumn{13}{c}{\textbf{ResNet-50 (Acc. 73.27) }}
% \\ \Xhline{2\arrayrulewidth} %\hline
% Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
% Pruning Ratio& Ours& NM& prune& Ours& NM& prune& Ours& NM& prune& Ours& NM& prune
% \\ \Xhline{2\arrayrulewidth}
% 10\%& \textbf{77.31}& 77.28& 75.14& \textbf{77.20}& 76.92& 74.49& \textbf{77.55}& 77.21& 75.07& \textbf{76.14}& 72.18& 58.12\\ \hline
% 20\%& \textbf{73.24}& 72.73& 63.39& \textbf{73.46}& 72.32& 63.54& \textbf{73.20}& 72.24& 61.84& \textbf{70.59}& 59.62& 26.87\\ \hline
% 30\%& \textbf{66.63}& 64.47& 39.96& \textbf{67.07}& 64.01& 39.01& \textbf{66.30}& 63.07& 35.77& \textbf{62.22}& 39.45& 2.59 \\ \hline
% 40\%& \textbf{51.46}& 46.40& 15.32& \textbf{50.60}& 46.17& 13.14& \textbf{48.07}& 45.98& 12.59& \textbf{41.90}& 17.77& 3.08 \\ \hline
% 50\%& \textbf{28.74}& 25.98& 5.22& \textbf{30.66}& 23.44& 4.32& \textbf{22.06}& 21.98& 4.25& \textbf{22.07}& 7.17 & 2.20 \\ \Xhline{2\arrayrulewidth}
% Average Acc.& \textbf{59.48}& 57.37& 39.81& \textbf{59.80}& 56.57& 38.90& \textbf{57.44}& 56.10& 37.90& \textbf{54.58}& 39.24& 18.57 \\ 
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% \caption{Compenssation results of ResNet-50 on CIFAR-100}
% \label{tab:ResNet50-CIFAR100}

% \end{table}

==> backup/ICML22_bak/intro.tex <==
\section{Introduction} \label{sec:intro}


% 1. Network pruning has been extensively studied in neural networks. 
%    its simplicity, reasonable performance
Network pruning is one of the most well-studied model compression technique for an overparameterized deep neural network, and many different pruning strategies have been introduced with the goal of removing less important parameters from the original network. Due to its simplicity in terms of both implementation and methodology, network pruning has been pretty popular to the point that it is provided as a default model compression function in standard libraries like TensorFlow\footnote{https://www.tensorflow.org/model\_optimization/guide/pruning} and PyTorch\footnote{https://pytorch.org/tutorials/intermediate/pruning\_tutorial.html}, along with the other compression options such as quantization \cite{Coreset}. Among two major pruning schemes, namely weight pruning (\textit{a.k.a.} unstructured pruning) \cite{Lottery,Songhan,SNIP,Synaptic,OptimalPruning} and filter pruning (\textit{a.k.a.} structured pruning), filter pruning is more actively studied \cite{FPGM,Lasso,EagleEye,Rethinking,Thinet,DCP} due to its strength of reducing the actual computation cost at inference time without any special hardware support. In this sense, this paper also focuses on filter pruning.

% \cite{GlobalRanking,AMC,FPGM,Lasso,EagleEye,Dynamic,Rethinking,CURL,Thinet,Importance,Reborn,NISP,DCP}

% To deploy large neural networks to resource-constrained mobile and edge devices, network pruning has been extensively studied due to implementation-friendly and compatibility with other network compression methods \cite{DBLP:conf/eccv/HeLLWLH18, DBLP:conf/cvpr/HeLWHY19} In general, Network pruning methods is fall in to two parts : Weight pruning(Unstructured pruning) and Filter pruning(Structured pruning). Weight pruning encourage parameters of neural network sparse during the training process or post process. As a result, Number of parameters in neural networks can be reduced parameters more than 90\% \cite{NIPS2015_ae0eb3ee} However, Because of irregular sparse connections Weight pruning need a special software to accelerate inference speed. On the other hand, Filter pruning removes unimportant filter so can accelerate inference time without special software. 

% 2. Most of pruning methods require an expensive training process
%    e.g., iterative training(on the fly), fine-tuning(post process)
% 3. A long fine-tuning eventually determines the final accuracy 
%    That is why existing pruning methods use only a few 2-3 epochs of fine-tuning

Even though many of the existing pruning methods achieve a reasonable level of the final accuracy, it mostly comes at an expensive cost of retraining at the end of (or in the middle of) pruning phase. For instance, iterative filter pruning methods \cite{Soft,FPGM,Dynamic} alternately perform pruning phase and retraining phase so that the original model can gradually be compressed as well as recovered over the hundreds of epochs. Another major approach is to conduct \textit{one-shot pruning} and then fine-tune the pruned network for its original performance to be recovered \cite{EagleEye,CURL,Importance,NISP,DCP}. In most one-shot pruning techniques, the fine-tuning phase does not take longer than a few dozens of epochs probably because there is no big difference in accuracy among pruning criteria beyond that point. In fact, it is reported that even a randomly pruned network can reach comparable performance after fine-tuning of hundreds or thousands of epochs \cite{Rethinking}. Thus, if we do not have any constraints on time, computing resources, or training data for a long fine-tuning process, one-shot pruning methods would be less meaningful.

% 4. Therefore, they obviously need a quiet complete set of training data
%    (mostly exactly the same as the original train set) or need to collect as 
%    many samples as the origin
% 5. However, in practice, the train data is neither available nor easy to collect
% 6. Therefore, a few recent works have tried to address above with using much small data ( still need data, train process anyway)
% 7. Meanwhile, a few works commonly employ the neuron similarity in order to 
%    reduce the bad effect of pruning Thus, a similar neuron can be replaced
%    limitations of NM, 
%    1) it is based on strong naive assumption, which is not the case in NNs.
%    2) a single neuron can't compensate due to the error term we found yet not discussed

\begin{figure*}[t!]
   \centering 
    \includegraphics[width=1.9\columnwidth]{./figure/LBYL_figures.pdf}
   \caption{The conceptual overview of our LBYL method, showing how the original output resulting from a pruned filter at $\ell$-th layer, that is, the output of $(\ell+1)$-th convolutional layer, can be recovered by all the other preserved filters at the same layer (\textit{i.e.}, $\ell$-th layer) through convolution, batch normalization, and activation function (\textit{i.e.}, ReLU), where $s, s',$ and $s^*$ are the coefficients that quantify how much each preserved filter should carry the information of the pruned filter.}
   \label{fig:framework}
\end{figure*}


Somewhat fortunately, however, this is not the case in many practical scenarios where we cannot access or re-collect the original data due to its large volume or some commercial issues \cite{DBLP:conf/eccv/MahajanGRHPLBM18}. Even though some recent works \cite{CURL,Reborn} attempt to use only a small amount of training data instead, but they still suffer from a time-consuming process of fine-tuning to achieve satisfactory performance. Furthermore, it would not be always possible to collect samples in the same domain as the original data, regardless of whether they are labeled or not. Only quite a few works \cite{NM,Data-free} have been introduced to recover pruned networks without using any data and fine-tuning process. Their common approach is what we call \textit{one-to-one compensation}, where the most similar unpruned neuron takes the role of a pruned neuron. This approach is based on the strong assumption that there exists such a neuron quite similar to each one being pruned at the same layer. Not surprisingly, this assumption cannot be guaranteed in deep neural networks, which is even reported in the result of \cite{NM} showing that the pairwise similarity on filters gets extremely low particularly in deeper layers. In addition, according to our theoretical analysis on the reconstruction error, a single neuron can only lead to a very rough approximation to the original output even if the neuron is similar enough to its pruned counterpart.



% However, they obviously still require a quiet complete set of train data to recover a original network performance because as presented in \cite{DBLP:conf/aaai/TangYXH0SXZ20}, compressed network hard to reach original performance with a few data. Moreover, in many practice application, the train data is neither accessible nor easy to collect due to commercial profits \cite{DBLP:conf/eccv/MahajanGRHPLBM18}. There are two trials to fine-tune the pruned model with small data using knowledge distilation \cite{Knowledge_Distilation} and extra trainable parameters. \cite{CURL} propose fine-tuning method based on knowledge distillation using a few data. More specifically, they employ soft target of the pre-trained model regarding the small data to fine-tuning the pruned model. \cite{Reborn} appends the additional convolution modules due to hardness to fine-tune using the small data and then retrain the extra modules with existing modules fixed. after fine-tuning on the supplementary modules with sparsity, the compressed model combines with additional convolution module and original modules to recover the original performance. However, they obviously exploit the small data to restore performance of original network.


% A few works \cite{NM, Data-free} commonly employ the neuron similarity in order to reduce catastrophic loss induced by removed filters without using any data and any fine-tuning process. They have a strong assumption that a filter can be replaced with a most similar filter but these assumption in neural networks have the limitations. It depends on that pruned filters have a single similar filter in neural networks. As presented in \cite{NM}, if the layer in networks become more deeper, the correlation between the filters in layer gradually decrease. Thus, preserved filter which is a most similar with removed filter isn't actually similar with pruned filter. That is, it turn out that a single similar filter can't significantly compensate. Moreover, they have ignored the error term we found yet not discussed in \cite{NM}.



% As shown above the pruned model, if filters in layer be pruned, the corresponding channels of filter in $i$+1-th layer are removed, which leads to loss of the feature maps in $i$+1-th layer. However, LBYL restores catastrophic loss pruned from filters in $i$-th layer by compensating the channels of filter $i$+1-th with a our assumption that compensation of pruned filter in $i$-th layer can be made with relationship between the pruned filter and preserved filters in $i$-th layer. The overall recovery process is as follow: first, we use a assumption that pruned filter in i-th layer is represented by multiple preserved filters on the same layer. Secondly, we can obtain the approximation scale to compensate pruned filter by extending the our assumption to normalization, activation layer, and convolution outputs (\textit{e.g.} feature maps in i+1 layer). Thirdly, before removing the channels of filters in $i$+1-th resulted from the pruned filter in $i$-th layer, they would be multipled by approximation scale and then add their weights to preserved filter in i+1 layer as shown in the last part above. Finally, we significantly recover the information loss induced by pruned filters in $i$-th layer


In this paper, we propose a theoretically more rigorous and robust method, called \textit{Leave Before You Leave} (\textit{LBYL}), to effectively compensate for pruned filters, which is also free of any data and fine-tuning. As depicted in Figure \ref{fig:framework}, we significantly relax the strong assumption by observing the fact that a pruned filter is better to be represented by a linear combination of as many preserved filters as possible than it is done by a single filter. We first mathematically analyze how the reconstruction error can be formulated between the original network and its pruned network, and thereby discover three components of the error. Based on our formulation, we provide a closed form solution that can minimize the reconstruction error to compensate for information loss caused by pruned filters, which does not need any training process at all. Through extensive experiments, we show that LBYL outperforms the existing one-to-one compensation scheme \cite{NM} regardless of pruning criterion. For instance, LBYL achieves at pruning ratio 30\% on the average 17.92\% higher accuracy than those of \cite{NM} for ResNet-101 \cite{ResNet} trained with ImageNet \cite{deng2009imagenet}.



% LBYL achieves at pruning ratio 40\% on average 3.53\% higher accuracy than \cite{NM} for ResNet-50 \cite{ResNet} on CIFAR-100 \cite{krizhevsky2009learning} and also in case of large dataset (i.e., ImageNet \cite{deng2009imagenet}), .



% using CIFAR \cite{krizhevsky2009learning} and ImageNet \cite{deng2009imagenet}








==> backup/ICML22_bak/method.tex <==
\section{Proposed Method of Restoring Pruned Filters} \label{sec:method}
In this section, we first theoretically examine how the reconstruction error of Eq. (\ref{eq:goal}) can be formulated in a way free of using data-dependent parameters. Based on this analysis, we present our train-free recovery method that has a closed form solution for minimizing the formulated reconstruction loss.

%is composed of with respect to our proposed methodology using multiple filters to approximate a pruned filter, so-called \textit{many-to-one}. Our approach is in fact a generalized version of the existing one-to-one compensation methods \cite{NM,Data-free}. Finally, we present our train-free recovery method that has a closed form solution for minimizing the formulated reconstruction error.

\subsection{Data-Independent Reconstruction Loss} \label{sec:method:a}
For brevity, we deal with a simple case of pruning only a single filter, which can trivially be extended to cover multiple filters. Without loss of generality, let the $j$-th filter of the $\ell$-th layer be pruned. 

\smalltitle{Leave Before You Leave (LBYL) assumption}
In order to transform Eq. (\ref{eq:goal}) to a data-free version, our proposed assumption is that each filter being pruned can \textit{leave} its pieces of information for the remaining ones by adding its corresponding pruned channel to each of the other channels in the next layer. Since the quantity of information depends on how much the pruned filter is related to a particular remaining filter, we need to multiply the pruned channel with a different value before addition. Based on this assumption, for a case of pruning only the $j$-th filter, the delivery matrix $\boldsymbol{\S^*} \in \mathbb{R}^{m \times (m-1)}$ is defined to be in the following form:
\begin{eqnarray}\begin{split}\label{eq:matrix}
\boldsymbol{\S^*}_{i,k} = 
  \begin{cases} 
   1 & \text{if } i = i'_k \\
   s_{i'_k} & \text{if } i = j \\
   0 & \text{otherwise}
  \end{cases}
  \end{split}
\end{eqnarray}
 $\text{s.t. } i, i'_k \in [1, m] \text{ and } k \in [1, m-1],$ where $s_{i'_k}$ is a scalar value that quantifies to what extent the $i'_k$-th filter is related to the $j$-th filter being pruned. Figure \ref{fig:matrix:b} shows an example of the delivery matrix for our LBYL method.


\smalltitle{Without BN and an activation function}
Starting with Eq. (\ref{eq:goal}), we first derive its data-free version without considering both a BN procedure and an activation function, and then make an extension for them. With the proposed form of the delivery matrix in Eq. (\ref{eq:matrix}) together with Eq. (\ref{eq:fmap_approx}), the $i$-th channel of $\mathbf{\hat{Z}}^{{(\ell+1)}}$ is now represented as:
\begin{equation}
{{\mathbf{\hat{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast (\mathbf{W}_{i,k}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j}^{(\ell+1)}).
\nonumber
\end{equation}
Then, the reconstruction error for the $i$-th channel of the feature map at the $(\ell+1)$-th layer can be derived as:
\begin{equation}
{\mathbf{Z}_{i}^{{(\ell+1)}}}-{\mathbf{\hat{Z}}_{i}^{{(\ell+1)}}}=(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\circledast \mathbf{W}_{i,j}^{(\ell+1)}.
\label{eq:eq5}
\end{equation}
By Eq. (\ref{eq:eq5}), we have the following form of the reconstruction error for the case of pruning the $j$-th filter at the $\ell$-th layer:
\begin{eqnarray}\begin{split}
\sum\limits_{{i} = 1}^{m^{\prime}}\|{\mathbf{Z}_{i}^{{(\ell+1)}}-\mathbf{\hat{Z}}_{i}^{{(\ell+1)}}}\|_1 ~~~~~~~~~~~~~~~~~\\ 
=\sum\limits_{{i} =  1}^{m^{\prime}}\|(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\circledast\mathbf{W}_{i,j}^{(\ell+1)}\|_1.
\end{split}
\label{eq:eq6}
\end{eqnarray}
Based on Eq. (\ref{eq:eq6}), we can reduce the problem of minimizing Eq. (\ref{eq:goal}) into the one of minimizing the following error term:
\begin{equation} \label{eq:goal2}
\|(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\|_1,
\end{equation}
where we need to find scalars $s_{k}$'s such that ${ \mathbf{A}_{j}^{(\ell)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}}$.

Without considering BN and any activation function, we simply have $\mathbf{A}^{(\ell)} = \mathbf{Z}^{(\ell)}$, and consequently Eq. (\ref{eq:goal2}) can be represented as:
\begin{gather*}
    %  \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} \\
    % = \| (\mathbf{A}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(\ell)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times (\mathbf{A}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(\ell)} ) \|_{1} \nonumber \\
    % = 
     \| (\mathbf{A}^{(\ell-1)}  \circledast (\mathbf{W}_{j}^{(\ell)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(\ell)} ) \|_{1}.
\end{gather*}
Since $\mathbf{A}^{(\ell-1)}$ is data-dependent yet independent to pruned filters, it can be regarded as a constant factor of the reconstruction error that depends on which filters are pruned. Thus, it suffices to minimize the other part of the term, which we call \textit{Residual Error} (\textit{RE}) denoted by $\boldsymbol{\E}$ as the following definition:
\begin{definition} \label{def:re}
Given a pruned filter $\mathbf{W}_{j}^{(\ell)}$ at the $\ell$-th layer, the Residual Error (RE) is defined as:
$$
\boldsymbol{\E} = \mathbf{W}_{j}^{(\ell)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(\ell)}.
$$
\end{definition}
Note that $\boldsymbol{\E}$ can be minimized by using only the original network without any support from data.


% Since we cannot access $\mathbf{A}^{(\ell-1)}$ without data, the only thing we can do is minimizing the other part of the term. We call this error term \textit{Residual Error} (\textit{RE}) and denote it by $\boldsymbol{\E}$

\smalltitle{Considering batch normalization} 
We now incorporate a BN procedure in the process of minimizing Eq. (\ref{eq:goal2}). In this case, as we have $\mathbf{A}^{(\ell)} = \N(\mathbf{Z}^{(\ell)})$, Eq. (\ref{eq:goal2}) can be derived as Lemma \ref{lem:bn}.
\begin{lemma} \label{lem:bn}
If there is only batch normalization between a feature map and its activation map, the reconstruction error can be formulated as follows:
\begin{equation} \label{eq:bn}
\| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)} \circledast \boldsymbol{\E})} + \boldsymbol{\B}\|_{1},
\end{equation}
% \begin{equation} \label{eq:bn}
% \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)} \circledast \boldsymbol{\E})} +
% \frac{\gamma_{j}}{\sigma_{j}} 
% \{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j + \frac{\sigma_{j}}{\gamma_{j}}\beta_j\} \|_{1},
% \end{equation}
where $\boldsymbol{\B} = \frac{\gamma_{j}}{\sigma_{j}} 
 \{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j + \frac{\sigma_{j}}{\gamma_{j}}\beta_j\}$, $\mu$, $\gamma$, $\sigma$, and $\beta$ are batch normalization parameters.
\end{lemma}
\begin{proof}
See Appendix.
\end{proof}
Hereafter, the notation $\boldsymbol{\E}$ is a bit differently defined such that $s_k$ from Definition \ref{def:re} should be substituted with $s_k \frac{\sigma_j}{\gamma_j} \frac{\gamma_k}{\sigma_k}$ due to the BN procedure. We call the second term $\boldsymbol{\B}$ of Eq. (\ref{eq:bn}) Batch Normalization Error (BE).

\begin{definition}
Given a pruned filter $\mathbf{W}_{j}^{(\ell)}$ at the $\ell$-th layer, the Batch Normalization Error (BE) is defined as:
$$
\boldsymbol{\B} = \frac{\gamma_{j}}{\sigma_{j}} 
\{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j  + \frac{\sigma_{j}}{\gamma_{j}}\beta_j \}.
$$
\end{definition}



% below Eq. (\ref{eq:eq9}).
% \begin{eqnarray} \begin{split}\label{eq:eq9}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \N (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}
% Eq. (\ref{eq:eq9}) is further derived and finally we can conclude to the following lemma:


\smalltitle{Considering activation function}
Lastly, we proceed our analysis to cover a general CNN architecture including both BN and the ReLU activation function. For an activation function $\F$, we now have $\mathbf{A}^{(\ell)} = \F(\N(\mathbf{Z}^{(\ell)}))$, and thereby Eq. (\ref{eq:goal2}) is derived to be the following theorem:
\begin{theorem} \label{thm:relu}
If there are both batch normalization and a ReLU function between a feature map and its activation map, the reconstruction error can be formulated as follows:
    \begin{equation} \label{eq:relu}
     \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)}\circledast\boldsymbol{\E})}+ \boldsymbol{\B} + \boldsymbol{\R}\|_{1},
     \nonumber
     \end{equation}
     where $\boldsymbol{\R} = \sum\limits_{k=1, k \neq j}^{m} s_{k}  \min(0,\N(\mathbf{Z}_{k}^{(\ell)}))-\min(0,\N(\mathbf{Z}_{j}^{(\ell)}))$ represents the \textit{Activation Error} (\textit{AE}).
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

\smalltitle{Data-free loss function}
As concluded in Theorem \ref{thm:relu}, we discover the fact that the reconstruction error of Eq. (\ref{eq:goal}) can finally be decomposed into three different components, namely RE, BE, and AE. This brings us to formulate the following reconstruction loss that does not require any training data. 
\begin{equation}
     \mathcal{L}_{re} =  \|\boldsymbol{\E}\|_2^{2} + \lambda_1 \|\boldsymbol{\B}\|_2^{2} + \lambda_2 \|\mathbf{s}\|_{2}^{2},
\label{eq:loss}
\end{equation}
where $\mathbf{s} =  [s_{1}~...~s_{j-1}~s_{j+1}~...~s_{m}]$.

Unlike RE and BE, we cannot exactly control the AE term as $\mathbf{Z}^{(\ell)}$ can only be obtained by using the actual data. Therefore, we instead introduce a regularization term $\|\mathbf{s}\|_{2}^{2}$ for the purpose of mitigating the explosion of $\boldsymbol{\R}$, inspired by the fact that each error value of $\boldsymbol{\R}$ is proportional to $s_k$. Furthermore, since our intention is to participate as many preserved filters as possible in restoring a pruned filter, it would be better for the $s_k$ values to be more uniformly distributed. Both purposes can be fulfilled by this L2-based regularization term. 

\begin{algorithm}[t]
  \scriptsize
  \caption{LBYL method}
  \label{alg:Recovery}
  \KwIn{$\mathbf{\Theta}$ = $[\mathbf{W}^{{(1)}}$, .... ,$\mathbf{W}^{{(L)}}] := $ Original model}
  \KwOut{$\hat{\mathbf{\Theta}}$ = $[{\mathbf{\hat{W}}}^{{(1)}}$, .... ,$\mathbf{\hat{W}}^{(L)}] : = $ Pruned \& restored model}
   
  \For{each layer $\ell \in [1, L]$ that has been pruned}%$\in$ $\mathbb{R}^{n_{l} \times k \times k}$   $\mathbf{in}$ $\mathbf{W}^{(\ell)}$}
    {
    ${\boldsymbol{\S}}^{(\ell)} \leftarrow $ a zero-valued matrix
    
    \For{each filter $\mathbf{W}_i^{(\ell)}$ s.t. $i$ $\in$ $[1,m]$}{
        \If{$\mathbf{W}_i^{(\ell)}$ is not pruned} 
            {
            $\boldsymbol{\S}_{i,k}^{(\ell)} = 
              \begin{cases} 
              1  & \text{if  } i = i'_k \\
              0  & \text{otherwise } \\
              \end{cases}
             $
            }
        \Else{        
        $\boldsymbol{\S}_{i,:}^{(\ell)} \leftarrow {\argmin\limits_{\mathbf{s}}~\|\boldsymbol{\E}\|_2^{2} + \lambda_1 \|\boldsymbol{\B}\|_2^{2} + \lambda_2 \|\mathbf{s}\|_{2}^{2}}$  \tcp{obtained by Theorem \ref{thm:closedform}} 
        }
      }
    $\hat{\mathbf{W}}^{(\ell+1)} = \mathbf{W}^{(\ell+1)} \times_2 \boldsymbol{\S}^{(\ell)^T} $
    }
\Return $\hat{\mathbf{\Theta}}$
\end{algorithm}


\smalltitle{One-to-one vs. LBYL}
In one-to-one compensation approaches \cite{NM,Data-free}, they deliver the missing information for a pruned filter only to the most similar one of the remaining filters as shown in Figure \ref{fig:matrix:c}. Thus, this assumption is identical to the case that we have only one $s_{k}$ in Eq. (\ref{eq:goal2}), which would return a quite rough solution for the problem of minimizing the reconstruction error. Indeed, this one-to-one approach particularly fails to reduce the RE term as shown in Figure \ref{fig:error_components} of our experiments.

\begin{table*}[t] % 
\centering
{\scriptsize 
\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{VGG-16 (Acc. 93.7)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{92.04} & 91.93 & 89.43 & \textbf{92.15} & 91.82 & 88.83 & 91.85 & \textbf{91.97} & 89.85 & \textbf{88.05} & 86.52 & 74.87 \\\hline
20\%& \textbf{87.84} & 87.24 & 71.77 & \textbf{87.97} & 86.42 & 72.04 & \textbf{89.51} & 86.93 & 73.64 & \textbf{75.24} & 63.33 & 37.19 \\ \hline
30\%& \textbf{83.25} & 76.91 & 56.95 & \textbf{82.83} & 75.58 & 52.40 & \textbf{81.80} & 75.01 & 49.79 & 45.67 & \textbf{46.86} & 12.81 \\ \hline
40\%& \textbf{66.81} & 54.32 & 31.74 & \textbf{67.19} & 52.24 & 30.46 & \textbf{56.63} & 52.54 & 17.78 & \textbf{31.34} & 26.79 & 10.00 \\ \hline
50\%& \textbf{45.71} & 32.58 & 12.37 & \textbf{49.46} & 32.13 & 11.71 & \textbf{43.32} & 27.87 & 10.43 & \textbf{21.56} & 18.08 & 10.00 \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{75.13} & 68.60 & 52.45 & \textbf{75.92} & 67.64 & 51.09 & \textbf{72.62} & 66.86 & 48.30 & \textbf{52.37} & 48.32 & 28.97\\ \Xhline{2\arrayrulewidth}   
\end{tabular}
}
\vspace{-1.5mm}
\caption{Recovery results of VGG-16 on CIFAR-10}
\label{tab:VGG16-CIFAR10}
\vspace{1.5mm}
% \end{table}
%%%%%%%
% \begin{table}[t]
{\scriptsize

\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{ResNet34 - ImageNet (Acc. 73.27)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{69.22} & 66.96 & 63.74 & \textbf{69.12} & 66.59 & 61.76 & \textbf{69.07} & 66.30 & 62.05 & \textbf{65.90} & 64.75& 52.97 \\ \hline
20\%& \textbf{62.49} & 55.70 & 42.81 & \textbf{62.27} & 55.39 & 43.45 & \textbf{61.18} & 53.95 & 40.61 & \textbf{50.64} & 48.40& 18.62 \\ \hline
30\%& \textbf{47.59} & 39.22 & 17.02 & \textbf{49.43} & 37.97 & 15.74 & \textbf{46.88} & 35.56 & 12.58 & 22.92 & \textbf{23.69} & 1.35  \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{59.77} & 53.96 & 41.19 & \textbf{60.27} & 53.32 & 40.32 & \textbf{59.04} & 51.94 & 38.41 & \textbf{46.49} & 45.61& 19.10\\ \Xhline{2\arrayrulewidth}
\end{tabular}
}
\vspace{-1.5mm}
\caption{Recovery results of ResNet-34 on ImageNet}
\label{tab:ResNet34-ImageNet}
\vspace{1.5mm}

% \end{table}
% \begin{table}[t]
{\scriptsize

\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{ResNet101 - ImageNet (Acc. 77.31)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune
\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{74.59} & 72.36 & 68.90 & \textbf{74.54} & 72.38 & 68.38 & \textbf{74.19} & 72.05 & 68.33 & \textbf{59.78} & 57.13 & 46.55 \\ \hline
20\%& \textbf{68.47} & 61.42 & 45.78 & \textbf{69.03} & 61.02 & 46.25 & \textbf{68.52} & 60.57 & 44.57 & \textbf{34.85} & 15.78 & 6.83  \\ \hline
30\%& \textbf{55.51} & 37.38 & 10.32 & \textbf{56.65} & 33.74 & 7.65  & \textbf{56.11} & 36.43 & 9.32  & \textbf{13.27} & 2.31  & 0.60  \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{66.19} & 57.05 & 41.67 & \textbf{66.74} & 55.71 & 40.76 & \textbf{66.27} & 56.35 & 40.74 & \textbf{35.97} & 25.07 & 17.99\\\Xhline{2\arrayrulewidth}
\end{tabular}
}
\vspace{-1.5mm}
\caption{Recovery results of ResNet-101 on ImageNet} \label{tab:ResNet101-ImageNet}
\vspace{1.5mm}
\end{table*}


\subsection{Our Train-Free Recovery Method with a Closed Form Solution}
Based on our data-free loss function in Eq. (\ref{eq:loss}), we now present our proposed train-free recovery method, called LBYL. First of all, we theoretically prove that the problem of minimizing $\mathcal{L}_{re}$ of Eq. (\ref{eq:loss}) has a closed form solution at the following theorem.
\begin{theorem} \label{thm:closedform}
The loss function $\mathcal{L}_{re}$ of Eq. (\ref{eq:loss}) is convex with a unique optimal solution as follows:
\begin{equation}
\small
    \boldsymbol{s}=[X^{T}X+\lambda_{1}\frac{\gamma_{j}^2}{\sigma_{j}^2} \boldsymbol{p}\boldsymbol{p}^{T}+\lambda_{2}I]^{-1}[X^{T}\boldsymbol{y}+\frac{\lambda_{1}\gamma_{j}}{\sigma_{j}}(\frac{\mu_{j}\gamma_{j}}{\sigma_{j}}-\beta_{j})\boldsymbol{p}],
    \nonumber
\end{equation}
where (1) $X = [\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{1}}{\sigma_{1}}\boldsymbol{f_{1}}~~...~~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j-1}}{\sigma_{j-1}}\boldsymbol{f_{j-1}}~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j+1}}{\sigma_{j+1}}\boldsymbol{f_{j+1}}~~...~~ \\
\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{m}}{\sigma_{m}}\boldsymbol{f_{m}}]$ such that $\boldsymbol{f_{i}}$ is the vectorized $i$-th filter in the $\ell$-th layer, (2) $\boldsymbol{y}$ is the vectorized $j$-th filter in the $\ell$-th layer, and (3) $\boldsymbol{p} =  [p_{1}~...~p_{j-1}~p_{j+1}~...~p_{m}]^T$ such that $p_{i} ={\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{i}}{\sigma_{i}}}{(\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i})}$.
% where (1) $X = [~...~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j-1}}{\sigma_{j-1}}\boldsymbol{f_{j-1}}~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j+1}}{\sigma_{j+1}}\boldsymbol{f_{j+1}}~...~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{m}}{\sigma_{m}}\boldsymbol{f_{m}}]$ such that $\boldsymbol{f_{i}}$ is the vectorized $i$-th filter in the $\ell$-th layer, (2) $\boldsymbol{y}$ is the vectorized $j$-th filter in the $\ell$-th layer, and (3) $\boldsymbol{p} =  [p_{1}~...~p_{j-1}~p_{j+1}~...~p_{m}]^T$ such that $p_{i} ={\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{i}}{\sigma_{i}}}{(\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i})}$.
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

Finally, given $\lambda_{1}$ and $\lambda_{2}$, Algorithm \ref{alg:Recovery} presents the whole procedure of our LBYL method using the closed form solution in Theorem \ref{thm:closedform}.

\smalltitle{Extension of LBYL to neuron pruning}
Even though this paper focuses on filter pruning, our LBYL method can also be applied to prune and restore neurons in vanilla feedforward neural networks consisting of only FC layers. We present the details in Appendix due to the space limitation.

% based on LBYL assumption in real time using the closed form solution in Theorem 1. Actually, this restoration algorithm can be extended to multiple pruned filters through just implementing above works iteratively. We represent the whole procedure in Algorithm \ref{alg:Recovery}.



% \smalltitle{Reasonable loss function}
% As shown in Lemma 2, there are three error components in (12), which are related with Sum of Squared Error(SSE) and Batch normalization Error(BE) and Activation Error(AE), respectively. Unfortunately, we cannot control data driven feature map $\mathbf{Z}^{(\ell-1)$ and matrix $R$. So we alternatively try to minimize the norm of two terms, $\boldsym{\epsilon}$ and $B$ respectively. Moreover, we place regularization term in loss function lastly for the purpose of mitigating explosion of matrix $R$. For example, one element of matrix $R$ maybe too large if some of the coefficients are positively large and elements corresponding to that coefficients are negative, but elements corresponding to others are positive. Finally, we formulate the reasonable restoration loss function as below Eq.(16).








% \begin{lemma} If there are both BN and ReLU between feature map and activation map, the reconstruction error can be formulated in a data-free manner as follows:
%     \begin{equation} 
%     \| \mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)}\|_{1}=
%      \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{Z}^{(\ell-1)}\circledast\boldsymbol{\epsilon})}+ B + R\|_{1},
%      \end{equation}\nonumber
%      \label{lemma}
% where $\mathbf{\epsilon}=\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)}$, $B$=$\gamma_{j} \over \sigma_{j}$$\{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j $, $R$ is w $\times$ h matrix where $ R_{u,v}$ = |$\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,u,v}^{(l+1)})-min(0,\mathbf{Z}_{j,u,v}^{(l+1)})$|, and $\mu,\gamma,\sigma,\beta$ are the batch normalization parameters.
% \end{lemma}
% where,$\mathbf{\epsilon}=\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)}$, $B$=$\gamma_{j} \over \sigma_{j}$$\{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j $, $R$ is w $\times$ h matrix where $ R_{u,v}$ = |$\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,u,v}^{(l+1)})-min(0,\mathbf{Z}_{j,u,v}^{(l+1)})$|, and $\mu,\gamma,\sigma,\beta$ are the batch normalization parameters.



 

% Our approximation scale for pruned filter in $\ell$-th layer is computed to recovery filters in $\ell+1$-th layer. Algorithm of our proposed method is largely two parts. In the case of remained filter, we do not compute the approximation scale. And in the case of pruned filter, we compute the approximation scale on remained filters. Through the process to minimize Eq. (\ref{eq:eq10}), we can get the approximation scales for preserved filter. Approximation scale is computed each $\ell$-th layers that perform pruning.

 
 
 
%  is vectorized $i$-th filter in $l$-th layer for $i \in [1,m_{l}] \setminus$ \{$j$\}, $\boldsymbol{y}$ is vectorized $j$-th filter in $l$-th layer, $\boldsymbol{p}$ is ($m_{l}-1$)-dimensional vector whose i-th component is $\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}$ for $i \in [1,m_{l}] \setminus$ \{$\textit{j}$\}.

% Meanwhile, our LBYL method can have more flexibility in Error components. We consider a reasonable loss function that reflect all error components comprehensively. Through this loss function, we can find more optimal solution $\boldsymbol{s}$ in Eq.(10) than One-to-One compensation method.





% They consider SSE and BE and AE to a degree, but their methods are so heuristic and can have large disadvantage of SSE. For example, Kim \textit{et.al} \cite{NM} choose one of the preserved filters based on their customized score which reflect SSE and BE at different degree. This degree is decided by parameter $\lambda$ which need to be searched. Furthermore, Kim \textit{et.al} \cite{NM} decide whether to compensate or not based on cosine similarity between the preserved and pruned filter at the end. That is, they are both depend on the similarity between pruned and preserved filter, and they suffer from little similarity in some layers as shown in \cite{NM} which result in large SSE. On the other hand, they may have advantage in terms of BE since they have only one BN parameter in $\boldsymbol{B}$ term. 




% We should consider batch normalization to minimize reconstruction form. In case of BN, we also assume that the the feature map $\mathbf{Z}_{j,:,:}^{(\ell+1)}$ generated by pruned filter $\mathbf{W}_{j,:,:,:}^{(\ell)}$ can be represented linear combination of feature maps $\mathbf{Z}_{i,:,:}^{(\ell+1)}$ generated by preserved filters $\mathbf{W}_{i,:,:,:}^{(\ell)} i \in [1,m] \setminus {\{$\textit j$\}}$.

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \text{Eq.} (\ref{equation1}). &= \| \N(\mathbf{Z}_{j,:,:,:}^{(\ell)}) - \sum\limits_{i = 1, i \neq j }^{m} {s}_{i}^{\prime} \times \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)} ) \|_{1} \\ 
%  &=\| \frac{\gamma_{j}(\mathbf{Z}_{j,:,:,:}^{(l)} - \mu_j)}{\sigma_{j}} + \beta_{j}- \sum\limits_{i = 1, i \neq j }^{m}{{s}_{i}^{\prime} \times \{ \frac{\gamma_{i}(\mathbf{Z}_{i,:,:,:}^{(l)} - \mu_i)}{\sigma_{i}} + \beta_{i}}\} +B \|_{1}\\
% \end{split}
% \end{eqnarray}
% where ${s}_{i}^{\prime}$ = $\frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}}{s}_{i}$ is the scale considered by batch normalization and
% we want bias caused by considering the batch normalization to be zeroed. $B=\frac{\sigma_{j}}{\gamma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j$ \} and $\mu,\gamma, \sigma$ is the batch normalization parameters $\in \mathbb{R}^{n \times w \times h}$ for feature maps. 


% % $\mathbf{B} = \frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j + \frac{\gamma_{j}}{\sigma_{j}}(\mathbf{Z}^{(\ell)}\circledast\boldsymbol{\epsilon} \} + \beta_j$ \} to $\mathbf{B}=\frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j \} + \beta_j$ \} and $\mu,\gamma, \sigma$ is the batch normalization parameters $\in \mathbb{R}^{n \times w \times h}$ for feature maps. 

% Through the lemma below, we can find the reconstruction error caused by batch normalization layer.
% \newtheorem*{lemma}{Lemma} 
% \begin{lemma} From the above equation, we can get the reconstruction error considering batch normalization.
%     \begin{equation} 
%     \| \mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)}\|_{1}  = \| \frac{\sigma_{j}(\mathbf{Z}^{(\ell-1)} \circledast \mathbf{\epsilon})}{\gamma_{j}} + B \|_{1}\\
%     \end{equation}\nonumber
% \end{lemma}

% Therefore, we want both $B$ and  $\mathbf{\epsilon}$ zero..

% \smalltitle{Considering Activation Function}
% Moreover, our assumption should extend to next layer that is activation layer. Therefore we assume that activation map generated by pruned filter can be represented by linear combination of activation maps generated by remained filters.

% \begin{eqnarray} \begin{split}\label{eq:eq}
%      \text{Eq.} (\ref{equation1}). &= \| \F\circ(\N(\mathbf{Z}_{j,:,:,:}^{(\ell)})) - \sum\limits_{i = 1, i \neq j }^{m} {s}_{i}^{\ast} \times \F\circ(\N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)})) \|_{1} \\ 
%      &= \| \F\{\N(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}),0\} - \sum\limits_{i = 1, i \neq j }^{m_{i}} \F\{\boldsymbol{s}_{i}^{\ast} \times \N(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})\} +\F(\boldsymbol{K}) \} \|_1
%      \end{split}
% \end{eqnarray}

% \begin{lemma} From the above equation, we can get the reconstruction error considering activation. More detailed derivation is in appendix.
%     \begin{equation} 
%      \| \frac{\sigma_{j}}{\gamma_{j}}(\mathbf{Z}^{(\ell)}\circledast\boldsymbol{\epsilon})+ B + AE\|_{1}
%      \end{equation}\nonumber
%      \label{lemma}
% \end{lemma}
% where, $ AE = \sum\limits_{m=1}^{h^{\prime}}\sum\limits_{n=1}^{w^{\prime}}-min(0,\mathbf{Z}_{j,m,n}^{(l+1)})+\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,m,n}^{(l+1)}) \in \boldsymbol{R}^{h^{\prime} \times w^{\prime}}$

% Finally, we should minimize $B$ and  $\mathbf{\epsilon}$ and activation error zero..


% \smalltitle{Objective Function}
% As shown in lemma(\ref{lemma}) above, we should minimize the $b$ to reduce the reconstruction error,which leads to reduction of the error caused from activation. Plus, we also reduce the difference between pruned filter and remained filters. Therefore, we design the loss to minimize reconstruction with errors we consider above.  
% \begin{equation}
%      \mathcal{L}_{re} =  \| \mathbf{W}_{j,:,:,:}^{(\ell)} - \sum\limits_{i = 1, i \neq j }^{m} s_{i} \mathbf{W}_{i,:,:,:}^{(\ell)} \|_2^{2} + \lambda_1 \|B\|_2^{2} + \lambda_2 \|s_i \|_{2}^{2},
% \label{eq:eq10}
% \end{equation}
% where $i \in [1,m] \setminus {\{$\textit j$\}}$.

% By using the loss function to find the optimized scale, we can control the three error components. First, Sum of Squared Error(\textit{SSE}) that means difference between pruned filter and linear combination of remained filters can be minimized by first terms in Eq. (\ref{eq:eq10}). Second, Batch normalization Error (\textit{BE}) that means error caused by batch normalization layer also can be reduced. Finally, the Activation Error (\textit{AE}) that error from the activation error can be decreased weakly by third term in Eq. (\ref{eq:eq10}) in the sense of preventing amplification of some coefficient $s_{i}$ that may amplify the activation error term. Through this loss function, we can find more optimal solution 
% $s$ than one-to-one compensation method. Furthermore, we investigate that minimizing loss function is truly helpful in Theorem 1 because we substitute scale ($\boldsymbol{\mathcal{S}}^{\prime}$) for scale ($\boldsymbol{\mathcal{S}}^{\ast}$) considering the activation.

% % The difference between  $\boldsymbol{Z}_{j,:,:}^{(l+1)}$ and $ \sum\limits_{n = 1, n \neq j}^{m_{l}}{S_{n}} \boldsymbol{Z}_{n,:,:}^{(l+1)}$ can be quantified as below Theorem 1.
% % \smalltitle{\textit{Theorem 1}} If we assume Eq. (\ref{eq:eq6})., we can assume s_{i}^{\prime} = \frac{\gamma_{j}}{\sigma_{j}}\frac{\sigma_{i}}{\gamma_{i}}s_{i}$ for $i \in [1,m] \setminus$ \{$j$\} and $\| \boldsymbol{Z}_{j,:,:}^{(l+1)} - \sum\limits_{n = 1, n \neq k}^{m}{S_{k}} \boldsymbol{Z}_{k,:,:}^{(l+1)}\|_{1}$ can be represented as below. The detailed derivation process is in appendix.



% From Theorem 1, we get to know that we should minimize $b$ and $\boldsymbol{\epsilon}$ and the last term concerned with activation layer to minimize the reconstruction error. Thus, in general compensation method, we should find the scalars $s_{i}$ for $i \in [1,m] \setminus$ \{$\textit{j}$\} which minimize the three error components.



% \subsection{Our Train-Free Recovery Method with a Closed Form Solution}

% Moreover, as mentioned earlier, To propose data-free and training-free method. We use the closed form solution and then compensate pruned filter in a real time. Our loss function is the loss function is convex and there exists a unique solution as shown below at Theorem 2.

% \smalltitle{\textit{Theorem 2}} The loss function in Eq. (\ref{eq:eq10}). is convex and there exists a unique optimal solution. More detailed derivation is in appendix.
% \begin{equation}
%     s_{i}=[X^{T}X+\lambda_{1}\frac{\gamma_{j}^2}{\sigma_{j}^2} \boldsymbol{p}\boldsymbol{p}^{T}]^{-1}[X^{T}\boldsymbol{y}+\frac{\lambda_{1}\gamma_{j}}{\sigma_{j}}(\frac{\mu_{j}\gamma_{j}}{\sigma_{j}}-\beta_{j})\boldsymbol{p}]
% \label{eq:eq}\nonumber
% \end{equation}
%  where $X_{:,i}$ is vectorized $i$-th filter in $l$-th layer for $i \in [1,m_{l}] \setminus$ \{$j$\}, $\boldsymbol{y}$ is vectorized $j$-th filter in $l$-th layer, $\boldsymbol{p}$ is ($m_{l}-1$)-dimensional vector whose i-th component is $\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}$ for $i \in [1,m_{l}] \setminus$ \{$\textit{j}$\}.

% Finally, given $\lambda_{1}$ and $\lambda_{2}$, we can implement many-to-one compensation Algorithm in real time using the closed form solution in Theorem 2. Actually, this compensation algorithm can be extended to multiple pruned filters through just implementing above works iteratively. We call this compensation Algorithm LBYL. We represent how LBYL works in Algorithm \ref{alg:Recovery}. Our approximation scale for pruned filter in $\ell$-th layer is computed to recovery filters in $\ell+1$-th layer. Algorithm of our proposed method is largely two parts. In the case of remained filter, we do not compute the approximation scale. And in the case of pruned filter, we compute the approximation scale on remained filters. Through the process to minimize Eq. (\ref{eq:eq10}), we can get the approximation scales for preserved filter. Approximation scale is computed each $\ell$-th layers that perform pruning.

% \begin{algorithm}[htb]
%   \caption{LBYL Algorithm}
%   \label{alg:Recovery}
%   \KwIn{$\boldsymbol{W}^{{(\ell)}}$ $\in$ $\boldsymbol{R}^{m_l \times n_l\times k \times k}$, set of remained filter $R = \{r_1, r_2, ..., r_{t_l}\}$} 
%   \KwOut{Approximation matrix $s^{(\ell)}$ $\in$ $\boldsymbol{R}^{m_{l} \times t_l}$}
   
%   Initialize ${s}^{(\ell)}$ $\in$ $\boldsymbol{R}^{m_{l} \times t_l}$ with 0
  
%   \For{each filter $w_m$ $\in$ $\mathbb{R}^{n_{l} \times k \times k}$   $\mathbf{in}$ $\mathbf{W}^{(\ell)}$}
%     {
%     \If{w_m $\in$ R} 
%         {
%         ${i} \leftarrow $index of $w_m$ within $\boldsymbol{W}^{{(\ell)}}$
        
%         $s_{i,m}^{(\ell)} \leftarrow$ 1
%         }
%     \Else{        
%     approximation~scale~list $\leftarrow$ $\underset{s^{\ell}}{\mathrm{argmin}}$ Eq. \ref{eq:eq10}.
    
%     ${i} \leftarrow $ index of $w_m$
    
%         \For{each scale $\mathbf{in}$ approximation scale list}
%             {
%                 ${j} \leftarrow $index of scale within approximation scale list
                
%                 $s_{i,j}^{(\ell)} \leftarrow $scale \times \frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}} 
                
%           }
%       }
%     }
% \Return $s^{(\ell)}$
% \end{algorithm}


% \smalltitle{Discussion on one-to-one vs. many-to-one approach}
% In one-to-one compensation \cite{NM,Data-free}, they prudently choose one of the preserved filters corresponding to one pruned filter, and then compensate like general compensation method. so in this case, there is one $s_{i}$ in Eq. (\ref{eq:eq6}).
% They consider SSE and BE and AE to a degree, but their methods are so heuristic and can have large disadvantage of SSE. For example, Kim \textit{et.al} \cite{NM} choose one of the preserved filters based on their customized score which reflect SSE and BE at different degree. This degree is decided by parameter $\lambda$ which need to be searched. Furthermore, Kim \textit{et.al} \cite{NM} decide whether to compensate or not based on cosine similarity between the preserved and pruned filter at the end. That is, they are both depend on the similarity between pruned and preserved filter, and they suffer from little similarity in some layers as shown in \cite{NM} which result in large SSE. On the other hand, they may have advantage in terms of BE since they have only one BN parameter in $\boldsymbol{B}$


%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Proposed Method} \label{sec:method}

% Most of filter pruning methods try to select filters to be pruned prudently so that pruned network's output be similar to the original network's. To this end, they prune the unimportant filters and then fine-tune the pruned network with using the train data. How can we restore the the pruned networks without any data? In other words, it implies that we cannot use any data-driven values(i.e., activation maps) and we can only exploit the values of original filters. In that case, the only thing we can do maybe changing the weights of remained filters appropriately not to amplify the difference between pruned and unpruned network's outputs through the information of original filters.



% \smalltitle{Problem Statement} For a Convolutional Neural Network (CNN) with $L$ layers, we denote $\mathbf{Z}{^{(\ell-1)}}$ $\in$ $\mathbb{R}^{n_{l} \times h_{l} \times w_{l}} $ is activation maps at $l$-th layer, where $n_{l}$, $h_{l}$ and $w_{l}$ are the number of channels, height and width in activation maps, respectively. and we denote $\mathbf{W}^{{(\ell)}}$ $\in$  $\mathbb{R}^{m_l \times n_l\times k \times k}$ is covolution filters in $l$ -th layer,where $m_l$, $n_l$ and $k$ are the number of filters, number of channels and kernel size, respectively. Trough the convolution operation using activation map $\mathbf{Z}{^{(\ell-1)}}$ and convolution filter $\mathbf{W}^{{(\ell)}}$ in $l$-th layer, the feature maps $\boldsymbol{\mathcal{A}}^{{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l} \times h_{l+1} \times w_{l+1}}$ is computed as shown in Eq. (\ref{eq:eq1}).

% \begin{equation}
% \boldsymbol\alpha^{(l+1)} = {\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)}}
% \label{eq:eq1}
% \end{equation}

% and the feature maps passed through the BN and ReLU layer are activation maps $\mathbf{Z}{^{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l} \times h_{l+1} \times w_{l+1}} $ in $i+1$ -th layer as shown in Eq. (\ref{eq:eq2}).

% \begin{equation}
% \mathbf{Z}^{(l+1)} = \mathcal{F}({\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)}})
% \label{eq:eq2}
% \end{equation}
% where $\mathcal{F}$ is the function that implement batch normalization and non-linear activation(e.g., ReLU).

% If the filter pruning is performed in $l$-th layer, the shape of original filters $\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_l \times n_l\times k \times k}$ is modified to ${\hat {\mathbf{W}}^{(\ell)}}$ $\in$ $\mathbb{R}^{t_l \times n_l\times k \times k}$, where $t_l$ $<$ $m_l$ by pruning criterion. Therefore, the pruned activation maps ${\hat {\mathbf{Z}}}{^{(l+1)}}$ $\in$ $\mathbb{R}^{t_{l} \times h_{l+1} \times w_{l+1}}$ in ($l+1$)-th layer is computed by Eq. (\ref{eq:eq3}).

% \begin{equation}
% \mathbf{\hat{Z}}^{(l+1)} = \mathcal{F}({\mathbf{Z}^{(\ell)} \circledast {\mathbf{\hat{W}}}^{(\ell)}})
% \label{eq:eq3}
% \end{equation}

% Moreover, corresponding channels of each filters in ($l+1$) -th layer are sequentially removed. As a result, shape of original filters $\mathbf{W}^{{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times m_l\times k \times k}$ in ($l+1$) -th layer is changed to  ${\hat {\mathbf{W}}^{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times t_l\times k \times k}$. Although the pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times h_{l+1} \times w_{l+1}}$ in ($l+2$) -th layer have same shape with original feature maps $\boldsymbol{\mathcal{A}}^{{(l+2)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times h_{l+1} \times w_{l+1}}$, the pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ are damaged. Thus, we make approximation scales $\testit{s}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$ with relationship between the pruned filter and preserved filters in $l$-th layer and then apply it to the original filters in ($l+1$) -th layer to compensate for pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ as shown in Eq. (\ref{eq:eq4}).
% (i.e., change $\hat{\mathbf{W}}^{(l+1)}$ to ${\mathbf{W}}^{(l+1)}$ \circledast  ${\boldsymbol{\mathcal{S}}} $)

% \begin{equation}
% \boldsymbol\alpha^{(l+2)} = {\mathbf{Z}}^{(l+1)} \circledast {\mathbf{W}}^{(l+1)}
% \approx {\hat{\mathbf{Z}}^{(l+1)} \circledast {\mathbf{W}}^{(l+1)} \circledast  {\boldsymbol{\mathcal{S}}} = \boldsymbol{\hat{\alpha}}^{{(l+2)}}}
% \label{eq:eq4}
% \end{equation}

% Our goal is finding the approximation scales $\testit{s}$ to minimize the reconstruction error between the pruned model and the original model without any data, and consequently compensating for pruned filters in neural network using this approximation scales $\testit{s}$,which can be represented as below in Eq. (\ref{eq:eq5}).

% \begin{equation}
% \boldsymbol{\mathcal{S}} =  \underset{{\mathcal{S}}}{\mathrm{argmin}} \sum\limits_{{i} = 1}^{m_{l+1}}\|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}-\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+2)}}}\|_1
% \label{eq:eq5}
% \end{equation}


% \kim{From this part(below), should be checked thoroughly again!! this part is so important. There are too many mathematical expression error.....}
% \subsection{One-to-one compensation}
% As mentioned in introduction, in one-to-one compensation, they assume that one pruned filter can be approximated by one remained filter\cite{NM,Data-free}(i.e., $ W_{pruned} \approx S\circledastW_{remained} $ ). And more clearly, This can be represented as below.\kim{the below equation and below sentences are not matched each other! You should check it carefully!}


% \begin{equation}
% % \boldsymbol{W}_{j,:,:,:}^{(\ell)} ={\boldsymbol\beta}_{:,j}^{(\ell)} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)}  + \boldsymbol{\epsilon}
% \boldsymbol{W}_{j,:,:,:}^{(\ell)} = \boldsymbol{S} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} 
% \label{eq:eq6}
% \end{equation}
% where $i$-th filter is the the preserved filter in $l$ -th layer and $j$-th filter is the pruned filter in the same layer and $\mathcal{S}$ is the scale and ${\boldsymbol{\epsilon}}$ is the residual. \kim{I think that the definition of scale more clearly.}

% the reconstruction error formula can be represented as below.
% \begin{eqnarray} \begin{split}\label{eq:eq7}
%         \mathcal{L}_{re} = \sum\limits_{{i} = 1}^{m_{l+1}} \|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}- \mathcal{F}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}}) \circledast  \mathbf{W}_{i,:,:,:}^{(l+1)} \circledast \boldsymbol {\mathcal{S}}_{i,:}^{(\ell)}\|_1 
% \end{split}
% \end{eqnarray}
% The channels of preserved filter in ($l+1$)-th layer are compensated using the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ obtained from the relationship between pruned filter and preserved filter in $l$-th layer \cite{NM,Data-free}. \cite{NM} first prudently choose one of the preserved filters corresponding to each pruned filter in $l$-th layer based on the cosine similarity and bias caused by batch normalization. Then calculate the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ reflecting the batch normalization scale. Finally, \cite{NM} determine whether to apply the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ to the original filters or not.\kim{I think the exact description about S is needed!!}

% \subsection{Many-to-one compensation}
% We propose the many-to-one compensation method to sufficiently compensate for the pruned filter. To this end, we approximate the pruned filter with the linear combination of preserved filter. Actually, one-to-one compensation ignore the residual term. in real case, there exists non trivial residual. Therefore it can be showed more clearly as below Eq. (\ref{eq:eq7}).

% \begin{equation}
% \boldsymbol{W}_{j,:,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)}  + \boldsymbol{\epsilon} 
% \label{eq:eq8}
% \end{equation}

% The reconstruction error about the many-to-one compensation can be represented using Eq. (\ref{eq:eq9}).


% \begin{eqnarray} \begin{split}\label{eq:eq9}
%     \mathcal{L}_{re} = \sum\limits_{{i} = 1}^{m_{l+1}}\|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}- \mathcal{F}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}}) \circledast  \mathbf{W}_{i,:,:,:}^{(l+1)} \circledast \boldsymbol{{\mathcal{S}}}_{i,:}^{(\ell)}\|_1 
% \end{split}
% \end{eqnarray}
% where $\boldsymbol{\mathcal{K}}$ = $\frac{\gamma_{j}}{\sigma_{j}}[\sum\limits_{{i} = 0 , i \neq j}^{m_{i}}\{(\boldsymbol{S}_{i}\mu_{i} -\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}) - \mu_{j} \} ]+ \beta_{j}$ is bias term about the batch normalization. The derivation process for the above reconstruction error formula is in appendix.\kim{Where is K?? and to add it in appendix, you prefer to make it Lemma or Theorem!!}


% \smalltitle{\textit{Approximation for scale}} To find out the optimized approximation scale for compensation, We start from our assumption pruned filter is represented by linear combination of multiple filters in $l$-th layer and extend our assumption to up to next activation maps in $l+1$-th layer and then compute the approximation scale. First, we can extend our assumption to the followed feature map generated by pruned filter using our assumption as shown below.
% \begin{equation}
% \boldsymbol{\alpha}_{j,:,:}^{(l+1)} =\sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i} \times \boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{W}_{i,:,:,:}^{(\ell)}   +  \boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{\epsilon}
% \label{eq:eq10}
% \end{equation}



% As we assume that the pruned filter is represented by linear combination of preserved filter, in batch normalization layer, we can also assume that the the feature map generated by pruned filter can be represented linear combination of feature maps generated by preserved filters as shown in Eq. (\ref{eq:eq11}). \kim{at below equation, what is mi? is m depend on i? this is strange. }

% \begin{eqnarray} \begin{split}\label{eq:eq11}
%     \boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) &= \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})    +\boldsymbol{K} \\
%  \frac{\gamma_{j}(\boldsymbol{\alpha}_{j,:,:}^{(\ell)} - \mu_j)}{\sigma_{j}} + \beta_{j} & =  \sum\limits_{i = 1, i \neq j }^{m_{i}}{\boldsymbol{S}_{i}^{\prime} \times \{ \frac{\gamma_{i}(\boldsymbol{\alpha}_{i,:,:}^{(\ell)} - \mu_i)}{\sigma_{i}} + \beta_{i}}\} +\boldsymbol{K} \\
% \end{split}
% \end{eqnarray}
% \kim{K dimension error!! Add operation cannot be used!}
% where $\boldsymbol{S}_{i}^{\prime} = \frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}}\boldsymbol{S}_{i}$ and $\boldsymbol{K} = \frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m_{i}}(\boldsymbol{\alpha}_{j,:,:}^{(\ell)}\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j + (\boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{\epsilon})\} + \beta_j$.

% And our assumption should extend to next layer that is activation layer as shown in Eq. (\ref{eq:eq12}). 
% \begin{eqnarray} \begin{split}\label{eq:eq12}
%     \boldsymbol{max}\{\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}),0\} &= \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{max}\{\boldsymbol{S}_{i}^{\ast} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}),0\} +\boldsymbol{max}(\boldsymbol{K},0)
% \end{split}
% \end{eqnarray}
% Unfortunately, we can't extend our assumption without any data. That is, it means we should consider all cases for possible branches. Therefore, we extend our assumption feature maps passed through the batch normalization layer in $l+1$-th layer as shown in Eq. (\ref{eq:eq13}). 
% \begin{eqnarray} \begin{split}\label{eq:eq13}
%     \boldsymbol{\alpha}_{j,:,:}^{(l+2)} & = \boldsymbol{BN}(\boldsymbol{\alpha}_{:,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,:,:,:}^{(l+1)}) \\
%     &\approx \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{\acute{W}}_{j,i,:,:}^{(l+1)}) = \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}\{\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast (\boldsymbol{W}_{j,i,:,:}^{(l+1)}+\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{W}_{j,j,:,:}^{(l+1)}) \}\\
%     &=\sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,i,:,:}^{(l+1)}) + \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}) \circledast  \boldsymbol{W}_{j,j,:,:}^{(l+1)}\\
%     &=\sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,i,:,:}^{(l+1)}) + (\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \boldsymbol{K})\circledast  \boldsymbol{W}_{j,j,:,:}^{(l+1)}   % \text{ by Eq. }(\ref{eq:eq11})
% \end{split}
% \end{eqnarray}

% we should minimize $\boldsymbol{K}$,which leads to ultimately reduce the reconstruction error in $l$-th layer induced from removed filter in $l$-th layer the from Eq. (\ref{eq:eq13}). 
% Moreover, we decompose $\boldsymbol{K}$ to optimize the the approximation scale that minimize the reconstruction error and discover that the $\boldsymbol{K}$ is composed of three error terms,which are Sum of Squares Error (\textit{SSE}, $\boldsymbol{\varepsilon}$), Batch Normalization Error (\textit{BE}, \boldsymbol{K}) and Activation Error (\textit{AE}, $\boldsymbol{\mathds{1}}$).
% \begin{eqnarray} \begin{split}\label{eq:eq14}
%         \boldsymbol{\|\boldsymbol{K}\|_1} & =  \|\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})  \|_1 \\
%         & = \|\boldsymbol{\varepsilon} -\boldsymbol{\mathds{1}}\times\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) + \sum\limits_{i = 0, i \neq j }^{m_i}\boldsymbol{\mathds{1}_{i}} \times\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}) \|_1 \\
%         & \le  \|\boldsymbol{\varepsilon}\|_1 + \|\sum\limits_{i = 0, i \neq j }^{m_i}\boldsymbol{\mathds{1}_{i}} \times\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})  -\boldsymbol{\mathds{1}}\times\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)})\|_1
% \end{split}
% \end{eqnarray}
% where $\boldsymbol{\mathds{1}}$ is the indicator variable$\boldsymbol{\varepsilon}$ = $\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})$. \kim{Is it better than the direc delta? and the indicator notation is not correct!! you should describe about indicator more clearly!}

% Therefore, we set a reasonable loss function as below that can overall control SSE and BE (and weakly AE through L2-regularization) Eq. (\ref{eq:eq14}) and optimizing this loss function, we can obtain nicely a closed form solution as Theorem 1.

% \smalltitle{\textit{Theorem 1}} The unique closed form solution. we will use the property of positive definite matrix and weak vector calculus to prove that (in appendix). \kim{The sentence in Theorem 1 is not that!!}
% \begin{equation}
%     \mathcal{L}_{re} =  \| \boldsymbol{W}_{j,:,:,:}^{(\ell)} - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{\mathcal{S}}^{l} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} \|_2 + \boldsymbol{\lambda_1} {\|\boldsymbol{K}\|_2} + \boldsymbol{\lambda_1} {\|\boldsymbol{\mathcal{S}}^{(\ell)}\|_2}
% \label{theorem:theorem1}
% \end{equation}

% Using this closed form solution, we can compensate pruned filter in a real time. we call this compensation method LBYL. LBYL can have advantage in the perspective of SSE. Furthermore, LBYL also reduces other error components (BE, AE) so that pruned filter can be compensated more optimally.\kim{there are some nuance difference.. for example.. are we reducing all BE and AE??(specifically we are not controlling AE clearly!!) I think the previous representation that I wrote is more valid.......} There is the whole procedure of LBYL described in Algorithm 1.


% \begin{algorithm}[tb]
%   \caption{Compensation Algorithm}
%   \label{alg:Compensation}
%   \KwIn{$\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_l \times n_l\times k \times k}$, set of remained filter $R = \{r_1, r_2, ..., r_{t_l}\}$, set of pruned filter $P = \{p_1, p_2, ..., p_{m_{l}-{t_l}}\}$}
%   \KwOut{Approximated scale matrices $\boldsymbol{\mathcal{S}}^{l}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$}
   
%   Initialize $\boldsymbol{\mathcal{S}}^{l}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$ with 0 \;
  
%   \For {each filter w_m $\in$ $\mathbb{R}^{n_{l} \times k \times k}$ \  $\mathbf{in}$ \ \mathbf{W}^{(\ell)}}
%     {
%     \If{w_m $\in$ $R$} 
%         {
%         ${i} \leftarrow $index of $w_m \ $within \mathbf{W}^{{(\ell)}} \\
%         $\boldsymbol{\mathcal{S}}_{i,m}^{(\ell)} \leftarrow$ 1
%         }
        
%     \Else{
%         ${approximation \ scale \ list} \leftarrow $ \underset{\mathcal{S}^{l}}{\mathrm{argmin}} Eq. \ref{eq:eq12} \\
%         ${i} \leftarrow $index of w_m \\
        
%         \For {scale $\mathbf{in}$ approximation scale list}
%         {
%             ${j} \leftarrow $index of scale within approximation scale list \\
%             ${\boldsymbol{\mathcal{S}}_{i,j}^{(\ell)}} \leftarrow scale $\\
            
%         }
%         }
%     }
%     \Return $\boldsymbol{\mathcal{S}}^{(\ell)}$
% \end{algorithm}





% \begin{equation}
% {\boldsymbol{\tilde{\mathbf{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast \mathbf{W}_{i,k}^{(\ell+1)}
% \label{eq:eq}
% \end{equation}




% By compensation in a manner like Eq.(4), the pruned feature map (5) change to the compensated feature map ${{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}}$ as below Eq.(7).

% \begin{equation}
% {{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast (\mathbf{W}_{i,k}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j}^{(\ell+1)})
% \label{eq:eq}
% \end{equation}




% By using Eq.(8), the reconstruction error of feature map in $(\ell+1)$-th layer can be represented as below Eq.(9).





% \smalltitle{Without BN, ReLU}
% As shown in Eq.(11), we should find scalars $s_{k}$ such that $\mathbf{A}_{j}^{(\ell+1)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(l+1)}$ to minimize the reconstruction error (5). We start the error analysis cosidering the situation where there are no BN and ReLU between feature map and activation map. BN and ReLU will be reflected sequentially. In that case, $\mathbf{A}^{(\ell)} = \mathbf{Z}^{(\ell)}$ and as a result, (12) can be represented as below Eq.(13).

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1} \\
%      = &~\| (\mathbf{Z}^{(\ell-1)}  \circledast (\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}

% Since we cannot control the data driven feature map $\mathbf{Z}^{(\ell-1)}$, the only thing we can do is minimizing the term $(\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)} )$ which is called SSE.

% In order for the information carried by the pruned filter to be delivered to the other filters at the same layer, we have to examine how the value of the pruned filter is related to those of the others. Our proposed assumption is that a pruned filter can be represented as a \textit{linear combination} of all the preserved filters. Let $\mathbf{W}_{j,:,:,:}^{(\ell)}$ denote such a pruned filter at the $\ell$-th layer. Then, it can be represented as follows:
% \begin{equation}
% \mathbf{W}_{j,:,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m} s_{i} \times \mathbf{W}_{i,:,:,:}^{(\ell)}  + \epsilon,
% \label{eq:linear}
% \end{equation}
% where $s_i$ quantifies to what extent each $i$-th preserved filter can contribute to form the pruned filter and $\epsilon$ is an approximation error.


% With the proposed assumption of Eq. (\ref{eq:linear}), let us examine how the reconstruction error of Eq. (\ref{eq:goal}) can further be derived in a way of not using any data-dependent values.

% Meanwhile, $i$-th channel of feature map $\mathbf{Z}_{i,:,:}^{{(\ell+1)}}$ in $(\ell+1)$-th layer can be showed as below.

% \begin{equation}
% {{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1}^{m} {\mathbf{A}}_{k,:,:}^{(\ell)} \circledast \mathbf{W}_{i,k,:,:}^{(\ell+1)}
% \label{eq:eq3}
% \end{equation}

% The pruned feature map in the same position can be showed as below.

% \begin{equation}
% {\boldsymbol{\tilde{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k,:,:}^{(\ell)} \circledast \mathbf{W}_{i,k,:,:}^{(\ell+1)}
% \label{eq:eq}\nonumber
% \end{equation}

% And the compensated feature map in the same position can be showed as below.

% \begin{equation}
% {\tilde{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1}^{t}\mathbf{\tilde{A}}_{k,:,:}^{(\ell)}\circledast({\mathbf{W}}^{(\ell+1)} \times_{2} \boldsymbol{\mathcal{S}})_{i,k,:,:}
% \label{eq:eq4}
% \end{equation}

% By a few manipulation, we can make approximation matrix $\boldsymbol{\mathcal{S}}$ so that a pruned channel corresponding to a pruned filter in $l$-th layer is divided into preserved channels in each filters in $(l+1)$-th layer. Through this matrix, we can make compensated feature map ${\tilfde{\mathbf{Z}}_{i,:,:}^{{(l+1)}}}$ which is represented as below.

% \begin{equation}
% {{\tilde{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k,:,:}^{(\ell)} \circledast (\mathbf{W}_{i,k,:,:}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j,:,:}^{(\ell+1)})
% \label{eq:eq}\nonumber
% \end{equation}

% Then, using Eq. (\ref{eq:eq3}). and Eq. (\ref{eq:eq4})., the reconstruction error after pruning and compensation can be represented as below.

% \begin{equation}
% {\mathbf{Z}_{i,:,:}^{{(\ell+1)}}}-{\mathbf{\tilde{Z}}_{i,:,:}^{{(l+1)}}}=(\mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)})\circledast\mathbf{W}_{i,j,:,:}^{(l+1)}
% \label{eq:eq5}
% \end{equation}

% And using Eq. (\ref{eq:eq5})., the whole reconstruction error of feature maps in $(\ell+1)$-th layer can be represented as below Eq. \ref{eq:eq6}).

% \begin{equation}
% \sum\limits_{{i} = 1}^{m^{\prime}}\|{\mathbf{Z}_{i,:,:}^{{(\ell+1)}}-\mathbf{\hat{Z}}_{i,:,:}^{{(\ell+1)}}}\|_1 = \sum\limits_{{i} = 1}^{m^{\prime}}\|(\mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)})\circledast\mathbf{W}_{i,j,:,:}^{(\ell+1)}\|_1
% \label{eq:eq6}
% \end{equation}


% \smalltitle{Without BN, ReLU}
% As shown in Eq. (\ref{eq:eq6})., we should find scalars $s_{k}$ such that $\mathbf{A}_{j,:,:}^{(\ell+1)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(l+1)}$ to minimize the reconstruction error. 

% \begin{equation}
% \mathbf{Z}_{j,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m} {s}_{i} \times \mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)} +  \mathbf{Z}^{(\ell-1)} \circledast \boldsymbol{\epsilon}
% \label{eq:eq7}
% \end{equation}

% \smalltitle{Considering BN} Now we should consider Batch Normalization to minimize Eq. (\ref{eq:goal2}). In this case, $\mathbf{A}^{(\ell)} = \N(\mathbf{Z}^{(\ell)})$, where $\N$ is Batch Normalization function and as a result (12) can be represented as below Eq.(14).

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \N (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}































% % In that case, reconstruction error formula Eq.(\ref{eq:eq5}) can be represented as theorem (\ref{theorem:theorem2})
% % If we compensate one filter with multiple filters, the reconstruction error formula can be obtained as below.
% To optimize the the approximation scale that minimize the reconstruction error, we decompose the how the reconstruction error consist of and discover that the reconstruction error is composed of three error terms,which are Sum of Squares Error(SSE), Batch Normalization Error(BE) and Activation Error(AE).

% \smalltitle{\textit{Theorem 1}} The reconstruction error is decomposed as below.
% \begin{eqnarray} \begin{split}\label{Theorem:Theorem1}
%         \boldsymbol{\|\mathcal{K}\|_1} & =  \|\boldsymbol{\alpha}_{j}^{{(l+1)}} - \sum\limits_{i = 0, i \neq j }^{m_i} {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}} \|_1 \\
%         & = \|\boldsymbol{\varepsilon} -\boldsymbol{\mathds{1}}\times\boldsymbol{\alpha}_{j}^{{(l+1)}} + \sum\limits_{i = 0, i \neq j }^{m_i}(\boldsymbol{\mathds{1}_{i}} \times {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}}) \|_1 \\
%         & \le  \|\boldsymbol{\varepsilon}\|_1 + \|\sum\limits_{i = 0, i \neq j }^{m_i}(\boldsymbol{\mathds{1}_{i}} \times {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}})  -\boldsymbol{\mathds{1}}\times\boldsymbol{\alpha}_{j}^{{(l+1)}}\|_1
% \end{split}
% \end{eqnarray}
% where, $\boldsymbol{\mathds{1}}$ is the indicator variable, $\boldsymbol{\varepsilon}$ = $\|\boldsymbol{\alpha}_{j}^{{(l+1)}} - \sum\limits_{i = 0, i \neq j }^{m_i} {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}} \|_1$. More detailed derivation above formula is in appendix. \kim{Is it better than the direc delta?}

% As we can see, Theorem (\ref{theorem:theorem2}) is generalized version of Theorem (\ref{theorem:theorem1}).
% We set a reasonable loss function as below that can overall control SSE and BE (and weakly AE through L2-regularization) Eq. \ref{eq:eq12} and optimizing this loss function, we can obtain nicely a closed form solution as Theorem \ref{theorem:theorem3}

% \begin{equation}
% loss = \| \boldsymbol{W}_{j,:,:,:}^{(\ell)} - \boldsymbol{\beta} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} \|_2 + \boldsymbol{\lambda_1} {\|\boldsymbol{\mathcal{K}}\|_2} + \boldsymbol{\lambda_1} {\|\boldsymbol{\beta}\|_2}
% \label{eq:eq12}
% \end{equation}

% \smalltitle{\textit{Theorem 3}} \kim{the unique closed form solution. we will use the property of positive definite matrix and weak vector calculus to prove that (in appendix).}
% \begin{eqnarray} \begin{split}\label{theorem:theorem3}
%     \mathcal{L}_{re} = 
% \end{split}
% \end{eqnarray}

% Using this closed form solution, we can compensate pruned filter in a real time. we call this compensation method LBYL(leave Before You Leave). LBYL can have advantage in the perspective of SSE. Furthermore, LBYL also relect other error components(BE,AE) so that pruned filter can be compensated more optimally.\kim{The whole procedure of LBYL is described in Algorithm 1.}



% As the pruned filter is represented by similar preserved filter, the activation maps generated by pruned filter can represent as shown in Eq. (\ref{eq:eq7}) because both pruned filter and preserved filter have same activation maps $\mathbf{Z}^{(\ell)}$

% \begin{equation}
% \boldsymbol{\hat{\alpha}}_{j,:,:}^{(l+1)} =\mathcal{S} \times \boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}  + \boldsymbol{\epsilon}  \circledast \mathbf{Z}^{(\ell)} 
% \label{eq:eq7}
% \end{equation}

% However, \cite{NM} chooses a most similar the pruned filter with preserved filter based on $\boldsymbol{\mathcal{B}}$ which consider the batch normalization as shown Eq. (\ref{eq:eq8}) and then recompute scale $\mathcal{S}$ as adjusted scale $\mathcal{K}$. 

% \begin{equation}
% \boldsymbol{BN}(\boldsymbol{\hat{\alpha}}_{j,:,:}^{{(l+1)}}) =\mathcal{K} \times \boldsymbol{BN}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}})  + \boldsymbol{\mathcal{B}}
% \label{eq:eq8}
% \end{equation}
% where $\mathcal{K}$ = s$\frac{\gamma_{j}\sigma_{i}}{\gamma_{i}\sigma_{j}}$, $\boldsymbol{\mathcal{B}}$ = $\frac{\gamma_{j}}{\sigma_{j}}[s(-\frac{\sigma_{i}\beta_{i}}{\gamma_{i}} + \mu_{i}) - \mu_{j} ] + \beta_{j}$ are the adjusted scale and bias considering the batch normalization respectively, here s = $\frac{||\boldsymbol{W}_{j,:,:,:}^{(\ell)}||_2}{||\boldsymbol{W}_{i,:,:,:}^{(\ell)}||_2}$


% Finally, \cite{NM} consider the activation layer (\textit{e.g.,} ReLU) using the non-negative cosine similarity between the pruned filter and preserved filter. In other words, scale matrices $ {\boldsymbol\beta}^{(\ell)}$ in $l$-th layer is computed for all pairs of be 

% $\mathcal{K}$  has only non-negative entries with at most one strictly positive entry per column. Therefore, the pruned filter with negative similarity is not compensated.

% % limitations
% Therefore, there are limitations of one-to-one compensation. First of all, they should decide a similarity threshold about how similar pruned filter is. That is, if not exist a sufficiently similar filter, pruned filter is not compensated. Moreover, Even if there is a quiet similar filter about the pruned filter, its residual term  is not still zero because the scale is computed based on magnitude about the pruned filter and preserved filter. In other words, they only focus on how pruned filter is similar to preserved filter. 



==> backup/ICML22_bak/problem.tex <==
\section{Problem Formulation} \label{sec:probdef}

This section formally defines the problem of restoring a given pruned network with only using its original pretrained CNN in a way free of data and fine-tuning.



% Unlike many existing works utilize data for identifying unimportant filters as well as fine-tuning to this end, we cannot evaluate the filter importance by data-dependent values like activation maps (\textit{a.k.a.} channels) as our focus in this paper is not to use any training data. Thus, in our problem setting, we can only exploit the values of filters in the original network, and thereby have to make some changes in the remaining filters of the pruned network so that the network can return the output not too much different from the original one.

% No matter how much we carefully select unimportant filters to be pruned, some kinds of retraining process appears inevitable as done by the most existing works to this end. However, since our focus in this paper is not to use any training data, we cannot evaluate the importance of filters by data-dependent values like activation maps (\textit{a.k.a.} channels). 

% To this end, they not only use a careful criterion (\textit{e.g.}, L1-norm), but also fine-tune the network using the original data.
% Most of filter pruning methods try to select filters to be pruned prudently so that pruned network's output be similar to the original network's. To this end, they prune the unimportant filters and then fine-tune the pruned network with using the train data. 

% How can we restore the the pruned networks without any data? In other words, it implies that we cannot use any data-driven values(i.e., activation maps) and we can only exploit the values of original filters. In that case, the only thing we can do maybe changing the weights of remained filters appropriately not to amplify the difference between pruned and unpruned network's outputs through the information of original filters.

\begin{figure*}[t]
	\centering
    \subfigure[\label{fig:matrix:a}Pruning matrix]{\hspace{6mm}\includegraphics[width=0.35\columnwidth]{./figure/LBYL_figure_2_1.pdf}\hspace{6mm}} 
    \subfigure[\label{fig:matrix:b}Delivery matrix for LBYL]{\hspace{6mm}\includegraphics[width=0.35\columnwidth]{./figure/LBYL_figure_2_2.pdf}\hspace{6mm}}
    \subfigure[\label{fig:matrix:c}Delivery matrix for one-to-one]{\hspace{9mm}\includegraphics[width=0.35\columnwidth]{./figure/LBYL_figure_2_3.pdf}\hspace{9mm}} 
    \caption{Comparison between pruning matrix and delivery matrix, where the $4$-th and $6$-th filters are being pruned among $6$ original filters}
	\label{fig:matrix}
	\vspace{-2mm}
\end{figure*}



\subsection{Filter Pruning in a CNN}
Consider a given CNN to be pruned with $L$ layers, where each $\ell$-th layer starts with a convolution operation on its input channels, which are the output of the previous $(\ell-1)$-th layer $\mathbf{A}^{(\ell-1)}$, with the group of convolution filters $\mathbf{W}^{{(\ell)}}$ and thereby obtain the set of \textit{feature maps} $\mathbf{Z}^{(\ell)}$ as follows:
\begin{equation}
\boldsymbol{\mathbf{Z}}^{(\ell)} = {\mathbf{A}^{(\ell-1)} \circledast {\mathbf{W}}^{(\ell)}},
\nonumber
\end{equation}
where $\circledast$ represents the convolution operation. Then, this convolution process is normally followed by a batch normalization (BN) process and an activation function such as ReLU, and the $\ell$-th layer finally outputs an \textit{activation map} $\mathbf{A}^{(\ell)}$ to be sent to the $(\ell+1)$-th layer through this sequence of procedures as:
\begin{equation}
\mathbf{A}^{(\ell)} = \F(\N(\mathbf{Z}^{(\ell)})),
\nonumber
\end{equation}
where $\F(\cdot)$ is an activation function and $\N(\cdot)$ is a BN procedure.

Note that all of $\mathbf{W}^{(\ell)}$, $\mathbf{Z}^{(\ell)}$, and $\mathbf{A}^{(\ell)}$ are tensors such that: $\mathbf{W}^{(\ell)} \in \mathbb{R}^{m \times n \times k \times k}$ and $\mathbf{Z}^{(\ell)},\mathbf{A}^{(\ell)} \in \mathbb{R}^{m \times w \times h}$, where (1) $m$ is the number of filters, which also equals the number of output activation maps, (2) $n$ is the number of input activation maps resulting from the $(\ell-1)$-th layer, (3) $k \times k$ is the size of each filter, and (4) $w \times h$ is the size of each output channel for the $\ell$-th layer.

\smalltitle{Filter pruning as n-mode product}
When filter pruning is performed at the $\ell$-th layer, all three tensors above are consequently modified to their \textit{damaged} versions, namely $\mathbf{\Tilde{W}}^{(\ell)}$, $\mathbf{\Tilde{Z}}^{(\ell)}$, and $\mathbf{\Tilde{A}}^{(\ell)}$, respectively, in a way that: $\mathbf{\Tilde{W}}^{(\ell)} \in \mathbb{R}^{t \times n \times k \times k}$ and $\mathbf{\Tilde{Z}}^{(\ell)},\mathbf{\Tilde{A}}^{(\ell)} \in \mathbb{R}^{t \times w \times h}$, where $t$ is the number of remaining filters after pruning and therefore $t < m$. Mathematically, the tensor of remaining filters, \textit{i.e.}, $\mathbf{\Tilde{W}}^{(\ell)}$, is obtained by the \textit{$1$-mode product} \cite{DBLP:journals/siamrev/KoldaB09} of the tensor of the original filters $\mathbf{W}^{(\ell)}$ with a \textit{pruning matrix} $\boldsymbol{\S} \in \mathbb{R}^{m \times t}$ (see Figure \ref{fig:matrix:a})
as follows:
\begin{eqnarray}\begin{split}\label{eq:pruning}
\mathbf{\Tilde{W}}^{(\ell)} = {\mathbf{W}}^{(\ell)} \times_{1} {\boldsymbol{\S}}^{T},\text{where }\boldsymbol{\S}_{i,k} = 
  \begin{cases} 
   1~ \text{if } i = i'_k \\
   0~ \text{otherwise}
  \end{cases} \\
  \text{s.t. } i, i'_k \in [1, m] 
  \text{ and } k \in [1, t].
  \end{split}
\end{eqnarray}
  
By Eq. (\ref{eq:pruning}), each $i'_k$-th filter is not pruned and the other $(m-t)$ filters are completely removed from $\mathbf{W}^{(\ell)}$ to be $\mathbf{\Tilde{W}}^{(\ell)}$.

This reduction at the $\ell$-th layer causes another reduction for each filter of the $(\ell+1)$-th layer so that $\mathbf{W}^{(\ell+1)}$ is now modified to $\mathbf{\Tilde{W}}^{(\ell+1)} \in \mathbb{R}^{m' \times t \times k' \times k'}$, where $m'$ is the number of filters of size $k' \times k'$ in the $(\ell+1)$-th layer. Due to this series of information losses, the resulting feature map (\textit{i.e.}, $\mathbf{Z}^{(\ell+1)}$) would severely be damaged to be $\mathbf{\Tilde{Z}}^{(\ell+1)}$ as shown below:
\begin{equation}
{\mathbf{\Tilde{Z}}}^{{(\ell+1)}} = \mathbf{\Tilde{A}}^{(\ell)} \circledast {\mathbf{\Tilde{W}}}^{(\ell+1)}~~~\not\approx~~~\mathbf{Z}^{(\ell+1)}
\label{eq:eq}\nonumber
\end{equation}
The shape of $\mathbf{\Tilde{Z}}^{(\ell+1)}$ remains the same unless we also prune filters for the $(\ell+1)$-th layer. If we do so as well, the loss of information will be accumulated and further propagated to the next layers. Note that $\mathbf{\Tilde{W}}^{(\ell+1)}$ can also be represented by the \textit{$2$-mode product} \cite{DBLP:journals/siamrev/KoldaB09} of $\mathbf{W}^{(\ell+1)}$ with the transpose of the same matrix $\boldsymbol{\S}$ as:
\begin{equation} \label{eq:pruning2}
\mathbf{\Tilde{W}}^{(\ell+1)} = {\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\S}^T}
\end{equation}




\subsection{Problem of Restoring a Pruned Network without Data and Fine-Tuning}
As mentioned earlier, our goal is to restore a pruned and thus damaged CNN without using any data and re-training process, which implies the following two facts. First, we have to use a pruning criterion exploiting only the values of filters themselves such as L1-norm. In this sense, this paper does not focus on proposing a sophisticated pruning criterion but intends to recover a network somehow pruned by such a simple criterion. Secondly, since we cannot make appropriate changes in the remaining filters by fine-tuning, we should make the best use of the original network and identify how the information carried by a pruned filter can be delivered to the remaining filters.

% For brevity, we formulate our problem here with respect to a specific layer, say $\ell$, and then it can trivially be generalized for the entire network. 
\smalltitle{Delivery matrix}
In order to represent the information to be delivered to the preserved filters, let us first think of what the pruning matrix $\boldsymbol{\S}$ means. As defined in Eq. (\ref{eq:pruning}) and shown in Figure \ref{fig:matrix:a}, each row is either a zero vector (for filters being pruned) or a one-hot vector (for remaining filters), which is intended only to remove filters without delivering any information. Intuitively, we can transform this pruning matrix into a \textit{delivery matrix} that carries information for filters being pruned by replacing some meaningful values with some of the zero values therein. Once we find such an \textit{ideal} $\boldsymbol{\S^*}$, we can plug it into $\boldsymbol{\S}$ of Eq. (\ref{eq:pruning2}) to deliver missing information propagated from the $\ell$-th layer to the filters at the $(\ell+1)$-th layer, which will hopefully generate an approximation $\mathbf{\hat{Z}}^{(\ell+1)}$ close to the original feature map as follows:
\begin{equation} \label{eq:fmap_approx}
{\mathbf{\hat{Z}}}^{{(\ell+1)}} = {\mathbf{\Tilde{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\S^*}^T})}
~~~\approx~~~\mathbf{Z}^{(\ell+1)}
\end{equation}
Thus, using the delivery matrix $\boldsymbol{\mathcal{S^*}}$, the information loss caused by pruning at each layer is recovered at the feature map of the next layer.

\smalltitle{Problem statement}
Given a pretrained CNN, our problem aims to find the best delivery matrix $\boldsymbol{\mathcal{S^*}}$ for each layer without any data and training process such that the following \textit{reconstruction error} is minimized:
\begin{equation}
\sum\limits_{i = 1}^{m'}\|{{\mathbf{Z}}_{i}^{{(\ell+1)}}-{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}}\|_1,
\label{eq:goal}
\end{equation}
where ${\mathbf{Z}}_i^{{(\ell+1)}}$ and ${\hat{\mathbf{Z}}}_i^{{(\ell+1)}}$ indicate the $i$-th original feature map and its corresponding approximation, respectively, out of $m'$ filters in the $(\ell+1)$-th layer. Note that what is challenging here is that we cannot obtain the activation maps in $\mathbf{A}^{(\ell)}$ and $\mathbf{\Tilde{A}}^{(\ell)}$ without data as they are data-dependent values.

% = \sum\limits_{i = 1}^{m'}\|{{\mathbf{Z}}_{i}^{{(\ell+1)}}-{\mathbf{\Tilde{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\mathcal{S^*}^T}})}}\|_{1}


% Our goal is finding the approximation matrix $\boldsymbol{\mathcal{S}}$ to minimize the reconstruction error between the pruned model and the original model without any data, and effectively deliver missing information for pruned filters using this approximation matrix


% $\testit{s}$,which can be represented as below.

% \begin{equation}
% \boldsymbol{\mathcal{S}} =  \underset{{\boldsymbol{\mathcal{S}}}}{\mathrm{argmin}} \sum\limits_{{i} = 1}^{m_{\ell+1}} \|{{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}-{\hat{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}}\|_{1} 
% \label{eq:eq1}
% \end{equation}



% Let us first recall that the ultimate goal of network pruning is to make the output of a pruned network as close as possible to that of its original network. Unlike many existing pruning methods, our focus is not to use any training data at all for the entire pruning and recovery process, and this implies the following two facts. First, we cannot evaluate the filter importance by data-dependent values like activation values or gradients, but have to use a pruning criterion exploiting only the values of filters themselves such as L1-norm. Furthermore, instead of fine-tuning with data, the only thing we can do for the pruned network is to make appropriate changes in the remaining filters by identifying some relationships between pruned filters and the other preserved ones without any support from data. Based on this intuition, this section mathematically and generally defines the problem of restoring a pruned neural network in a manner free of data and fine-tuning.


% Thus, we make approximation matrix $\testit{s}$ $\in$ $\mathbb{R}^{m_{\ell} \times t_{\ell}}$ with relationship between the pruned filter and preserved filters in $\ell$-th layer and then apply it to the original filters in $(\ell+1)$-th layer to compensate for pruned feature maps $\boldsymbol{\hat{\mathbf{Z}}}^{{(\ell+1)}}$ as shown below.
% (\textit{i.e.}, Let $\hat{\mathbf{W}}^{(\ell+1)}$ be ${\mathbf{W}}^{(\ell+1)}$ $\times_2$ ${{\textit{s}}} $, where $\times_2$ is 2-mode matrix product) 

% \begin{equation}
% \mathbf{Z}^{(\ell+1)} = {\mathbf{A}}^{(\ell)} \circledast {\mathbf{W}}^{(\ell+1)}
% \approx {\hat{\mathbf{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {{s}}) = {\hat{\mathbf{Z}}}^{{(\ell+1)}}}
% \label{eq:eq}\nonumber
% \end{equation}




% For a Convolutional Neural Network (CNN) with $L$ layers, we denote $\mathcal{A}{^{(\ell-1)}}$ $\in$ $\mathbb{R}^{n_{\ell -1 } \times h_{\ell -1} \times w_{\ell -1}}$ is activation maps at $\ell-1$-th layer, where $n_{\ell -1}$, $h_{\ell -1}$ and $w_{\ell -1}$ are the number of channels, height and width in activation maps, respectively. and we denote $\mathbf{W}^{{(\ell )}}$ $\in$  $\mathbb{R}^{m_{\ell} \times n_{\ell -1}\times k \times k}$ is covolution filters in $\ell$-th layer,where $m_{\ell}$, $n_{\ell-1}$ and $k$ are the number of filters, number of channels and kernel size, respectively. Trough the convolution operation using activation map $\mathcal{A}{^{(\ell-1)}}$ and convolution filter $\mathbf{W}^{{(\ell)}}$ in $\ell$-th layer, the feature maps $\boldsymbol{\mathbf{Z}}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_{\ell} \times h_{\ell+1} \times w_{\ell+1}}$ is computed as shown as below.


% \begin{equation}
% \boldsymbol{\mathbf{Z}}^{(\ell)} = {\mathcal{A}^{(\ell-1)} \circledast {\mathbf{W}}^{(\ell)}}
% \label{eq:eq1}\nonumber
% \end{equation}
% where $\circledast$ is convolution operation.

% and the feature maps passed through the BN and ReLU layer are activation maps $\mathcal{A}{^{(\ell)}}$ $\in$ $\mathbb{R}^{m_{{\ell}} \times h_{\ell+1} \times w_{\ell+1}} $ in $\ell$-th layer as shown as below.

% \begin{equation}
% \mathcal{A}^{(\ell)} = \mathcal{F}(\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)})
% \label{eq:eq2}\nonumber
% \end{equation}
% where $\mathcal{F}$ is the function that implement batch normalization and non-linear activation(\textit{e.g.}, ReLU).

% \smalltitle{Filter Pruning}
% If the filter pruning is performed in $\ell$-th layer, the shape of original filters $\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_{\ell} \times n_{\ell-1}\times k \times k}$ is modified to ${\hat {\mathbf{W}}^{(\ell)}}$ $\in$ $\mathbb{R}^{t_{\ell} \times n_{\ell-1}\times k \times k}$, where $t_{\ell}$ $<$ $m_{\ell}$ by pruning criterion. Therefore, the pruned activation maps ${\hat {\mathcal{A}}}{^{({\ell+1})}}$ $\in$ $\mathbb{R}^{t_{{\ell}} \times h_{{\ell+2}} \times w_{{\ell+2}}}$ in (${\ell+1}$)-th layer is computed as below.

% \begin{equation}
% \mathbf{\hat{A}}^{(l+1)} = \mathcal{F}({\mathbf{A}^{(\ell)} \circledast {\mathbf{\hat{W}}}^{(\ell+1)}})
% \label{eq:eq3}\nonumber
% \end{equation}

% Moreover, corresponding channels of each filters in ($\ell +1$)-th layer are sequentially removed. As a result, shape of original filters $\mathbf{W}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times m_{\ell}\times k \times k}$ in ($\ell+1$)-th layer is changed to  ${\hat {\mathbf{W}}^{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times t_{\ell}\times k \times k}$. Although feature maps ${\hat{\mathbf{Z}}}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times h_{\ell+2} \times w_{\ell+2}}$ in ($\ell+1$)-th layer after pruning have same shape with original feature maps ${\mathbf{Z}}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times h_{\ell+2} \times w_{\ell+2}}$, the pruned feature maps $\boldsymbol{\hat{\mathbf{Z}}}^{{(\ell+1)}}$ are damaged.

==> backup/ICML22_bak/related.tex <==
\section{Related Works} \label{sec:related}
Many filter pruning methods have been studied without considering such a case where we cannot use any data, whether real or synthetic, to restore a pruned network. They mostly go through an expensive retraining process either iteratively \cite{Soft,FPGM,Dynamic} or lastly as a fine-tuning phase \cite{GlobalRanking,Importance,NISP}. In this paper, we focus on the opposite case, which is more challenging in practice, where fine-tuning with any data is not available.

\smalltitle{Pruning with less fine-tuning} 
Most of the existing filter pruning methods have tried to avoid an expensive fine-tuning process by means of a carefully designed criterion for identifying unimportant filters such that the loss of information is minimized when they are pruned. To this end, they often make the best use of data-dependent values like channels and gradients that can be obtained by making inferences with some data. \citet{Thinet} propose a greedy algorithm that prunes the filters whose corresponding channels minimize the layer-wise reconstruction error. Similarly, \citet{Lasso} formulate this problem of channel selection as lasso regression and least square reconstruction. \citet{CoreSet_ICLR} introduce data-independent pruning criterion based on coreset together with an intermediate recovery method without training in order to reduce the overhead of fine-tuning. Despite their proposed methods on effective channel or neuron selection, a few epochs of fine-tuning process as well as some training data is inevitable for the pruned network to be sufficiently recovered. 


\smalltitle{Pruning with less fine-tuning and less data}
For the case of pruning with limited data, several methods \cite{CURL,Reborn} utilize knowledge distillation \cite{Knowledge_Distilation} not to use the entire original data in the recovery process. \citet{CURL} recently propose \textit{CURL} that globally prunes filters using a KL-divergence based criterion and perform knowledge distillation with a small dataset as a fine-tuning process. \citet{Reborn} tackle the similar problem and devise a way of transforming all the filters in a layer into compact ones, called \textit{reborn filters}, using only the limited data. These methods do not use the entire original data, but they still require some kinds of retraining process with a small amount of data. Meanwhile, there is a branch of data-free pruning methods \cite{Data-Free-NetworkPruning, DeepInversion} that still fine-tune the pruned model with synthetically generated data but not real data. In addition to the heavy fine-tuning process, these methods require another non-trivial training process to build a generative model for obtaining synthetic data.

\smalltitle{Pruning with no fine-tuning and no data} In the literature of filter pruning, there are only a couple of works \cite{NM, Data-free} that adopt the same problem setting as ours, that is, pruning filters without any data and fine-tuning. Both methods are based on the strong assumption that we can always find a pair of filters that are quite similar to each other and therefore a pruned filter can be compensated by its similar unpruned one. However, this assumption does not hold in modern convolutional neural networks (CNNs) having a number of filters in a fairly deep architecture. As even presented in \cite{NM}, the cosine similarity between each filter and its nearest one gets extremely low (\textit{e.g.}, around 0.2) in back layers to the point that it is better to do nothing for some pruned neurons that do not have sufficiently similar preserved neurons. In this paper, we remedy this problem by using as many preserved filters as possible to compensate for each pruned filter, and thereby propose a more robust method that successfully relaxes the assumption made by these existing works.

% \smalltitle{



% \lee{ \citet{RedPlus} focuses on reducing the number of computations by changing identical operations to identical memory access to a unique operation. That is, \citet{RedPlus} needs the hypothesis that memory access and allocation should run faster than mathematical operations, while our LBYL method do not need a specific hardware assumption. Therefore \citet{RedPlus} is orthogonal to our method. In this paper, we remedy problem of similarity based compensation \cite{NM, Data-free} by using as many preserved filters as possible to compensate for each pruned filter, and thereby propose a more robust method that successfully relaxes the assumption made by these existing works.}


==> backup/abstract.tex <==
\begin{abstract}
Although network pruning has been highly popularized to compress deep neural networks, its resulting accuracy heavily depends on a fine-tuning process that is often computationally expensive and requires the original data. However, this may not be the case in real-world scenarios, and hence a few recent works attempt to restore pruned networks without any expensive retraining process. Their strong assumption is that every neuron being pruned can be replaced with another one quite similar to it, but unfortunately this does not hold in many neural networks, where the similarity between neurons is extremely low in some layers. In this paper, we propose a more rigorous and robust method of restoring pruned networks in a fine-tuning free and data-free manner, called \textit{LBYL} (\textit{Leave Before You Leave}). LBYL significantly relaxes the aforementioned assumption in a way that each pruned neuron \textit{leaves} its pieces of information to as many preserved neurons as possible and thereby multiple neurons together obtain a more robust approximation to the original output of the neuron who just \textit{left}. Our method is based on a theoretical analysis on how to formulate the reconstruction error between the original network and its approximation, which nicely leads to a closed form solution for our derived loss function. Through the extensive experiments, LBYL is confirmed to be indeed more effective to approximate the original network and consequently able to achieve higher accuracy for restored networks, compared to the recent approaches exploiting the similarity between two neurons.
\end{abstract}



\begin{IEEEkeywords}
Article submission, IEEE, IEEEtran, journal, \LaTeX, paper, template, typesetting.
\end{IEEEkeywords}


==> backup/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
This paper proposed the problem of restoring a pruned CNN in a way free of training data and fine-tuning. We mathematically formulated how filter pruning can make a damage to the output of the pruned network, and focused on how to model the information carried by each pruned filter to be delivered to the other remaining filters. Our proposed assumption is inspired by the fact that the more the remaining filters participate in the recovery process, the better the approximation we can obtain for the original output. With this assumption, we successfully decomposed the reconstruction error into the three different components, and thereby designed a data-free loss function along with its closed form solution. Our future work would be to extend the proposed loss function so as to cover different activation functions other than ReLU.

==> backup/coverletter.tex <==
\onecolumn


\section*{Cover Letter}

\vspace{10mm}

\setcounter{table}{0}
\setcounter{figure}{0}

\renewcommand{\thetable}{C\arabic{table}}  
\renewcommand{\thefigure}{C\arabic{figure}}
\renewcommand{\thesubsection}{C\arabic{subsection}}
		
Dear ACs and reviewers for AAAI-22,

We would like to submit our paper entitled ``Leave Before You Leave: Data-Free Restoration of Pruned Neural Networks Without Fine-Tuning,'' for your consideration in AAAI-22 conference. In this version, we have made the following revisions to best appreciate all the previous comments raised by reviewers of NeurIPS-21.

\begin{enumerate}
    \item We have confirmed by new experimental results that LBYL is practically useful even when fine-tuning with data is available. Please refer to Table \ref{tab:finetune_scratch} and Figure \ref{fig:Fine tuning and From Scratch}.
    \item We have shown by supplementary experimental results on MobileNet-V2 that LBYL is also effective in tiny architectures. Please refer to Table \ref{tab:mobilenet}.
    \item We further improved our presentation quality by revising figures more descriptive, presenting a notation table in Appendix, and correcting all the typos and ambiguous expressions. Please particularly refer to Figure \ref{fig:framework} and Table \ref{tab:notations}.
    \item All the additional experimental results have been shown in either manuscript or Appendix.
\end{enumerate}


The followings are the detailed responses to each of the reviewers' comments.

\subsection*{Reviewer fQob}

\smalltitle{Comment 1}
\textit{By LBYL, the pruned network can recover the outputs of the original model with minimal approximation. But how to explain why LBYL can lead to even better performance than the original model.}

\smalltitle{Response 1}
As our goal is to approximate the layer-wise output after pruning, it would be impossible for a restored model to beat the original model. This question is probably due to the result of ResNet-50 on CIFAR-100 in Table A1 of the previous version of Appendix, where there was a typo in the table such that the accuracy of the original ResNet-50 should be 78.82, not 73.27. We have corrected this typo in this version.

\smalltitle{Comment 2}
\textit{The authors do not provide how to tackle the residual issue. How to make sure that the output is still lossless when residual connections are presented.}

\smalltitle{Response 2}
For a CNN with skip connections, we have used the common pruning scheme that prunes only first two conv layers within each residual block so that the dimension of each block's output remains the same after pruning. Furthermore, since our restoration method is only applied to each pruned layer, the output of each block would properly be restored regardless of residual connections.


\smalltitle{Comment 3}
\textit{It seems that the LBYL works well in models with much redundancy. How about the performance of trunk pruning in efficient models such as mobilenet.}

\smalltitle{Response 3}
Computationally efficient architectures such as MobileNet are already highly optimized in terms of model size, and hence pruning these compact models would lead to severe drop in accuracy. Furthermore, these tiny architectures commonly have depth-wise convolution layers, which makes us difficult to apply our restoration method in a straightforward way. Nevertheless, we have conducted a series of experiments using MobileNet-v2 using the scheme that prunes only the first layer of each block. This scheme can be seen as a naive adaptation of our method for MobileNet-v2. Table \ref{tab:mobilenet} summarizes the corresponding experimental results, where we can clearly observe that LBYL outperforms NM in most cases and is quite effective to recover the performance of pruned networks.


\smalltitle{Comment 4}
\textit{It would be nice to provide an algorithm table for a better understanding of the method.}

\smalltitle{Response 4}
Due to page limits, we have added a notation table in Appendix. Please refer to Table \ref{tab:notations}, which would further help to understand our methodology.



%%% Limitations And Societal Impact:
%%% The authors do not address the limitations and potential negative societal impact of their work. The authors can discuss how the proposed pruning method affects the development of edge AI.

% \smalltitle{Limitations and Societal Impact}
% The potential negative societal impact of our work can be to make less accurate yet lightweight models highly prevalent in the era of edge AI. This is because our method is extremely simple to implement and easy to apply to any heavyweight models even without using any data and fine-tuning.


%--> it is difficult to prune the computation efficient models such as mobile net without fine-tuning process becacues they are developed with considering the computation. However we experment the mobilenet-V2 using the scheme that prune first layer for each block and calculate the scale, compensating in the last layer. Actually, this compensation method is not fully match with our proposed method due to depthwise convolutional layer in block. but we can loose approximate the output.






\subsection*{Reviewer VxV3}

% Thank you for the very detailed and structured reviews.

%%% I don't think these implications are true. implications: The nonexistence of data implies the following two facts. First, we have to use a pruning criterion exploiting only the values of filters themselves such as L1-norm, Secondly, since we cannot make appropriate changes in the remaining filters by fine-tuning.....
%There are techniques like conserving synaptic flow... just because there's no training data doesn't mean that synthetic inputs can't be fed to the network.

\smalltitle{Comment 1}
\textit{I'd like to have seen comparisons to other data-free approaches, even if they require fine-tuning, since there can be time for fine-tuning, even if there's no data available.}


\smalltitle{Response 1}
This work is intended not to use any data regardless of whether it is real or synthetic. Nevertherless, we provide the comparison between NM and LBYL on the accuracy after fine-tuning with real data. As shown in Table \ref{tab:finetune_scratch} and Figure \ref{fig:Fine tuning and From Scratch}, we observe that LBYL converges much faster than NM in the middle of fine-tuning, and thereby achieves the best accuracy after 20 epochs of fine-tuning.





% In the CRC version, we can further clarify this issue. However, we would still like to point out the following two facts in response to your detailed comments.

% 1. \textit{conserving synaptic flow} [27] is a weight pruning (a.k.a. unstructured pruning) method, and hence it cannot be directly compared to any structured pruning methods like filter pruning that this paper focuses on. 

% 2. To the best of our knowledge, there is no existing work on fine-tuning with synthetic data a compressed model whose filters are pruned. In general, however, we agree that it would be valuable to study whether it is effective to use synthetic data generated by approaches like \textit{Deep Inversion} [2] in order to fine-tune a pruned network even though it will require heavy computation as mentioned by the reviewer.


% %%% I'd like to have seen comparisons to other data-free approaches, even if they require fine-tuning, since there can be time for fine tuning, even if there's no data available.

% Unfortunately, we have time limit for rebuttal, and therefore we cannot implement such a fine-tuning method via synthetic data for the comparison. Alternatively, we provide the comparison between NM and LBYL on the accuracy after fine-tuning with real data. As shown table below, we observe that LBYL converges much faster than NM in the middle of fine-tuning, and thereby achieves the best accuracy after 20 epochs of fine-tuning.

% \begin{table}[h]
% \centering
% \scriptsize
% \begin{tabular}{c||c|c|c} \Xhline{2\arrayrulewidth}
% Pruning ratio& LBYL& NM& Prune \\ \Xhline{2\arrayrulewidth}
% 10 \% & \textbf{78.14} $\rightarrow$ \textbf{78.3}  & 77.28 $\rightarrow$ 77.57 & 75.14 $\rightarrow$ 77.67\\\hline
% 20 \% & \textbf{76.15} $\rightarrow$ \textbf{77.22} &  72.73 $\rightarrow$ 75.62 &  63.39 $\rightarrow$ 75.4\\\hline
% 30 \% & \textbf{73.29} $\rightarrow$ \textbf{75.99} & 64.47 $\rightarrow$ 73.03 &  39.96 $\rightarrow$ 73.18\\\hline
% 40 \% & \textbf{65.21} $\rightarrow$ \textbf{74.13} & 46.4 $\rightarrow$ 69.71 &  15.32 $\rightarrow$ 70.12\\\hline
% 50 \% & \textbf{52.61} $\rightarrow$ \textbf{71.15} & 25.98 $\rightarrow$ 65.03 &  5.22 $\rightarrow$ 65.72\\\Xhline{2\arrayrulewidth}
% \end{tabular}%
% \vspace{2mm}
% \caption{Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion, where all the pruned models are fine-tuned for 20 epochs.}
% \label{cov:tab:fine-tuning}
% \end{table}


%%% While the writing is mostly understandable with few typos, I still may not understand how the technique works. If layer i is pruned, and the remaining filters share its duties, is the output of layer i the original size, or half-sized due to half the neurons being pruned? Relatedly, does the next layer downstream see a reduced-size input, and correspondingly have its own input dimension pruned?

\smalltitle{Comment 2}
\textit{While the writing is mostly understandable with few typos, I still may not understand how the technique works. If layer i is pruned, and the remaining filters share its duties, is the output of layer i the original size, or half-sized due to half the neurons being pruned? Relatedly, does the next layer downstream see a reduced-size input, and correspondingly have its own input dimension pruned?}

\smalltitle{Response 2}
The reviewer's understanding is indeed correct. If half of filters in layer $i$ are pruned, the output of layer $i$ is half-sized. This leads to the reduction of the number of input channels in layer $(i+1)$, what the reviewer calls the input dimension of the next layer. More specifically, if $j$-th filter of $\ell$-th layer is pruned, its corresponding channel of filters in $(\ell+1)$-th layer is consequently removed. However, it does not imply that the output size of $(\ell+1)$-th layer is also reduced, but its value is \textit{damaged} by the loss of $j$-th input channel.

In this version, we have added the following description to the caption of Figure \ref{fig:framework}:
$s, s',$ and $s^*$ are the coefficients that quantify how much each preserved filter should carry the information of the pruned filter.

We have double-checked the paper and revised all the typos therein as well.


\smalltitle{Comment 3}
\textit{You can always show top-1 or top-5 accuracy on a data set, but in the absence of such a data set, how will the deployer know when to stop pruning? There's a big accuracy gap between 10\% and 20\% pruning on the ImageNet results.}

\smalltitle{Response 3}
First of all, if there is no available data, we have no choice but to compress the target network in a data-free manner anyway, which is equally applied to both LBYL and NM. A possible way to determine when to stop pruning is to keep track of how the values of our two data-free error terms (i.e., RE and BE) are changing. As shown in Figure \ref{fig:error_components}, we can roughly guess how good the final performance would be by observing both RE and BE, which strongly contribute the reconstruction error. 

Also, our method can still be useful when we are given a target model size yet the final accuracy is not the most critical factor (e.g., recommendation app running in mobile devices).

\smalltitle{Comment 4}
\textit{This technique also seems like it would be useful as a pre-processing step before performing fine-tuning, potentially encouraging accuracy recovery or reducing the amount of fine-tuning required.}

\smalltitle{Response 4}
We agree with the reviewer that our method can also be seen as a preprocessing step before fine-tuning. As shown in Table \ref{tab:finetune_scratch} and Figure \ref{fig:Fine tuning and From Scratch}, we found that LBYL is indeed effective for fast convergence during the fine-tuning phase. 





% As you said, the accuracy of restored model decreases dramatically as pruning ratio increases. If we have a table of restored model's performances according to pruning ratio in experimental setting and the situation where our method is applied is similar with the experimental setting, the performance can be guessed through this table.

% But, when this is not the case, we suggest a naive solution to know when to stop pruning. A naive solution is to employ random noisy images(e.g., gaussian random samples) and then measure weighted average reconstruction error(WARE) between original model and pruned model. Increasing the pruning ratio and Checking the WARE, we may be able to avoid drastic loss. but this is just a rough method.

% On the other hand, our proposed methods can be used practically when users need to compress the original model and performance loss is relatively not critical.(e.g., recommendation system) For example, Choosing whether to update or not the smartphone is relatively robust to poor performance of model.


%--> As you said, it is true that accuracy of restored model in pruning ratio 30$\%$ is dropped with large margin compared to original model. Therefore we suggest a naive solution to stop whether prune more or not without using any data. A naive solution is to employ random images and then measure weighted average reconstruction error(WARE) between pre-trained model and pruned model. Based on WARE, we can choose whether to prune more or not.

%our proposed methods can practically be used when users need to compress the pre-trained model without considering performance such as recommendation system. for example, choosing whether to update or not does smartphone not affects smartphone's performance much because our method can correctly increase the performance after pruning. 




%%% Q4) Figure 1 has elements labeled 's' - these should be explained in the caption.

% Thanks for your reminder. In figure 1, $s_{i}$s mean coefficients by which a pruned filter is approximated using remained filters in l-th layer. and this is same with the coefficients by which a pruned channel is approximated using remained channels after CONV.

% Similarly, $s^{'}_{i}$s and $s^{*}_{i}$s are the coefficients by which a pruned channel is approximated using remained channels after BN and ReLU, respectively.




% \begin{table}[]
% \centering
% \normalsize
% \begin{tabular}{c||c|c|c|c} \Xhline{2\arrayrulewidth}
% Pruning ratio& OURS& NM& Prune & From Scratch (80epochs) \\ \Xhline{2\arrayrulewidth}
% 10 \% & \textbf{78.3}   & 77.57  & 77.67  & 48.22 (72.07)\\\hline
% 20 \% & \textbf{77.22}  &  75.62  &  75.4   & 47.85 (72.01)\\\hline
% 30 \% & \textbf{75.99}  & 73.03  &  73.18  & 46.7 (72.24)\\\hline
% 40 \% & \textbf{74.13}  & 69.71  &  70.12  & 46.53 (72.88)\\\hline
% 50 \% & \textbf{71.15}  & 65.03  &  65.72  & 44 (69.33)\\\Xhline{2\arrayrulewidth}
% \end{tabular}%
% \vspace{2mm}
% \caption{Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion. We fine-tune pruned and restored models for 20 epochs to compare methods after fine-tuning, where we use a Nesterov SGD optimizer with 0.9 momentum and the initial learning rate to 0.00001 divided by 10 at 5, 10 and 15 epochs. In case of from scratch, we train the randomly initialized model for 20 epochs where we use a Nesterov SGD optimizer with 0.9 momentum and the initial learning rate to 0.1}
% \label{tab:params:Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion}
% \end{table}




% show the comparison between our method and other data-free approaches that uses synthetic data for fine-tuning. Alternatively, we provide the comparison result between NM and our method LBYL after fine-tuning. the result is shown below. Table \ref{tab:param:ResNet50-CIFAR100 using l2-norm} presents that 





% You mentioned about "conserving synaptic flow"[27], but as far as I know, that method is introduced for weight pruning. It is possible to prune convolutional filters using weight pruning methods but pruning filters with weight pruning can't guarantee performance of compressed model because many kinds of weight pruning methods rely on fine-tuning. On the contrary, filter pruning methods try to reduce the fine-tuning as mentioned in related works in our paper. Therefore as mentioned in our paper, we focused on the filter pruning not weight pruning. 

% However, I think it will be a valuable study that uses fine-tuning via synthetic data generated by pre-trained generating models although it may require a lot of computation time as you mentioned. and If that method is applicable in filter pruning, our second sentence "since we cannot make appropriate changes in the remaining filters by fine tuning" should be changed as you mentioned.










%--> Thank for your guidance, In figure 1, $s_{i}$ means coefficient considering the linearity between preserved filters and the pruned filter and $s^{'}_{i}$ means coefficient considering both linearity and a batch normalization layer and $s^{*}_{i}$ means optimized scales considering both linearity and layers such as batch normalization and activation layer.

% \smalltitle{Q5}
% %%% Q5) Typos noticed

% Thanks for reminder. We will correct all typo you said in the final CRC version. 




% \begin{table}[]
% \centering
% \normalsize
% \begin{tabular}{c||c|c|c} \Xhline{2\arrayrulewidth}
% Pruning ratio& OURS& NM& Prune \\ \Xhline{2\arrayrulewidth}
% 10 \% & \textbf{78.14}   & 77.28  & 75.14  \\\hline
% 20 \% & \textbf{76.15}  &  72.73  &  63.39 \\\hline
% 30 \% & \textbf{73.29}  & 64.47  &  39.96  \\\hline
% 40 \% & \textbf{65.21}  & 46.4  &  15.32  \\\hline
% 50 \% & \textbf{52.61}  & 25.98  &  5.22  \\\Xhline{2\arrayrulewidth}
% \end{tabular}%
% \vspace{2mm}
% \caption{Recovery results of ResNet-50 on CIFAR-100 using L2-norm criterion}
% \label{tab:param:ResNet50-CIFAR100 using l2-norm}
% % \end{table}
% % \begin{table}[]
% \centering
% \normalsize
% \begin{tabular}{c||c|c|c|c} \Xhline{2\arrayrulewidth}
% Pruning ratio& OURS& NM& Prune & From Scratch (80epochs) \\ \Xhline{2\arrayrulewidth}
% 10 \% & \textbf{78.3}   & 77.57  & 77.67  & 48.22 (72.07)\\\hline
% 20 \% & \textbf{77.22}  &  75.62  &  75.4   & 47.85 (72.01)\\\hline
% 30 \% & \textbf{75.99}  & 73.03  &  73.18  & 46.7 (72.24)\\\hline
% 40 \% & \textbf{74.13}  & 69.71  &  70.12  & 46.53 (72.88)\\\hline
% 50 \% & \textbf{71.15}  & 65.03  &  65.72  & 44 (69.33)\\\Xhline{2\arrayrulewidth}
% \end{tabular}%
% \vspace{2mm}
% \caption{Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion. We fine-tune pruned and restored models for 20 epochs to compare methods after fine-tuning, where we use a Nesterov SGD optimizer with 0.9 momentum and the initial learning rate to 0.00001 divided by 10 at 5, 10 and 15 epochs. In case of from scratch, we train the randomly initialized model for 20 epochs where we use a Nesterov SGD optimizer with 0.9 momentum and the initial learning rate to 0.1}
% \label{tab:params:Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion}
% \end{table}

\subsection*{Reviewer AsvP}

% Thank you for the positive feedback and insightful comments that we have not thought about.

\smalltitle{Comment 1}
\textit{Would like to see analysis on how merged filters are changed to accommodate the information from pruned filters. How much information in the un-pruned kernel is lost as a result of the process? Does classic kernel behavior in terms of learning specific features hold after the kernel merging process?}

\smalltitle{Response 1}
Even though it is not trivial to quantify how much information in the preserved filter is lost as a result of the restoration process, we can claim that such a side effect is not much in LBYL, compared to NM. This is because LBYL minimizes the amount of those changes in remaining filters by making as many filters as possible to participate in the restoration process. On the other hand, NM forces each pruned filter to deliver its information to only one remaining filter, which can dramatically change the role of the remaining filter. As shown the table below, the average and maximum of absolute scaling factors (i.e., coefficients) of LBYL are much smaller than those of NM. More specifically, each un-pruned filter in LBYL is multiplied by only 0.00005 on the average, and consequently the information loss of the filter cannot be significant.
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c||c|c}\Xhline{2\arrayrulewidth}
Statistic& LBYL & NM \\ \Xhline{2\arrayrulewidth}
Mean & 0.00005 & 0.00045 \\ \hline
Max & 0.03977 & 0.34971 \\ \hline
Min & 0 & 0 \\ \hline
\end{tabular}%
\label{cov:tab:scale}
\vspace{2mm}
\caption{Comparison on absolute scale coefficients between LBYL and NM}
\end{table}



\smalltitle{Comment 2}
\textit{One limitation of this method is that it looks at each layer individually when recovering pruned kernel information -- it might be interesting to see if this method could not be generalized for compatible cross-layer information recovery.}

\smalltitle{Response 2} 
Although our strategy is to minimize the layer-wise output error in this paper, it would be a promising future work to incorporate cross-layer information as well to further optimize the restoration process.



%that the large scales can lead to distortion of remained filter's property.


%--> Original property on remained filters is changed to capture features that the pruned filter captured. However, the amount of changes in remained filters is very small than NM because we assume linearity between pruned filter and preserved filters. That means our method give a appropriate information on pruned filter to the remained filters compared to NM that give a scale based on norm ratio between pruned and remained filter. In our github, we will show that scale on pruned filter is very small than NM that the large scales can lead to distortion of remained filter's property.


% \begin{figure}[!htbp]
% \centering
%   \includegraphics[width=14cm]{Figure_OURS}
%   \hfil
% \caption{OURS scale}
% \label{Figure_OURS}
% \end{figure} 

% \begin{figure}[!htbp]
% \centering
%   \includegraphics[width=14cm]{Figure_NM}
%   \hfil
% \caption{NM scale}
% \label{Figure_NM}
% \end{figure} 



\subsection*{Reviewer VcLn }

\smalltitle{Comment 1}
\textit{Understanding the entire idea took me a long time due to the constant switching between layers, notation (A vs Z) etc ... . I think this can be done in a much cleaner way.}

\smalltitle{Response 1}
We would like to point out that most reviewers other than this one commonly said our manuscript is well written and easy to understand.

Having said that, we have provided the table of notations frequently used throughout the paper in Appendix, which would help to understand how our method works. We have attached our notations in Figure 1 as well in order to clarify what each notation actually means in Figure \ref{fig:framework}. For example, $\mathbf{Z}^{(\ell)}$ are illustrated by blue squares, and $\mathbf{A}^{(\ell)}$ are represented by green squares in Figure 1.



\smalltitle{Comment 2}
\textit{While the experiments show it works better than a method based on a similar idea, it is not clear to me whether the approach works any better than training a smaller network to start with. (in essence training a smaller model from scratch). It would also be interesting to see how it compares against fine-tuning, or whether this approach can benefit from fine tuning.}

\smalltitle{Response 2}
Although our method is motivated by a data-free scenario and therefore is compared to another data-free pruning method, we totally agree with the reviewer that it is essential to test whether our method is also effective when the data becomes available later on. Therefore, we additionally present new experimental results in Table \ref{tab:finetune_scratch} on the final accuracy of each pruned or restored model after fine-tuning along with that of the same-sized architecture trained from scratch. In all the cases, our LBYL method outperforms the competitors particularly when the pruning ratio increases. In addition, as shown in Figure \ref{fig:Fine tuning and From Scratch}, LBYL shows the fastest convergence speed during the fine-tuning process. Both of these observations justify the fact that our LBYL method is useful in practice even when the data is available.


% Our approach is essentially based on data-free assumption. so our method may have benefit compared to the smaller network that requires fine-tuning in the sense that our method can be used when the training data is not available or the training data is available but the computing resource is constrained.(e.g., mobile device...)

% Even when the training data and fine-tuning process are available, our method can have benefit compared to the smaller network which is trained from scratch in the sense that the restored model converge much more faster than From Scratch model shown in the table \ref{tab:params:Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion}.

% Our method can be used when the model compression is needed but training data is not available or heavy computation is burdensome. But as reviewer 2 mentioned, you may wonder when to stop the pruning in real world because the accuracy of restored model decreases dramatically as pruning ratio increases. In this case, 
% If we have a table of restored model's performances according to pruning ratio in experimental setting and the situation where our method is applied is similar with the experimental setting, the performance can be guessed through this table.

% But, when this is not the case, we suggest a naive solution to know when to stop pruning. A naive solution is to employ random noisy images(e.g., gaussian random samples) and then measure weighted average reconstruction error(WARE) between original model and pruned model. Increasing the pruning ratio and checking the WARE, we may be able to avoid drastic loss. but this is just a rough method.

% On the other hand, our proposed methods can be used practically when users need to compress the original model and performance loss is relatively not critical.(e.g., recommendation system) For example, Choosing whether to update or not the smartphone is relatively robust to poor performance of model.

% Or, As reviewer 2 mentioned and shown in the table \ref{tab:params:Fine-tuned results of ResNet-50 on CIFAR100 using L2-norm criterion}, our method can also be used as the pre-processing step before performing fine-tuning. We found the converge time is reduced by comparison with NM and From Scratch.

% \kim{continued}
%--> Our method shows better performance compared to randomly initialized model with same fine-tuning epochs. However, if we train predefined small model from scratch during a lot of epochs, result will show similar performance regardless of restored methods because a few works[1,2] show that randomly initialized small models reaches the similar performance regardless of pruning methods. 
%Actually, performing the fine-tuning process assumes that there are sufficient data and computation such as GPU. Unfortunately, in practice, these assumptions are not always satisfactory. Therefore, our proposed method can be used in the following situations. Our method can be used in resource-constrained devices such as edge device and also pre-processing step before fine-tuning as the reviewer3 said too.

%[1] rethinking of network pruning
%[2] pruning from scratch 







==> backup/experiments.tex <==
\section{Experiments} \label{sec:experiments}
In this section, we empirically validate the performance and effectiveness of our proposed LBYL method, compared to a one-to-one compensation method, called \textit{Neuron Merging} (\textit{NM})  \cite{NM} as well as a baseline called \textit{Prune} that does not perform any recovery process after pruning. For a fair comparison, we exploit the code provided by the authors of \cite{NM} and then implement our proposed method using PyTorch \cite{PyTorch}. LBYL uses two hyperparameters, namely $\lambda_1$ and $\lambda_2$, that adjust the weights of loss terms BE and AE, respectively. The details of hyperparameter settings are presented in Appendix. Also, our implementation is available at our anonymized github.\footnote{https://github.com/anonymous}

\smalltitle{Pruning criteria and ratio}
We evaluate LBYL using the following four data-independent pruning criteria: L1-norm \cite{PFEC}, L2-norm \cite{Soft}, L2-GM \cite{FPGM}, and lastly even random. We prune only convolution filters in CNNs, and hence the pruning ratio is the ratio of pruned filters for each convolution layer.
% Random pruning is intended to show the robustness of each method when a norm-based criterion is not used.

\subsection{Experiments using CIFAR-10 and CIFAR-100}
\smalltitle{Dataset and pretrained model} 
The CIFAR-10 dataset \cite{krizhevsky2009learning} consists 60K images of 10 different classes, where each class includes 5K training images along with 1K validation images and the size of every image is 32 × 32. CIFAR-100 \cite{krizhevsky2009learning} also include 60K images for 100 different classes, where 500 training images along with 100 validation images are included for each class. We test VGG-16 \cite{VGG} for CIFAR-10 and ResNet-50 \cite{ResNet} for CIFAR-100, and present the result of CIFAR-100 only in Appendix as 
their experimental results of CIFAR-10 and CIFAR-100 show the similar trend.


% In case of CIFAR-100, we evaluate the our proposed method using the ResNet-50 \cite{ResNet}. To train the ResNet-50, we exploit SGD with Nesterov momentum of 0.9. the initial learning rate is 0.1 and it is divided by 5 at 60, 120, 160 epochs. the weight decay is set to 5e-4, the train epochs is 200 with batch size 128. 

\smalltitle{Results}
We first prune VGG-16 on CIFAR-10, which is a representative single-branched CNN, using the layer-by-layer pruning scheme with four different criteria, and then update the remaining filters in each layer to restore the pruned VGG-16. As shown in Table \ref{tab:VGG16-CIFAR10}, our LBYL method achieves up to 6.16\% higher average accuracy than NM \cite{NM}. In particular, LBYL outperforms NM with clear margins when the pruning ratio increases. This is probably because NM might have trouble finding a filter sufficiently close to each pruned filter with less remaining filters due to a higher pruning ratio.

\subsection{Experiments using ImageNet (ILSVRC2012)}

\smalltitle{Dataset and pre-trained model} 
The ImageNet dataset \cite{deng2009imagenet} contains 1,000 classes and consist of 1.28M training images and 50K validation images of size 256 $\times$ 256. For ImageNet, we use pretrained ResNet-34 and ResNet-101, both of which are released by PyTorch\footnote{https://pytorch.org/vision/stable/models.html}. ResNet-34 and ResNet-101 respectively represent two different types of the ResNet architecture, namely the one consisting of basic blocks and the other one consisting of bottleneck blocks.

\smalltitle{Results}
To prune a ResNet architecture, we exploit the common strategy to remove each residual block, that is, pruning the first two convolutional layers and not changing the output dimension of the block. Tables \ref{tab:ResNet34-ImageNet} and \ref{tab:ResNet101-ImageNet} present the experimental results using ResNet-34 and ResNet-101 on ImageNet. Through the results, LBYL can still recover the damaged filters to a satisfactory extent.

\begin{figure*}[t]
	\centering 
	% vanilla WA
	\includegraphics[height=2mm]{./figure/error_key.pdf} \\
    \subfloat[\label{fig:expcos_:a}{RE} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/LBYL_figure_3_RE.pdf}\hspace{2mm}}
    %CTL + WA
    \subfloat[\label{fig:expcos_:b}{BE} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/LBYL_figure_3_BE.pdf}\hspace{2mm}}
    % ART+WA
    \subfloat[\label{fig:expcos_:c}{WARE} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/LBYL_figure_3_WARE.pdf}\hspace{2mm}}
    \caption{Comparison on the three error components with NM \cite{NM}, where each $m$\_$n\_k$ in the x-axis represents the $k$-th conv module in the $n$-th block at the $m$-th layer in ResNet-50}
	\label{fig:error_components}
	\vspace{-2mm}
\end{figure*}


\subsection{Effectiveness in terms of Reconstruction}
In order to see the effectiveness of our loss function on minimizing the reconstruction error, we compute the values of three error components, namely RE, BE, and AE, using ResNet-50 \cite{ResNet} on CIFAR-100 \cite{krizhevsky2009learning}. Both RE and BE can be measured without any inference with sample data, but AE is not easy to obtain. Therefore, we adopt the \textit{weighted average reconstruction error} (\textit{WARE}) introduced in \cite{NISP}, which shows the difference between the layer-wise output of the original model and that of the pruned model.

Figure \ref{fig:error_components} shows layer-wise values for each of RE, BE and WARE. It is clearly observed that NM returns a very rough approximation in terms of RE, compared to our LBYL method. This is due to the fact that NM uses only a single remaining filter to receive the missing information of a pruned filter, and consequently the final output can be quite far from the original.
In both BE and WARE, there is not much difference between LBYL and NM in early layers, but we can observe that the error values of NM become higher in the end. Thus, even though NM might be effective to reconstruct the original output in some layers, it shows unstable performance depending on the existence of similar filters and finally ends up with less accurate approximation. On the other hand, our LBYL method is less varied across layers and managed to keep the error values lower in the end for all three metrics.

\begin{table*}[t]
\centering
\normalsize
\begin{tabular}{c||c|c|c|c|c} \Xhline{2\arrayrulewidth}
Pruning Ratio& Ours & NM& Coreset&Prune & From Scratch (80 epochs) \\ \Xhline{2\arrayrulewidth}
10 \% & \textbf{78.3}   & 77.57  &76.55 & 77.67  & 48.22 (72.07)\\\hline
20 \% & \textbf{77.22}  &  75.62  &74.39&  75.4   & 47.85 (72.01)\\\hline 
30 \% & \textbf{75.99}  & 73.03  &71.88&  73.18  & 46.7 (72.24)\\\hline
40 \% & \textbf{74.13}  & 69.71  &68.14&  70.12  & 46.53 (72.88)\\\hline
50 \% & \textbf{71.15}  & 65.03  &62.88&  65.72  & 44 (69.33)\\\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{Fine-tuned or trained accuracies of ResNet-50 on CIFAR-100 using L2-norm criterion, where we fine-tune each model for 20 epochs and train the same-sized small architecture for 20 epochs (80 epochs)}
\label{tab:finetune_scratch}
\vspace{3mm}
\end{table*}

\begin{figure*}[t]
	\centering 
	\includegraphics[height=2mm]{./figure/f4_KEY.pdf} \\
    \subfloat[\label{fig:expcos:a}{10 \%} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/f4_10.pdf}\hspace{2mm}}
    \subfloat[\label{fig:expcos:b}{30 \%} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/f4_30.pdf}\hspace{2mm}}
    \subfloat[\label{fig:expcos:c}{50 \%} ]{\hspace{0mm}\includegraphics[width=0.5\columnwidth]{./figure/f4_50.pdf}\hspace{2mm}}
    \caption{Comparison on learning curves of fine-tuning restored networks for 20 epochs and that of training the same-sized small architecture from scratch for 80 epochs at different pruning ratios}
	\label{fig:Fine tuning and From Scratch}
 	\vspace{-2mm}
\end{figure*}

\smalltitle{Performance estimation}
One can be curious about how to set the appropriate pruning ratio for a particular target size and accuracy if we cannot use any data during the entire pruning and recovery process. Our two data-free error terms (i.e., RE and BE) can also be utilized in such a case. As shown in Figure \ref{fig:error_components}, we can roughly estimate WARE, which is also highly relevant to the final performance, by combining RE and BE.

\subsection{Practical Test with Data and Fine-Tuning}
Although this paper focuses on the problem of restoring pruned networks without data, we additionally test whether our method is also effective when the data becomes available later on. Table \ref{tab:finetune_scratch} shows the experimental results on the final accuracy of each pruned or restored model after fine-tuning along with that of the same-sized architecture trained from scratch. In this experiment, we take the data-independent pruning method based on coreset \cite{CoreSet_ICLR} as another competitor, which also introduces a training-free recovery method as an intermediate process. We fine-tune and train each model for 20 epochs, and also show the resulting accuracy of the model trained from scratch after 80 epochs. In all cases, our LBYL method outperforms its competitors particularly when the pruning ratio increases. Our best guess on why NM becomes eventually worse than just pruned model is that NM can choose a dissimilar filter to recover each pruned one in some layers, which makes it hard for fine-tuning to improve the performance.
\textit{Coreset} \cite{CoreSet_ICLR} shows the lowest accuracy probably because it does not focus on training-free recovery and hence 20 epochs of fine-tuning is not sufficient. As shown in Figure \ref{fig:Fine tuning and From Scratch}, LBYL shows the fastest convergence speed during the fine-tuning process. Both of these observations justify the fact that our LBYL method is practically useful when the data is available. 

% \TODO{Add Coreset method in Table 4 and Figure 4. Change Table 4 to have arrows}
% We also compare the Coreset\cite{CoreSet_ICLR} from the standpoint that update the weights of pruned model as shown in the Figure 4. \ref{fig:Fine tuning and From Scratch},where we present average accuracy of the Coreset \cite{CoreSet_ICLR}. The reason why Coreset \cite{CoreSet_ICLR} shows the lowest accuracy is that Coreset \cite{CoreSet_ICLR} do not focus on directly minimizing the output between pruned model and pre-trained model but concentrate on proving the error bound for output between pruned model and pre-trained model, which results in insignificant compensation.


% We measure the reconstruction errors (RE) generated by pruned filter and preserved filter and batch normalization error, which can minimize the reconstruction error, where both RE and BE are taken l2-norm to show magnitude. LBLY optimize the scale parameter to minimize the both RE and BE. Therefore, Our method has a lower error compared to NM \cite{NM} as shown in Figure \ref{fig:error_components}.Moreover we also calculate the Weighted Average Reconstruction Error (WARE) used in \cite{NISP} to measure the difference between original model and recovered model. From Figure \ref{fig:error_components}, LBLY tends to increase more gently in last layer because our method is based on the number of filters,leads to small reconstruction error than NM with considering relationship between pruned filter and only one remained filter.\cite{NM} 




% \begin{figure*}[t]
% 	\centering
% 	{
%     \includegraphics[height=2.5mm]{./figure/key.pdf}	\vspace{1mm}

% 		\begin{tabular}{cccc}
% 			\subfigure[\label{fig:cifar:a}2 tasks] {\includegraphics[height=32mm]{./figure/LBYL_figure_2}}  & 
% 		\end{tabular}
% 		\vspace{-3mm}
% 		\caption{Comparison on the accuracy for each incremental task using CIFAR-100}
% 		\label{fig:cifar}
% 	}

% \end{figure*}



% \begin{table}[]
% {\scriptsize

% \begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
% \multicolumn{13}{c}{\textbf{ResNet-50 (Acc. 73.27) }}
% \\ \Xhline{2\arrayrulewidth} %\hline
% Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
% Pruning Ratio& Ours& NM& prune& Ours& NM& prune& Ours& NM& prune& Ours& NM& prune
% \\ \Xhline{2\arrayrulewidth}
% 10\%& \textbf{77.31}& 77.28& 75.14& \textbf{77.20}& 76.92& 74.49& \textbf{77.55}& 77.21& 75.07& \textbf{76.14}& 72.18& 58.12\\ \hline
% 20\%& \textbf{73.24}& 72.73& 63.39& \textbf{73.46}& 72.32& 63.54& \textbf{73.20}& 72.24& 61.84& \textbf{70.59}& 59.62& 26.87\\ \hline
% 30\%& \textbf{66.63}& 64.47& 39.96& \textbf{67.07}& 64.01& 39.01& \textbf{66.30}& 63.07& 35.77& \textbf{62.22}& 39.45& 2.59 \\ \hline
% 40\%& \textbf{51.46}& 46.40& 15.32& \textbf{50.60}& 46.17& 13.14& \textbf{48.07}& 45.98& 12.59& \textbf{41.90}& 17.77& 3.08 \\ \hline
% 50\%& \textbf{28.74}& 25.98& 5.22& \textbf{30.66}& 23.44& 4.32& \textbf{22.06}& 21.98& 4.25& \textbf{22.07}& 7.17 & 2.20 \\ \Xhline{2\arrayrulewidth}
% Average Acc.& \textbf{59.48}& 57.37& 39.81& \textbf{59.80}& 56.57& 38.90& \textbf{57.44}& 56.10& 37.90& \textbf{54.58}& 39.24& 18.57 \\ 
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% }
% \caption{Compenssation results of ResNet-50 on CIFAR-100}
% \label{tab:ResNet50-CIFAR100}

% \end{table}

==> backup/intro.tex <==
\section{Introduction} \label{sec:intro}


% 1. Network pruning has been extensively studied in neural networks. 
%    its simplicity, reasonable performance
Network pruning is one of the most well-studied model compression technique for an overparameterized deep neural network, and many different pruning strategies have been introduced with the goal of removing less important parameters from the original network. Due to its simplicity in terms of both implementation and methodology, network pruning has been pretty popular to the point that it is provided as a default model compression function in standard libraries like TensorFlow\footnote{https://www.tensorflow.org/model\_optimization/guide/pruning} and PyTorch\footnote{https://pytorch.org/tutorials/intermediate/pruning\_tutorial.html}, along with the other compression options such as quantization \cite{Coreset}. Among two major pruning schemes, namely weight pruning (\textit{a.k.a.} unstructured pruning) \cite{Lottery,Songhan,SNIP,Synaptic,OptimalPruning} and filter pruning (\textit{a.k.a.} structured pruning), filter pruning is more actively studied \cite{FPGM,Lasso,EagleEye,Rethinking,Thinet,DCP} due to its strength of reducing the actual computation cost at inference time without any special hardware support. In this sense, this paper also focuses on filter pruning.

% \cite{GlobalRanking,AMC,FPGM,Lasso,EagleEye,Dynamic,Rethinking,CURL,Thinet,Importance,Reborn,NISP,DCP}

% To deploy large neural networks to resource-constrained mobile and edge devices, network pruning has been extensively studied due to implementation-friendly and compatibility with other network compression methods \cite{DBLP:conf/eccv/HeLLWLH18, DBLP:conf/cvpr/HeLWHY19} In general, Network pruning methods is fall in to two parts : Weight pruning(Unstructured pruning) and Filter pruning(Structured pruning). Weight pruning encourage parameters of neural network sparse during the training process or post process. As a result, Number of parameters in neural networks can be reduced parameters more than 90\% \cite{NIPS2015_ae0eb3ee} However, Because of irregular sparse connections Weight pruning need a special software to accelerate inference speed. On the other hand, Filter pruning removes unimportant filter so can accelerate inference time without special software. 

% 2. Most of pruning methods require an expensive training process
%    e.g., iterative training(on the fly), fine-tuning(post process)
% 3. A long fine-tuning eventually determines the final accuracy 
%    That is why existing pruning methods use only a few 2-3 epochs of fine-tuning

Even though many of the existing pruning methods achieve a reasonable level of the final accuracy, it mostly comes at an expensive cost of retraining at the end of (or in the middle of) pruning phase. For instance, iterative filter pruning methods \cite{Soft,FPGM,Dynamic} alternately perform pruning phase and retraining phase so that the original model can gradually be compressed as well as recovered over the hundreds of epochs. Another major approach is to conduct \textit{one-shot pruning} and then fine-tune the pruned network for its original performance to be recovered \cite{EagleEye,CURL,Importance,NISP,DCP}. In most one-shot pruning techniques, the fine-tuning phase does not take longer than a few dozens of epochs probably because there is no big difference in accuracy among pruning criteria beyond that point. In fact, it is reported that even a randomly pruned network can reach comparable performance after fine-tuning of hundreds or thousands of epochs \cite{Rethinking}. Thus, if we do not have any constraints on time, computing resources, or training data for a long fine-tuning process, one-shot pruning methods would be less meaningful.

% 4. Therefore, they obviously need a quiet complete set of training data
%    (mostly exactly the same as the original train set) or need to collect as 
%    many samples as the origin
% 5. However, in practice, the train data is neither available nor easy to collect
% 6. Therefore, a few recent works have tried to address above with using much small data ( still need data, train process anyway)
% 7. Meanwhile, a few works commonly employ the neuron similarity in order to 
%    reduce the bad effect of pruning Thus, a similar neuron can be replaced
%    limitations of NM, 
%    1) it is based on strong naive assumption, which is not the case in NNs.
%    2) a single neuron can't compensate due to the error term we found yet not discussed

\begin{figure*}[t!]
   \centering 
    \includegraphics[width=1.9\columnwidth]{./figure/LBYL_figures.pdf}
   \caption{The conceptual overview of our LBYL method, showing how the original output resulting from a pruned filter at $\ell$-th layer, that is, the output of $(\ell+1)$-th convolutional layer, can be recovered by all the other preserved filters at the same layer (\textit{i.e.}, $\ell$-th layer) through convolution, batch normalization, and activation function (\textit{i.e.}, ReLU), where $s, s',$ and $s^*$ are the coefficients that quantify how much each preserved filter should carry the information of the pruned filter.}
   \label{fig:framework}
\end{figure*}


Somewhat fortunately, however, this is not the case in many practical scenarios where we cannot access or re-collect the original data due to its large volume or some commercial issues \cite{DBLP:conf/eccv/MahajanGRHPLBM18}. Even though some recent works \cite{CURL,Reborn} attempt to use only a small amount of training data instead, but they still suffer from a time-consuming process of fine-tuning to achieve satisfactory performance. Furthermore, it would not be always possible to collect samples in the same domain as the original data, regardless of whether they are labeled or not. Only quite a few works \cite{NM,Data-free} have been introduced to recover pruned networks without using any data and fine-tuning process. Their common approach is what we call \textit{one-to-one compensation}, where the most similar unpruned neuron takes the role of a pruned neuron. This approach is based on the strong assumption that there exists such a neuron quite similar to each one being pruned at the same layer. Not surprisingly, this assumption cannot be guaranteed in deep neural networks, which is even reported in the result of \cite{NM} showing that the pairwise similarity on filters gets extremely low particularly in deeper layers. In addition, according to our theoretical analysis on the reconstruction error, a single neuron can only lead to a very rough approximation to the original output even if the neuron is similar enough to its pruned counterpart.



% However, they obviously still require a quiet complete set of train data to recover a original network performance because as presented in \cite{DBLP:conf/aaai/TangYXH0SXZ20}, compressed network hard to reach original performance with a few data. Moreover, in many practice application, the train data is neither accessible nor easy to collect due to commercial profits \cite{DBLP:conf/eccv/MahajanGRHPLBM18}. There are two trials to fine-tune the pruned model with small data using knowledge distilation \cite{Knowledge_Distilation} and extra trainable parameters. \cite{CURL} propose fine-tuning method based on knowledge distillation using a few data. More specifically, they employ soft target of the pre-trained model regarding the small data to fine-tuning the pruned model. \cite{Reborn} appends the additional convolution modules due to hardness to fine-tune using the small data and then retrain the extra modules with existing modules fixed. after fine-tuning on the supplementary modules with sparsity, the compressed model combines with additional convolution module and original modules to recover the original performance. However, they obviously exploit the small data to restore performance of original network.


% A few works \cite{NM, Data-free} commonly employ the neuron similarity in order to reduce catastrophic loss induced by removed filters without using any data and any fine-tuning process. They have a strong assumption that a filter can be replaced with a most similar filter but these assumption in neural networks have the limitations. It depends on that pruned filters have a single similar filter in neural networks. As presented in \cite{NM}, if the layer in networks become more deeper, the correlation between the filters in layer gradually decrease. Thus, preserved filter which is a most similar with removed filter isn't actually similar with pruned filter. That is, it turn out that a single similar filter can't significantly compensate. Moreover, they have ignored the error term we found yet not discussed in \cite{NM}.



% As shown above the pruned model, if filters in layer be pruned, the corresponding channels of filter in $i$+1-th layer are removed, which leads to loss of the feature maps in $i$+1-th layer. However, LBYL restores catastrophic loss pruned from filters in $i$-th layer by compensating the channels of filter $i$+1-th with a our assumption that compensation of pruned filter in $i$-th layer can be made with relationship between the pruned filter and preserved filters in $i$-th layer. The overall recovery process is as follow: first, we use a assumption that pruned filter in i-th layer is represented by multiple preserved filters on the same layer. Secondly, we can obtain the approximation scale to compensate pruned filter by extending the our assumption to normalization, activation layer, and convolution outputs (\textit{e.g.} feature maps in i+1 layer). Thirdly, before removing the channels of filters in $i$+1-th resulted from the pruned filter in $i$-th layer, they would be multipled by approximation scale and then add their weights to preserved filter in i+1 layer as shown in the last part above. Finally, we significantly recover the information loss induced by pruned filters in $i$-th layer


In this paper, we propose a theoretically more rigorous and robust method, called \textit{Leave Before You Leave} (\textit{LBYL}), to effectively compensate for pruned filters, which is also free of any data and fine-tuning. As depicted in Figure \ref{fig:framework}, we significantly relax the strong assumption by observing the fact that a pruned filter is better to be represented by a linear combination of as many preserved filters as possible than it is done by a single filter. We first mathematically analyze how the reconstruction error can be formulated between the original network and its pruned network, and thereby discover three components of the error. Based on our formulation, we provide a closed form solution that can minimize the reconstruction error to compensate for information loss caused by pruned filters, which does not need any training process at all. Through extensive experiments, we show that LBYL outperforms the existing one-to-one compensation scheme \cite{NM} regardless of pruning criterion. For instance, LBYL achieves at pruning ratio 30\% on the average 17.92\% higher accuracy than those of \cite{NM} for ResNet-101 \cite{ResNet} trained with ImageNet \cite{deng2009imagenet}.



% LBYL achieves at pruning ratio 40\% on average 3.53\% higher accuracy than \cite{NM} for ResNet-50 \cite{ResNet} on CIFAR-100 \cite{krizhevsky2009learning} and also in case of large dataset (i.e., ImageNet \cite{deng2009imagenet}), .



% using CIFAR \cite{krizhevsky2009learning} and ImageNet \cite{deng2009imagenet}








==> backup/method.tex <==
\section{Proposed Method of Restoring Pruned Filters} \label{sec:method}
In this section, we first theoretically examine how the reconstruction error of Eq. (\ref{eq:goal}) can be formulated in a way free of using data-dependent parameters. Based on this analysis, we present our train-free recovery method that has a closed form solution for minimizing the formulated reconstruction loss.

%is composed of with respect to our proposed methodology using multiple filters to approximate a pruned filter, so-called \textit{many-to-one}. Our approach is in fact a generalized version of the existing one-to-one compensation methods \cite{NM,Data-free}. Finally, we present our train-free recovery method that has a closed form solution for minimizing the formulated reconstruction error.

\subsection{Data-Independent Reconstruction Loss} \label{sec:method:a}
For brevity, we deal with a simple case of pruning only a single filter, which can trivially be extended to cover multiple filters. Without loss of generality, let the $j$-th filter of the $\ell$-th layer be pruned. 

\smalltitle{Leave Before You Leave (LBYL) assumption}
In order to transform Eq. (\ref{eq:goal}) to a data-free version, our proposed assumption is that each filter being pruned can \textit{leave} its pieces of information for the remaining ones by adding its corresponding pruned channel to each of the other channels in the next layer. Since the quantity of information depends on how much the pruned filter is related to a particular remaining filter, we need to multiply the pruned channel with a different value before addition. Based on this assumption, for a case of pruning only the $j$-th filter, the delivery matrix $\boldsymbol{\S^*} \in \mathbb{R}^{m \times (m-1)}$ is defined to be in the following form:
\begin{eqnarray}\begin{split}\label{eq:matrix}
\boldsymbol{\S^*}_{i,k} = 
  \begin{cases} 
   1 & \text{if } i = i'_k \\
   s_{i'_k} & \text{if } i = j \\
   0 & \text{otherwise}
  \end{cases}
  \end{split}
\end{eqnarray}
 $\text{s.t. } i, i'_k \in [1, m] \text{ and } k \in [1, m-1],$ where $s_{i'_k}$ is a scalar value that quantifies to what extent the $i'_k$-th filter is related to the $j$-th filter being pruned. Figure \ref{fig:matrix:b} shows an example of the delivery matrix for our LBYL method.


\smalltitle{Without BN and an activation function}
Starting with Eq. (\ref{eq:goal}), we first derive its data-free version without considering both a BN procedure and an activation function, and then make an extension for them. With the proposed form of the delivery matrix in Eq. (\ref{eq:matrix}) together with Eq. (\ref{eq:fmap_approx}), the $i$-th channel of $\mathbf{\hat{Z}}^{{(\ell+1)}}$ is now represented as:
\begin{equation}
{{\mathbf{\hat{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast (\mathbf{W}_{i,k}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j}^{(\ell+1)}).
\nonumber
\end{equation}
Then, the reconstruction error for the $i$-th channel of the feature map at the $(\ell+1)$-th layer can be derived as:
\begin{equation}
{\mathbf{Z}_{i}^{{(\ell+1)}}}-{\mathbf{\hat{Z}}_{i}^{{(\ell+1)}}}=(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\circledast \mathbf{W}_{i,j}^{(\ell+1)}.
\label{eq:eq5}
\end{equation}
By Eq. (\ref{eq:eq5}), we have the following form of the reconstruction error for the case of pruning the $j$-th filter at the $\ell$-th layer:
\begin{eqnarray}\begin{split}
\sum\limits_{{i} = 1}^{m^{\prime}}\|{\mathbf{Z}_{i}^{{(\ell+1)}}-\mathbf{\hat{Z}}_{i}^{{(\ell+1)}}}\|_1 ~~~~~~~~~~~~~~~~~\\ 
=\sum\limits_{{i} =  1}^{m^{\prime}}\|(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\circledast\mathbf{W}_{i,j}^{(\ell+1)}\|_1.
\end{split}
\label{eq:eq6}
\end{eqnarray}
Based on Eq. (\ref{eq:eq6}), we can reduce the problem of minimizing Eq. (\ref{eq:goal}) into the one of minimizing the following error term:
\begin{equation} \label{eq:goal2}
\|(\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)})\|_1,
\end{equation}
where we need to find scalars $s_{k}$'s such that ${ \mathbf{A}_{j}^{(\ell)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}}$.

Without considering BN and any activation function, we simply have $\mathbf{A}^{(\ell)} = \mathbf{Z}^{(\ell)}$, and consequently Eq. (\ref{eq:goal2}) can be represented as:
\begin{gather*}
    %  \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} \\
    % = \| (\mathbf{A}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(\ell)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times (\mathbf{A}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(\ell)} ) \|_{1} \nonumber \\
    % = 
     \| (\mathbf{A}^{(\ell-1)}  \circledast (\mathbf{W}_{j}^{(\ell)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(\ell)} ) \|_{1}.
\end{gather*}
Since $\mathbf{A}^{(\ell-1)}$ is data-dependent yet independent to pruned filters, it can be regarded as a constant factor of the reconstruction error that depends on which filters are pruned. Thus, it suffices to minimize the other part of the term, which we call \textit{Residual Error} (\textit{RE}) denoted by $\boldsymbol{\E}$ as the following definition:
\begin{definition} \label{def:re}
Given a pruned filter $\mathbf{W}_{j}^{(\ell)}$ at the $\ell$-th layer, the Residual Error (RE) is defined as:
$$
\boldsymbol{\E} = \mathbf{W}_{j}^{(\ell)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(\ell)}.
$$
\end{definition}
Note that $\boldsymbol{\E}$ can be minimized by using only the original network without any support from data.


% Since we cannot access $\mathbf{A}^{(\ell-1)}$ without data, the only thing we can do is minimizing the other part of the term. We call this error term \textit{Residual Error} (\textit{RE}) and denote it by $\boldsymbol{\E}$

\smalltitle{Considering batch normalization} 
We now incorporate a BN procedure in the process of minimizing Eq. (\ref{eq:goal2}). In this case, as we have $\mathbf{A}^{(\ell)} = \N(\mathbf{Z}^{(\ell)})$, Eq. (\ref{eq:goal2}) can be derived as Lemma \ref{lem:bn}.
\begin{lemma} \label{lem:bn}
If there is only batch normalization between a feature map and its activation map, the reconstruction error can be formulated as follows:
\begin{equation} \label{eq:bn}
\| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)} \circledast \boldsymbol{\E})} + \boldsymbol{\B}\|_{1},
\end{equation}
% \begin{equation} \label{eq:bn}
% \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)} \circledast \boldsymbol{\E})} +
% \frac{\gamma_{j}}{\sigma_{j}} 
% \{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j + \frac{\sigma_{j}}{\gamma_{j}}\beta_j\} \|_{1},
% \end{equation}
where $\boldsymbol{\B} = \frac{\gamma_{j}}{\sigma_{j}} 
 \{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j + \frac{\sigma_{j}}{\gamma_{j}}\beta_j\}$, $\mu$, $\gamma$, $\sigma$, and $\beta$ are batch normalization parameters.
\end{lemma}
\begin{proof}
See Appendix.
\end{proof}
Hereafter, the notation $\boldsymbol{\E}$ is a bit differently defined such that $s_k$ from Definition \ref{def:re} should be substituted with $s_k \frac{\sigma_j}{\gamma_j} \frac{\gamma_k}{\sigma_k}$ due to the BN procedure. We call the second term $\boldsymbol{\B}$ of Eq. (\ref{eq:bn}) Batch Normalization Error (BE).

\begin{definition}
Given a pruned filter $\mathbf{W}_{j}^{(\ell)}$ at the $\ell$-th layer, the Batch Normalization Error (BE) is defined as:
$$
\boldsymbol{\B} = \frac{\gamma_{j}}{\sigma_{j}} 
\{\sum\limits_{k = 1, k \neq j }^{m} s_{k}\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{k}}{\sigma_{k}} (\mu_{k} -  \frac{\sigma_{k}}{\gamma_{k}}\beta_k) - \mu_j  + \frac{\sigma_{j}}{\gamma_{j}}\beta_j \}.
$$
\end{definition}



% below Eq. (\ref{eq:eq9}).
% \begin{eqnarray} \begin{split}\label{eq:eq9}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \N (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}
% Eq. (\ref{eq:eq9}) is further derived and finally we can conclude to the following lemma:


\smalltitle{Considering activation function}
Lastly, we proceed our analysis to cover a general CNN architecture including both BN and the ReLU activation function. For an activation function $\F$, we now have $\mathbf{A}^{(\ell)} = \F(\N(\mathbf{Z}^{(\ell)}))$, and thereby Eq. (\ref{eq:goal2}) is derived to be the following theorem:
\begin{theorem} \label{thm:relu}
If there are both batch normalization and a ReLU function between a feature map and its activation map, the reconstruction error can be formulated as follows:
    \begin{equation} \label{eq:relu}
     \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{A}^{(\ell-1)}\circledast\boldsymbol{\E})}+ \boldsymbol{\B} + \boldsymbol{\R}\|_{1},
     \nonumber
     \end{equation}
     where $\boldsymbol{\R} = \sum\limits_{k=1, k \neq j}^{m} s_{k}  \min(0,\N(\mathbf{Z}_{k}^{(\ell)}))-\min(0,\N(\mathbf{Z}_{j}^{(\ell)}))$ represents the \textit{Activation Error} (\textit{AE}).
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

\smalltitle{Data-free loss function}
As concluded in Theorem \ref{thm:relu}, we discover the fact that the reconstruction error of Eq. (\ref{eq:goal}) can finally be decomposed into three different components, namely RE, BE, and AE. This brings us to formulate the following reconstruction loss that does not require any training data. 
\begin{equation}
     \mathcal{L}_{re} =  \|\boldsymbol{\E}\|_2^{2} + \lambda_1 \|\boldsymbol{\B}\|_2^{2} + \lambda_2 \|\mathbf{s}\|_{2}^{2},
\label{eq:loss}
\end{equation}
where $\mathbf{s} =  [s_{1}~...~s_{j-1}~s_{j+1}~...~s_{m}]$.

Unlike RE and BE, we cannot exactly control the AE term as $\mathbf{Z}^{(\ell)}$ can only be obtained by using the actual data. Therefore, we instead introduce a regularization term $\|\mathbf{s}\|_{2}^{2}$ for the purpose of mitigating the explosion of $\boldsymbol{\R}$, inspired by the fact that each error value of $\boldsymbol{\R}$ is proportional to $s_k$. Furthermore, since our intention is to participate as many preserved filters as possible in restoring a pruned filter, it would be better for the $s_k$ values to be more uniformly distributed. Both purposes can be fulfilled by this L2-based regularization term. 

\begin{algorithm}[t]
  \small
  \caption{LBYL method}
  \label{alg:Recovery}
  \KwIn{$\mathbf{\Theta}$ = $[\mathbf{W}^{{(1)}}$, .... ,$\mathbf{W}^{{(L)}}] := $ Original model}
  \KwOut{$\hat{\mathbf{\Theta}}$ = $[{\mathbf{\hat{W}}}^{{(1)}}$, .... ,$\mathbf{\hat{W}}^{(L)}] : = $ Pruned \& restored model}
   
  \For{each layer $\ell \in [1, L]$ that has been pruned}%$\in$ $\mathbb{R}^{n_{l} \times k \times k}$   $\mathbf{in}$ $\mathbf{W}^{(\ell)}$}
    {
    ${\boldsymbol{\S}}^{(\ell)} \leftarrow $ a zero-valued matrix
    
    \For{each filter $\mathbf{W}_i^{(\ell)}$ s.t. $i$ $\in$ $[1,m]$}{
        \If{$\mathbf{W}_i^{(\ell)}$ is not pruned} 
            {
            $\boldsymbol{\S}_{i,k}^{(\ell)} = 
              \begin{cases} 
              1  & \text{if  } i = i'_k \\
              0  & \text{otherwise } \\
              \end{cases}
             $
            }
        \Else{        
        $\boldsymbol{\S}_{i,:}^{(\ell)} \leftarrow {\argmin\limits_{\mathbf{s}}~\|\boldsymbol{\E}\|_2^{2} + \lambda_1 \|\boldsymbol{\B}\|_2^{2} + \lambda_2 \|\mathbf{s}\|_{2}^{2}}$  \tcp{obtained by Theorem \ref{thm:closedform}} 
        }
      }
    $\hat{\mathbf{W}}^{(\ell+1)} = \mathbf{W}^{(\ell+1)} \times_2 \boldsymbol{\S}^{(\ell)^T} $
    }
\Return $\hat{\mathbf{\Theta}}$
\end{algorithm}




\smalltitle{One-to-one vs. LBYL}
In one-to-one compensation approaches \cite{NM,Data-free}, they deliver the missing information for a pruned filter only to the most similar one of the remaining filters as shown in Figure \ref{fig:matrix:c}. Thus, this assumption is identical to the case that we have only one $s_{k}$ in Eq. (\ref{eq:goal2}), which would return a quite rough solution for the problem of minimizing the reconstruction error. Indeed, this one-to-one approach particularly fails to reduce the RE term as shown in Figure \ref{fig:error_components} of our experiments.

\begin{table*}[t] % 
\centering
{\normalsize 
\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{VGG-16 (Acc. 93.7)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{92.04} & 91.93 & 89.43 & \textbf{92.15} & 91.82 & 88.83 & 91.85 & \textbf{91.97} & 89.85 & \textbf{88.05} & 86.52 & 74.87 \\\hline
20\%& \textbf{87.84} & 87.24 & 71.77 & \textbf{87.97} & 86.42 & 72.04 & \textbf{89.51} & 86.93 & 73.64 & \textbf{75.24} & 63.33 & 37.19 \\ \hline
30\%& \textbf{83.25} & 76.91 & 56.95 & \textbf{82.83} & 75.58 & 52.40 & \textbf{81.80} & 75.01 & 49.79 & 45.67 & \textbf{46.86} & 12.81 \\ \hline
40\%& \textbf{66.81} & 54.32 & 31.74 & \textbf{67.19} & 52.24 & 30.46 & \textbf{56.63} & 52.54 & 17.78 & \textbf{31.34} & 26.79 & 10.00 \\ \hline
50\%& \textbf{45.71} & 32.58 & 12.37 & \textbf{49.46} & 32.13 & 11.71 & \textbf{43.32} & 27.87 & 10.43 & \textbf{21.56} & 18.08 & 10.00 \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{75.13} & 68.60 & 52.45 & \textbf{75.92} & 67.64 & 51.09 & \textbf{72.62} & 66.86 & 48.30 & \textbf{52.37} & 48.32 & 28.97\\ \Xhline{2\arrayrulewidth}   
\end{tabular}
}
\vspace{2mm}
\caption{Recovery results of VGG-16 on CIFAR-10}
\label{tab:VGG16-CIFAR10}
\vspace{1.5mm}
% \end{table}
%%%%%%%
% \begin{table}[t]
{\normalsize

\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{ResNet34 - ImageNet (Acc. 73.27)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{69.22} & 66.96 & 63.74 & \textbf{69.12} & 66.59 & 61.76 & \textbf{69.07} & 66.30 & 62.05 & \textbf{65.90} & 64.75& 52.97 \\ \hline
20\%& \textbf{62.49} & 55.70 & 42.81 & \textbf{62.27} & 55.39 & 43.45 & \textbf{61.18} & 53.95 & 40.61 & \textbf{50.64} & 48.40& 18.62 \\ \hline
30\%& \textbf{47.59} & 39.22 & 17.02 & \textbf{49.43} & 37.97 & 15.74 & \textbf{46.88} & 35.56 & 12.58 & 22.92 & \textbf{23.69} & 1.35  \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{59.77} & 53.96 & 41.19 & \textbf{60.27} & 53.32 & 40.32 & \textbf{59.04} & 51.94 & 38.41 & \textbf{46.49} & 45.61& 19.10\\ \Xhline{2\arrayrulewidth}
\end{tabular}
}
\vspace{2mm}
\caption{Recovery results of ResNet-34 on ImageNet}
\label{tab:ResNet34-ImageNet}
\vspace{1.5mm}

% \end{table}
% \begin{table}[t]
{\normalsize

\begin{tabular}{c||c|c|c||c|c|c||c|c|c||c|c|c}  \Xhline{2\arrayrulewidth}
\multicolumn{13}{c}{\textbf{ResNet101 - ImageNet (Acc. 77.31)}}
\\ \Xhline{2\arrayrulewidth} %\hline
Criterion & \multicolumn{3}{c||}{L2-norm} & \multicolumn{3}{c||}{L2-GM} & \multicolumn{3}{c||}{L1-norm}& \multicolumn{3}{c}{Random}\\ \hline
Pruning Ratio& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune& Ours& NM& Prune
\\ \Xhline{2\arrayrulewidth}
10\%& \textbf{74.59} & 72.36 & 68.90 & \textbf{74.54} & 72.38 & 68.38 & \textbf{74.19} & 72.05 & 68.33 & \textbf{59.78} & 57.13 & 46.55 \\ \hline
20\%& \textbf{68.47} & 61.42 & 45.78 & \textbf{69.03} & 61.02 & 46.25 & \textbf{68.52} & 60.57 & 44.57 & \textbf{34.85} & 15.78 & 6.83  \\ \hline
30\%& \textbf{55.51} & 37.38 & 10.32 & \textbf{56.65} & 33.74 & 7.65  & \textbf{56.11} & 36.43 & 9.32  & \textbf{13.27} & 2.31  & 0.60  \\ \Xhline{2\arrayrulewidth}
Average Acc. & \textbf{66.19} & 57.05 & 41.67 & \textbf{66.74} & 55.71 & 40.76 & \textbf{66.27} & 56.35 & 40.74 & \textbf{35.97} & 25.07 & 17.99\\\Xhline{2\arrayrulewidth}
\end{tabular}
}
\vspace{2mm}
\caption{Recovery results of ResNet-101 on ImageNet} \label{tab:ResNet101-ImageNet}
\vspace{1.5mm}
\end{table*}


\subsection{Our Train-Free Recovery Method with a Closed Form Solution}
Based on our data-free loss function in Eq. (\ref{eq:loss}), we now present our proposed train-free recovery method, called LBYL. First of all, we theoretically prove that the problem of minimizing $\mathcal{L}_{re}$ of Eq. (\ref{eq:loss}) has a closed form solution at the following theorem.
\begin{theorem} \label{thm:closedform}
The loss function $\mathcal{L}_{re}$ of Eq. (\ref{eq:loss}) is convex with a unique optimal solution as follows:
\begin{equation}
\small
    \boldsymbol{s}=[X^{T}X+\lambda_{1}\frac{\gamma_{j}^2}{\sigma_{j}^2} \boldsymbol{p}\boldsymbol{p}^{T}+\lambda_{2}I]^{-1}[X^{T}\boldsymbol{y}+\frac{\lambda_{1}\gamma_{j}}{\sigma_{j}}(\frac{\mu_{j}\gamma_{j}}{\sigma_{j}}-\beta_{j})\boldsymbol{p}],
    \nonumber
\end{equation}
where (1) $X = [\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{1}}{\sigma_{1}}\boldsymbol{f_{1}}~~...~~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j-1}}{\sigma_{j-1}}\boldsymbol{f_{j-1}}~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j+1}}{\sigma_{j+1}}\boldsymbol{f_{j+1}}~~...~~ \\
\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{m}}{\sigma_{m}}\boldsymbol{f_{m}}]$ such that $\boldsymbol{f_{i}}$ is the vectorized $i$-th filter in the $\ell$-th layer, (2) $\boldsymbol{y}$ is the vectorized $j$-th filter in the $\ell$-th layer, and (3) $\boldsymbol{p} =  [p_{1}~...~p_{j-1}~p_{j+1}~...~p_{m}]^T$ such that $p_{i} ={\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{i}}{\sigma_{i}}}{(\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i})}$.
% where (1) $X = [~...~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j-1}}{\sigma_{j-1}}\boldsymbol{f_{j-1}}~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{j+1}}{\sigma_{j+1}}\boldsymbol{f_{j+1}}~...~\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{m}}{\sigma_{m}}\boldsymbol{f_{m}}]$ such that $\boldsymbol{f_{i}}$ is the vectorized $i$-th filter in the $\ell$-th layer, (2) $\boldsymbol{y}$ is the vectorized $j$-th filter in the $\ell$-th layer, and (3) $\boldsymbol{p} =  [p_{1}~...~p_{j-1}~p_{j+1}~...~p_{m}]^T$ such that $p_{i} ={\frac{\sigma_{j}}{\gamma_{j}}\frac{\gamma_{i}}{\sigma_{i}}}{(\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i})}$.
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

Finally, given $\lambda_{1}$ and $\lambda_{2}$, Algorithm \ref{alg:Recovery} presents the whole procedure of our LBYL method using the closed form solution in Theorem \ref{thm:closedform}.

\smalltitle{Extension of LBYL to neuron pruning}
Even though this paper focuses on filter pruning, our LBYL method can also be applied to prune and restore neurons in vanilla feedforward neural networks consisting of only FC layers. We present the details in Appendix due to the space limitation.

% based on LBYL assumption in real time using the closed form solution in Theorem 1. Actually, this restoration algorithm can be extended to multiple pruned filters through just implementing above works iteratively. We represent the whole procedure in Algorithm \ref{alg:Recovery}.



% \smalltitle{Reasonable loss function}
% As shown in Lemma 2, there are three error components in (12), which are related with Sum of Squared Error(SSE) and Batch normalization Error(BE) and Activation Error(AE), respectively. Unfortunately, we cannot control data driven feature map $\mathbf{Z}^{(\ell-1)$ and matrix $R$. So we alternatively try to minimize the norm of two terms, $\boldsym{\epsilon}$ and $B$ respectively. Moreover, we place regularization term in loss function lastly for the purpose of mitigating explosion of matrix $R$. For example, one element of matrix $R$ maybe too large if some of the coefficients are positively large and elements corresponding to that coefficients are negative, but elements corresponding to others are positive. Finally, we formulate the reasonable restoration loss function as below Eq.(16).








% \begin{lemma} If there are both BN and ReLU between feature map and activation map, the reconstruction error can be formulated in a data-free manner as follows:
%     \begin{equation} 
%     \| \mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)}\|_{1}=
%      \| \frac{\gamma_{j}}{\sigma_{j}}{(\mathbf{Z}^{(\ell-1)}\circledast\boldsymbol{\epsilon})}+ B + R\|_{1},
%      \end{equation}\nonumber
%      \label{lemma}
% where $\mathbf{\epsilon}=\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)}$, $B$=$\gamma_{j} \over \sigma_{j}$$\{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j $, $R$ is w $\times$ h matrix where $ R_{u,v}$ = |$\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,u,v}^{(l+1)})-min(0,\mathbf{Z}_{j,u,v}^{(l+1)})$|, and $\mu,\gamma,\sigma,\beta$ are the batch normalization parameters.
% \end{lemma}
% where,$\mathbf{\epsilon}=\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)}$, $B$=$\gamma_{j} \over \sigma_{j}$$\{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j $, $R$ is w $\times$ h matrix where $ R_{u,v}$ = |$\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,u,v}^{(l+1)})-min(0,\mathbf{Z}_{j,u,v}^{(l+1)})$|, and $\mu,\gamma,\sigma,\beta$ are the batch normalization parameters.



 

% Our approximation scale for pruned filter in $\ell$-th layer is computed to recovery filters in $\ell+1$-th layer. Algorithm of our proposed method is largely two parts. In the case of remained filter, we do not compute the approximation scale. And in the case of pruned filter, we compute the approximation scale on remained filters. Through the process to minimize Eq. (\ref{eq:eq10}), we can get the approximation scales for preserved filter. Approximation scale is computed each $\ell$-th layers that perform pruning.

 
 
 
%  is vectorized $i$-th filter in $l$-th layer for $i \in [1,m_{l}] \setminus$ \{$j$\}, $\boldsymbol{y}$ is vectorized $j$-th filter in $l$-th layer, $\boldsymbol{p}$ is ($m_{l}-1$)-dimensional vector whose i-th component is $\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}$ for $i \in [1,m_{l}] \setminus$ \{$\textit{j}$\}.

% Meanwhile, our LBYL method can have more flexibility in Error components. We consider a reasonable loss function that reflect all error components comprehensively. Through this loss function, we can find more optimal solution $\boldsymbol{s}$ in Eq.(10) than One-to-One compensation method.





% They consider SSE and BE and AE to a degree, but their methods are so heuristic and can have large disadvantage of SSE. For example, Kim \textit{et.al} \cite{NM} choose one of the preserved filters based on their customized score which reflect SSE and BE at different degree. This degree is decided by parameter $\lambda$ which need to be searched. Furthermore, Kim \textit{et.al} \cite{NM} decide whether to compensate or not based on cosine similarity between the preserved and pruned filter at the end. That is, they are both depend on the similarity between pruned and preserved filter, and they suffer from little similarity in some layers as shown in \cite{NM} which result in large SSE. On the other hand, they may have advantage in terms of BE since they have only one BN parameter in $\boldsymbol{B}$ term. 




% We should consider batch normalization to minimize reconstruction form. In case of BN, we also assume that the the feature map $\mathbf{Z}_{j,:,:}^{(\ell+1)}$ generated by pruned filter $\mathbf{W}_{j,:,:,:}^{(\ell)}$ can be represented linear combination of feature maps $\mathbf{Z}_{i,:,:}^{(\ell+1)}$ generated by preserved filters $\mathbf{W}_{i,:,:,:}^{(\ell)} i \in [1,m] \setminus {\{$\textit j$\}}$.

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \text{Eq.} (\ref{equation1}). &= \| \N(\mathbf{Z}_{j,:,:,:}^{(\ell)}) - \sum\limits_{i = 1, i \neq j }^{m} {s}_{i}^{\prime} \times \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)} ) \|_{1} \\ 
%  &=\| \frac{\gamma_{j}(\mathbf{Z}_{j,:,:,:}^{(l)} - \mu_j)}{\sigma_{j}} + \beta_{j}- \sum\limits_{i = 1, i \neq j }^{m}{{s}_{i}^{\prime} \times \{ \frac{\gamma_{i}(\mathbf{Z}_{i,:,:,:}^{(l)} - \mu_i)}{\sigma_{i}} + \beta_{i}}\} +B \|_{1}\\
% \end{split}
% \end{eqnarray}
% where ${s}_{i}^{\prime}$ = $\frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}}{s}_{i}$ is the scale considered by batch normalization and
% we want bias caused by considering the batch normalization to be zeroed. $B=\frac{\sigma_{j}}{\gamma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{i}}{\gamma_{i}}\beta_i) - \mu_j \} + \beta_j$ \} and $\mu,\gamma, \sigma$ is the batch normalization parameters $\in \mathbb{R}^{n \times w \times h}$ for feature maps. 


% % $\mathbf{B} = \frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j + \frac{\gamma_{j}}{\sigma_{j}}(\mathbf{Z}^{(\ell)}\circledast\boldsymbol{\epsilon} \} + \beta_j$ \} to $\mathbf{B}=\frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m} s_{i} (\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j \} + \beta_j$ \} and $\mu,\gamma, \sigma$ is the batch normalization parameters $\in \mathbb{R}^{n \times w \times h}$ for feature maps. 

% Through the lemma below, we can find the reconstruction error caused by batch normalization layer.
% \newtheorem*{lemma}{Lemma} 
% \begin{lemma} From the above equation, we can get the reconstruction error considering batch normalization.
%     \begin{equation} 
%     \| \mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)}\|_{1}  = \| \frac{\sigma_{j}(\mathbf{Z}^{(\ell-1)} \circledast \mathbf{\epsilon})}{\gamma_{j}} + B \|_{1}\\
%     \end{equation}\nonumber
% \end{lemma}

% Therefore, we want both $B$ and  $\mathbf{\epsilon}$ zero..

% \smalltitle{Considering Activation Function}
% Moreover, our assumption should extend to next layer that is activation layer. Therefore we assume that activation map generated by pruned filter can be represented by linear combination of activation maps generated by remained filters.

% \begin{eqnarray} \begin{split}\label{eq:eq}
%      \text{Eq.} (\ref{equation1}). &= \| \F\circ(\N(\mathbf{Z}_{j,:,:,:}^{(\ell)})) - \sum\limits_{i = 1, i \neq j }^{m} {s}_{i}^{\ast} \times \F\circ(\N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)})) \|_{1} \\ 
%      &= \| \F\{\N(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}),0\} - \sum\limits_{i = 1, i \neq j }^{m_{i}} \F\{\boldsymbol{s}_{i}^{\ast} \times \N(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})\} +\F(\boldsymbol{K}) \} \|_1
%      \end{split}
% \end{eqnarray}

% \begin{lemma} From the above equation, we can get the reconstruction error considering activation. More detailed derivation is in appendix.
%     \begin{equation} 
%      \| \frac{\sigma_{j}}{\gamma_{j}}(\mathbf{Z}^{(\ell)}\circledast\boldsymbol{\epsilon})+ B + AE\|_{1}
%      \end{equation}\nonumber
%      \label{lemma}
% \end{lemma}
% where, $ AE = \sum\limits_{m=1}^{h^{\prime}}\sum\limits_{n=1}^{w^{\prime}}-min(0,\mathbf{Z}_{j,m,n}^{(l+1)})+\sum\limits_{k=1, k \neq j}^{m} s_{k}min(0,\mathbf{Z}_{k,m,n}^{(l+1)}) \in \boldsymbol{R}^{h^{\prime} \times w^{\prime}}$

% Finally, we should minimize $B$ and  $\mathbf{\epsilon}$ and activation error zero..


% \smalltitle{Objective Function}
% As shown in lemma(\ref{lemma}) above, we should minimize the $b$ to reduce the reconstruction error,which leads to reduction of the error caused from activation. Plus, we also reduce the difference between pruned filter and remained filters. Therefore, we design the loss to minimize reconstruction with errors we consider above.  
% \begin{equation}
%      \mathcal{L}_{re} =  \| \mathbf{W}_{j,:,:,:}^{(\ell)} - \sum\limits_{i = 1, i \neq j }^{m} s_{i} \mathbf{W}_{i,:,:,:}^{(\ell)} \|_2^{2} + \lambda_1 \|B\|_2^{2} + \lambda_2 \|s_i \|_{2}^{2},
% \label{eq:eq10}
% \end{equation}
% where $i \in [1,m] \setminus {\{$\textit j$\}}$.

% By using the loss function to find the optimized scale, we can control the three error components. First, Sum of Squared Error(\textit{SSE}) that means difference between pruned filter and linear combination of remained filters can be minimized by first terms in Eq. (\ref{eq:eq10}). Second, Batch normalization Error (\textit{BE}) that means error caused by batch normalization layer also can be reduced. Finally, the Activation Error (\textit{AE}) that error from the activation error can be decreased weakly by third term in Eq. (\ref{eq:eq10}) in the sense of preventing amplification of some coefficient $s_{i}$ that may amplify the activation error term. Through this loss function, we can find more optimal solution 
% $s$ than one-to-one compensation method. Furthermore, we investigate that minimizing loss function is truly helpful in Theorem 1 because we substitute scale ($\boldsymbol{\mathcal{S}}^{\prime}$) for scale ($\boldsymbol{\mathcal{S}}^{\ast}$) considering the activation.

% % The difference between  $\boldsymbol{Z}_{j,:,:}^{(l+1)}$ and $ \sum\limits_{n = 1, n \neq j}^{m_{l}}{S_{n}} \boldsymbol{Z}_{n,:,:}^{(l+1)}$ can be quantified as below Theorem 1.
% % \smalltitle{\textit{Theorem 1}} If we assume Eq. (\ref{eq:eq6})., we can assume s_{i}^{\prime} = \frac{\gamma_{j}}{\sigma_{j}}\frac{\sigma_{i}}{\gamma_{i}}s_{i}$ for $i \in [1,m] \setminus$ \{$j$\} and $\| \boldsymbol{Z}_{j,:,:}^{(l+1)} - \sum\limits_{n = 1, n \neq k}^{m}{S_{k}} \boldsymbol{Z}_{k,:,:}^{(l+1)}\|_{1}$ can be represented as below. The detailed derivation process is in appendix.



% From Theorem 1, we get to know that we should minimize $b$ and $\boldsymbol{\epsilon}$ and the last term concerned with activation layer to minimize the reconstruction error. Thus, in general compensation method, we should find the scalars $s_{i}$ for $i \in [1,m] \setminus$ \{$\textit{j}$\} which minimize the three error components.



% \subsection{Our Train-Free Recovery Method with a Closed Form Solution}

% Moreover, as mentioned earlier, To propose data-free and training-free method. We use the closed form solution and then compensate pruned filter in a real time. Our loss function is the loss function is convex and there exists a unique solution as shown below at Theorem 2.

% \smalltitle{\textit{Theorem 2}} The loss function in Eq. (\ref{eq:eq10}). is convex and there exists a unique optimal solution. More detailed derivation is in appendix.
% \begin{equation}
%     s_{i}=[X^{T}X+\lambda_{1}\frac{\gamma_{j}^2}{\sigma_{j}^2} \boldsymbol{p}\boldsymbol{p}^{T}]^{-1}[X^{T}\boldsymbol{y}+\frac{\lambda_{1}\gamma_{j}}{\sigma_{j}}(\frac{\mu_{j}\gamma_{j}}{\sigma_{j}}-\beta_{j})\boldsymbol{p}]
% \label{eq:eq}\nonumber
% \end{equation}
%  where $X_{:,i}$ is vectorized $i$-th filter in $l$-th layer for $i \in [1,m_{l}] \setminus$ \{$j$\}, $\boldsymbol{y}$ is vectorized $j$-th filter in $l$-th layer, $\boldsymbol{p}$ is ($m_{l}-1$)-dimensional vector whose i-th component is $\mu_{i}-\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}$ for $i \in [1,m_{l}] \setminus$ \{$\textit{j}$\}.

% Finally, given $\lambda_{1}$ and $\lambda_{2}$, we can implement many-to-one compensation Algorithm in real time using the closed form solution in Theorem 2. Actually, this compensation algorithm can be extended to multiple pruned filters through just implementing above works iteratively. We call this compensation Algorithm LBYL. We represent how LBYL works in Algorithm \ref{alg:Recovery}. Our approximation scale for pruned filter in $\ell$-th layer is computed to recovery filters in $\ell+1$-th layer. Algorithm of our proposed method is largely two parts. In the case of remained filter, we do not compute the approximation scale. And in the case of pruned filter, we compute the approximation scale on remained filters. Through the process to minimize Eq. (\ref{eq:eq10}), we can get the approximation scales for preserved filter. Approximation scale is computed each $\ell$-th layers that perform pruning.

% \begin{algorithm}[htb]
%   \caption{LBYL Algorithm}
%   \label{alg:Recovery}
%   \KwIn{$\boldsymbol{W}^{{(\ell)}}$ $\in$ $\boldsymbol{R}^{m_l \times n_l\times k \times k}$, set of remained filter $R = \{r_1, r_2, ..., r_{t_l}\}$} 
%   \KwOut{Approximation matrix $s^{(\ell)}$ $\in$ $\boldsymbol{R}^{m_{l} \times t_l}$}
   
%   Initialize ${s}^{(\ell)}$ $\in$ $\boldsymbol{R}^{m_{l} \times t_l}$ with 0
  
%   \For{each filter $w_m$ $\in$ $\mathbb{R}^{n_{l} \times k \times k}$   $\mathbf{in}$ $\mathbf{W}^{(\ell)}$}
%     {
%     \If{w_m $\in$ R} 
%         {
%         ${i} \leftarrow $index of $w_m$ within $\boldsymbol{W}^{{(\ell)}}$
        
%         $s_{i,m}^{(\ell)} \leftarrow$ 1
%         }
%     \Else{        
%     approximation~scale~list $\leftarrow$ $\underset{s^{\ell}}{\mathrm{argmin}}$ Eq. \ref{eq:eq10}.
    
%     ${i} \leftarrow $ index of $w_m$
    
%         \For{each scale $\mathbf{in}$ approximation scale list}
%             {
%                 ${j} \leftarrow $index of scale within approximation scale list
                
%                 $s_{i,j}^{(\ell)} \leftarrow $scale \times \frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}} 
                
%           }
%       }
%     }
% \Return $s^{(\ell)}$
% \end{algorithm}


% \smalltitle{Discussion on one-to-one vs. many-to-one approach}
% In one-to-one compensation \cite{NM,Data-free}, they prudently choose one of the preserved filters corresponding to one pruned filter, and then compensate like general compensation method. so in this case, there is one $s_{i}$ in Eq. (\ref{eq:eq6}).
% They consider SSE and BE and AE to a degree, but their methods are so heuristic and can have large disadvantage of SSE. For example, Kim \textit{et.al} \cite{NM} choose one of the preserved filters based on their customized score which reflect SSE and BE at different degree. This degree is decided by parameter $\lambda$ which need to be searched. Furthermore, Kim \textit{et.al} \cite{NM} decide whether to compensate or not based on cosine similarity between the preserved and pruned filter at the end. That is, they are both depend on the similarity between pruned and preserved filter, and they suffer from little similarity in some layers as shown in \cite{NM} which result in large SSE. On the other hand, they may have advantage in terms of BE since they have only one BN parameter in $\boldsymbol{B}$


%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Proposed Method} \label{sec:method}

% Most of filter pruning methods try to select filters to be pruned prudently so that pruned network's output be similar to the original network's. To this end, they prune the unimportant filters and then fine-tune the pruned network with using the train data. How can we restore the the pruned networks without any data? In other words, it implies that we cannot use any data-driven values(i.e., activation maps) and we can only exploit the values of original filters. In that case, the only thing we can do maybe changing the weights of remained filters appropriately not to amplify the difference between pruned and unpruned network's outputs through the information of original filters.



% \smalltitle{Problem Statement} For a Convolutional Neural Network (CNN) with $L$ layers, we denote $\mathbf{Z}{^{(\ell-1)}}$ $\in$ $\mathbb{R}^{n_{l} \times h_{l} \times w_{l}} $ is activation maps at $l$-th layer, where $n_{l}$, $h_{l}$ and $w_{l}$ are the number of channels, height and width in activation maps, respectively. and we denote $\mathbf{W}^{{(\ell)}}$ $\in$  $\mathbb{R}^{m_l \times n_l\times k \times k}$ is covolution filters in $l$ -th layer,where $m_l$, $n_l$ and $k$ are the number of filters, number of channels and kernel size, respectively. Trough the convolution operation using activation map $\mathbf{Z}{^{(\ell-1)}}$ and convolution filter $\mathbf{W}^{{(\ell)}}$ in $l$-th layer, the feature maps $\boldsymbol{\mathcal{A}}^{{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l} \times h_{l+1} \times w_{l+1}}$ is computed as shown in Eq. (\ref{eq:eq1}).

% \begin{equation}
% \boldsymbol\alpha^{(l+1)} = {\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)}}
% \label{eq:eq1}
% \end{equation}

% and the feature maps passed through the BN and ReLU layer are activation maps $\mathbf{Z}{^{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l} \times h_{l+1} \times w_{l+1}} $ in $i+1$ -th layer as shown in Eq. (\ref{eq:eq2}).

% \begin{equation}
% \mathbf{Z}^{(l+1)} = \mathcal{F}({\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)}})
% \label{eq:eq2}
% \end{equation}
% where $\mathcal{F}$ is the function that implement batch normalization and non-linear activation(e.g., ReLU).

% If the filter pruning is performed in $l$-th layer, the shape of original filters $\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_l \times n_l\times k \times k}$ is modified to ${\hat {\mathbf{W}}^{(\ell)}}$ $\in$ $\mathbb{R}^{t_l \times n_l\times k \times k}$, where $t_l$ $<$ $m_l$ by pruning criterion. Therefore, the pruned activation maps ${\hat {\mathbf{Z}}}{^{(l+1)}}$ $\in$ $\mathbb{R}^{t_{l} \times h_{l+1} \times w_{l+1}}$ in ($l+1$)-th layer is computed by Eq. (\ref{eq:eq3}).

% \begin{equation}
% \mathbf{\hat{Z}}^{(l+1)} = \mathcal{F}({\mathbf{Z}^{(\ell)} \circledast {\mathbf{\hat{W}}}^{(\ell)}})
% \label{eq:eq3}
% \end{equation}

% Moreover, corresponding channels of each filters in ($l+1$) -th layer are sequentially removed. As a result, shape of original filters $\mathbf{W}^{{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times m_l\times k \times k}$ in ($l+1$) -th layer is changed to  ${\hat {\mathbf{W}}^{(l+1)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times t_l\times k \times k}$. Although the pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times h_{l+1} \times w_{l+1}}$ in ($l+2$) -th layer have same shape with original feature maps $\boldsymbol{\mathcal{A}}^{{(l+2)}}$ $\in$ $\mathbb{R}^{m_{l+1} \times h_{l+1} \times w_{l+1}}$, the pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ are damaged. Thus, we make approximation scales $\testit{s}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$ with relationship between the pruned filter and preserved filters in $l$-th layer and then apply it to the original filters in ($l+1$) -th layer to compensate for pruned feature maps $\boldsymbol{\hat{\alpha}}^{{(l+2)}}$ as shown in Eq. (\ref{eq:eq4}).
% (i.e., change $\hat{\mathbf{W}}^{(l+1)}$ to ${\mathbf{W}}^{(l+1)}$ \circledast  ${\boldsymbol{\mathcal{S}}} $)

% \begin{equation}
% \boldsymbol\alpha^{(l+2)} = {\mathbf{Z}}^{(l+1)} \circledast {\mathbf{W}}^{(l+1)}
% \approx {\hat{\mathbf{Z}}^{(l+1)} \circledast {\mathbf{W}}^{(l+1)} \circledast  {\boldsymbol{\mathcal{S}}} = \boldsymbol{\hat{\alpha}}^{{(l+2)}}}
% \label{eq:eq4}
% \end{equation}

% Our goal is finding the approximation scales $\testit{s}$ to minimize the reconstruction error between the pruned model and the original model without any data, and consequently compensating for pruned filters in neural network using this approximation scales $\testit{s}$,which can be represented as below in Eq. (\ref{eq:eq5}).

% \begin{equation}
% \boldsymbol{\mathcal{S}} =  \underset{{\mathcal{S}}}{\mathrm{argmin}} \sum\limits_{{i} = 1}^{m_{l+1}}\|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}-\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+2)}}}\|_1
% \label{eq:eq5}
% \end{equation}


% \kim{From this part(below), should be checked thoroughly again!! this part is so important. There are too many mathematical expression error.....}
% \subsection{One-to-one compensation}
% As mentioned in introduction, in one-to-one compensation, they assume that one pruned filter can be approximated by one remained filter\cite{NM,Data-free}(i.e., $ W_{pruned} \approx S\circledastW_{remained} $ ). And more clearly, This can be represented as below.\kim{the below equation and below sentences are not matched each other! You should check it carefully!}


% \begin{equation}
% % \boldsymbol{W}_{j,:,:,:}^{(\ell)} ={\boldsymbol\beta}_{:,j}^{(\ell)} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)}  + \boldsymbol{\epsilon}
% \boldsymbol{W}_{j,:,:,:}^{(\ell)} = \boldsymbol{S} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} 
% \label{eq:eq6}
% \end{equation}
% where $i$-th filter is the the preserved filter in $l$ -th layer and $j$-th filter is the pruned filter in the same layer and $\mathcal{S}$ is the scale and ${\boldsymbol{\epsilon}}$ is the residual. \kim{I think that the definition of scale more clearly.}

% the reconstruction error formula can be represented as below.
% \begin{eqnarray} \begin{split}\label{eq:eq7}
%         \mathcal{L}_{re} = \sum\limits_{{i} = 1}^{m_{l+1}} \|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}- \mathcal{F}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}}) \circledast  \mathbf{W}_{i,:,:,:}^{(l+1)} \circledast \boldsymbol {\mathcal{S}}_{i,:}^{(\ell)}\|_1 
% \end{split}
% \end{eqnarray}
% The channels of preserved filter in ($l+1$)-th layer are compensated using the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ obtained from the relationship between pruned filter and preserved filter in $l$-th layer \cite{NM,Data-free}. \cite{NM} first prudently choose one of the preserved filters corresponding to each pruned filter in $l$-th layer based on the cosine similarity and bias caused by batch normalization. Then calculate the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ reflecting the batch normalization scale. Finally, \cite{NM} determine whether to apply the scale $\boldsymbol{\mathcal{S}}_{i,:}^{(\ell)}$ to the original filters or not.\kim{I think the exact description about S is needed!!}

% \subsection{Many-to-one compensation}
% We propose the many-to-one compensation method to sufficiently compensate for the pruned filter. To this end, we approximate the pruned filter with the linear combination of preserved filter. Actually, one-to-one compensation ignore the residual term. in real case, there exists non trivial residual. Therefore it can be showed more clearly as below Eq. (\ref{eq:eq7}).

% \begin{equation}
% \boldsymbol{W}_{j,:,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)}  + \boldsymbol{\epsilon} 
% \label{eq:eq8}
% \end{equation}

% The reconstruction error about the many-to-one compensation can be represented using Eq. (\ref{eq:eq9}).


% \begin{eqnarray} \begin{split}\label{eq:eq9}
%     \mathcal{L}_{re} = \sum\limits_{{i} = 1}^{m_{l+1}}\|{\boldsymbol{\alpha}_{i,:,:}^{{(l+2)}}- \mathcal{F}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}}) \circledast  \mathbf{W}_{i,:,:,:}^{(l+1)} \circledast \boldsymbol{{\mathcal{S}}}_{i,:}^{(\ell)}\|_1 
% \end{split}
% \end{eqnarray}
% where $\boldsymbol{\mathcal{K}}$ = $\frac{\gamma_{j}}{\sigma_{j}}[\sum\limits_{{i} = 0 , i \neq j}^{m_{i}}\{(\boldsymbol{S}_{i}\mu_{i} -\frac{\sigma_{i}}{\gamma_{i}}\beta_{i}) - \mu_{j} \} ]+ \beta_{j}$ is bias term about the batch normalization. The derivation process for the above reconstruction error formula is in appendix.\kim{Where is K?? and to add it in appendix, you prefer to make it Lemma or Theorem!!}


% \smalltitle{\textit{Approximation for scale}} To find out the optimized approximation scale for compensation, We start from our assumption pruned filter is represented by linear combination of multiple filters in $l$-th layer and extend our assumption to up to next activation maps in $l+1$-th layer and then compute the approximation scale. First, we can extend our assumption to the followed feature map generated by pruned filter using our assumption as shown below.
% \begin{equation}
% \boldsymbol{\alpha}_{j,:,:}^{(l+1)} =\sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i} \times \boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{W}_{i,:,:,:}^{(\ell)}   +  \boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{\epsilon}
% \label{eq:eq10}
% \end{equation}



% As we assume that the pruned filter is represented by linear combination of preserved filter, in batch normalization layer, we can also assume that the the feature map generated by pruned filter can be represented linear combination of feature maps generated by preserved filters as shown in Eq. (\ref{eq:eq11}). \kim{at below equation, what is mi? is m depend on i? this is strange. }

% \begin{eqnarray} \begin{split}\label{eq:eq11}
%     \boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) &= \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})    +\boldsymbol{K} \\
%  \frac{\gamma_{j}(\boldsymbol{\alpha}_{j,:,:}^{(\ell)} - \mu_j)}{\sigma_{j}} + \beta_{j} & =  \sum\limits_{i = 1, i \neq j }^{m_{i}}{\boldsymbol{S}_{i}^{\prime} \times \{ \frac{\gamma_{i}(\boldsymbol{\alpha}_{i,:,:}^{(\ell)} - \mu_i)}{\sigma_{i}} + \beta_{i}}\} +\boldsymbol{K} \\
% \end{split}
% \end{eqnarray}
% \kim{K dimension error!! Add operation cannot be used!}
% where $\boldsymbol{S}_{i}^{\prime} = \frac{\gamma_{j}\sigma_{i}}{\sigma_{j}\gamma_{i}}\boldsymbol{S}_{i}$ and $\boldsymbol{K} = \frac{\gamma_{j}}{\sigma_{j}} \{ \sum\limits_{i = 1, i \neq j }^{m_{i}}(\boldsymbol{\alpha}_{j,:,:}^{(\ell)}\mu_{i} -  \frac{\sigma_{j}}{\gamma_{j}}\beta_i) - \mu_j + (\boldsymbol{Z}_{i,:,:}^{(\ell)} \circledast \boldsymbol{\epsilon})\} + \beta_j$.

% And our assumption should extend to next layer that is activation layer as shown in Eq. (\ref{eq:eq12}). 
% \begin{eqnarray} \begin{split}\label{eq:eq12}
%     \boldsymbol{max}\{\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}),0\} &= \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{max}\{\boldsymbol{S}_{i}^{\ast} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}),0\} +\boldsymbol{max}(\boldsymbol{K},0)
% \end{split}
% \end{eqnarray}
% Unfortunately, we can't extend our assumption without any data. That is, it means we should consider all cases for possible branches. Therefore, we extend our assumption feature maps passed through the batch normalization layer in $l+1$-th layer as shown in Eq. (\ref{eq:eq13}). 
% \begin{eqnarray} \begin{split}\label{eq:eq13}
%     \boldsymbol{\alpha}_{j,:,:}^{(l+2)} & = \boldsymbol{BN}(\boldsymbol{\alpha}_{:,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,:,:,:}^{(l+1)}) \\
%     &\approx \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{\acute{W}}_{j,i,:,:}^{(l+1)}) = \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}\{\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast (\boldsymbol{W}_{j,i,:,:}^{(l+1)}+\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{W}_{j,j,:,:}^{(l+1)}) \}\\
%     &=\sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,i,:,:}^{(l+1)}) + \sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}) \circledast  \boldsymbol{W}_{j,j,:,:}^{(l+1)}\\
%     &=\sum\limits_{i = 1, i \neq j}^{m_{i}} \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)} \circledast \boldsymbol{W}_{j,i,:,:}^{(l+1)}) + (\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \boldsymbol{K})\circledast  \boldsymbol{W}_{j,j,:,:}^{(l+1)}   % \text{ by Eq. }(\ref{eq:eq11})
% \end{split}
% \end{eqnarray}

% we should minimize $\boldsymbol{K}$,which leads to ultimately reduce the reconstruction error in $l$-th layer induced from removed filter in $l$-th layer the from Eq. (\ref{eq:eq13}). 
% Moreover, we decompose $\boldsymbol{K}$ to optimize the the approximation scale that minimize the reconstruction error and discover that the $\boldsymbol{K}$ is composed of three error terms,which are Sum of Squares Error (\textit{SSE}, $\boldsymbol{\varepsilon}$), Batch Normalization Error (\textit{BE}, \boldsymbol{K}) and Activation Error (\textit{AE}, $\boldsymbol{\mathds{1}}$).
% \begin{eqnarray} \begin{split}\label{eq:eq14}
%         \boldsymbol{\|\boldsymbol{K}\|_1} & =  \|\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})  \|_1 \\
%         & = \|\boldsymbol{\varepsilon} -\boldsymbol{\mathds{1}}\times\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) + \sum\limits_{i = 0, i \neq j }^{m_i}\boldsymbol{\mathds{1}_{i}} \times\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)}) \|_1 \\
%         & \le  \|\boldsymbol{\varepsilon}\|_1 + \|\sum\limits_{i = 0, i \neq j }^{m_i}\boldsymbol{\mathds{1}_{i}} \times\boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})  -\boldsymbol{\mathds{1}}\times\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)})\|_1
% \end{split}
% \end{eqnarray}
% where $\boldsymbol{\mathds{1}}$ is the indicator variable$\boldsymbol{\varepsilon}$ = $\boldsymbol{BN}(\boldsymbol{\alpha}_{j,:,:}^{(l+1)}) - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{S}_{i}^{\prime} \times \boldsymbol{BN}(\boldsymbol{\alpha}_{i,:,:}^{(l+1)})$. \kim{Is it better than the direc delta? and the indicator notation is not correct!! you should describe about indicator more clearly!}

% Therefore, we set a reasonable loss function as below that can overall control SSE and BE (and weakly AE through L2-regularization) Eq. (\ref{eq:eq14}) and optimizing this loss function, we can obtain nicely a closed form solution as Theorem 1.

% \smalltitle{\textit{Theorem 1}} The unique closed form solution. we will use the property of positive definite matrix and weak vector calculus to prove that (in appendix). \kim{The sentence in Theorem 1 is not that!!}
% \begin{equation}
%     \mathcal{L}_{re} =  \| \boldsymbol{W}_{j,:,:,:}^{(\ell)} - \sum\limits_{i = 1, i \neq j }^{m_{i}} \boldsymbol{\mathcal{S}}^{l} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} \|_2 + \boldsymbol{\lambda_1} {\|\boldsymbol{K}\|_2} + \boldsymbol{\lambda_1} {\|\boldsymbol{\mathcal{S}}^{(\ell)}\|_2}
% \label{theorem:theorem1}
% \end{equation}

% Using this closed form solution, we can compensate pruned filter in a real time. we call this compensation method LBYL. LBYL can have advantage in the perspective of SSE. Furthermore, LBYL also reduces other error components (BE, AE) so that pruned filter can be compensated more optimally.\kim{there are some nuance difference.. for example.. are we reducing all BE and AE??(specifically we are not controlling AE clearly!!) I think the previous representation that I wrote is more valid.......} There is the whole procedure of LBYL described in Algorithm 1.


% \begin{algorithm}[tb]
%   \caption{Compensation Algorithm}
%   \label{alg:Compensation}
%   \KwIn{$\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_l \times n_l\times k \times k}$, set of remained filter $R = \{r_1, r_2, ..., r_{t_l}\}$, set of pruned filter $P = \{p_1, p_2, ..., p_{m_{l}-{t_l}}\}$}
%   \KwOut{Approximated scale matrices $\boldsymbol{\mathcal{S}}^{l}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$}
   
%   Initialize $\boldsymbol{\mathcal{S}}^{l}$ $\in$ $\mathbb{R}^{m_{l} \times t_l}$ with 0 \;
  
%   \For {each filter w_m $\in$ $\mathbb{R}^{n_{l} \times k \times k}$ \  $\mathbf{in}$ \ \mathbf{W}^{(\ell)}}
%     {
%     \If{w_m $\in$ $R$} 
%         {
%         ${i} \leftarrow $index of $w_m \ $within \mathbf{W}^{{(\ell)}} \\
%         $\boldsymbol{\mathcal{S}}_{i,m}^{(\ell)} \leftarrow$ 1
%         }
        
%     \Else{
%         ${approximation \ scale \ list} \leftarrow $ \underset{\mathcal{S}^{l}}{\mathrm{argmin}} Eq. \ref{eq:eq12} \\
%         ${i} \leftarrow $index of w_m \\
        
%         \For {scale $\mathbf{in}$ approximation scale list}
%         {
%             ${j} \leftarrow $index of scale within approximation scale list \\
%             ${\boldsymbol{\mathcal{S}}_{i,j}^{(\ell)}} \leftarrow scale $\\
            
%         }
%         }
%     }
%     \Return $\boldsymbol{\mathcal{S}}^{(\ell)}$
% \end{algorithm}





% \begin{equation}
% {\boldsymbol{\tilde{\mathbf{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast \mathbf{W}_{i,k}^{(\ell+1)}
% \label{eq:eq}
% \end{equation}




% By compensation in a manner like Eq.(4), the pruned feature map (5) change to the compensated feature map ${{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}}$ as below Eq.(7).

% \begin{equation}
% {{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k}^{(\ell)} \circledast (\mathbf{W}_{i,k}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j}^{(\ell+1)})
% \label{eq:eq}
% \end{equation}




% By using Eq.(8), the reconstruction error of feature map in $(\ell+1)$-th layer can be represented as below Eq.(9).





% \smalltitle{Without BN, ReLU}
% As shown in Eq.(11), we should find scalars $s_{k}$ such that $\mathbf{A}_{j}^{(\ell+1)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(l+1)}$ to minimize the reconstruction error (5). We start the error analysis cosidering the situation where there are no BN and ReLU between feature map and activation map. BN and ReLU will be reflected sequentially. In that case, $\mathbf{A}^{(\ell)} = \mathbf{Z}^{(\ell)}$ and as a result, (12) can be represented as below Eq.(13).

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1} \\
%      = &~\| (\mathbf{Z}^{(\ell-1)}  \circledast (\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}

% Since we cannot control the data driven feature map $\mathbf{Z}^{(\ell-1)}$, the only thing we can do is minimizing the term $(\mathbf{W}_{j}^{(l)} - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \mathbf{W}_{k}^{(l)} )$ which is called SSE.

% In order for the information carried by the pruned filter to be delivered to the other filters at the same layer, we have to examine how the value of the pruned filter is related to those of the others. Our proposed assumption is that a pruned filter can be represented as a \textit{linear combination} of all the preserved filters. Let $\mathbf{W}_{j,:,:,:}^{(\ell)}$ denote such a pruned filter at the $\ell$-th layer. Then, it can be represented as follows:
% \begin{equation}
% \mathbf{W}_{j,:,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m} s_{i} \times \mathbf{W}_{i,:,:,:}^{(\ell)}  + \epsilon,
% \label{eq:linear}
% \end{equation}
% where $s_i$ quantifies to what extent each $i$-th preserved filter can contribute to form the pruned filter and $\epsilon$ is an approximation error.


% With the proposed assumption of Eq. (\ref{eq:linear}), let us examine how the reconstruction error of Eq. (\ref{eq:goal}) can further be derived in a way of not using any data-dependent values.

% Meanwhile, $i$-th channel of feature map $\mathbf{Z}_{i,:,:}^{{(\ell+1)}}$ in $(\ell+1)$-th layer can be showed as below.

% \begin{equation}
% {{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1}^{m} {\mathbf{A}}_{k,:,:}^{(\ell)} \circledast \mathbf{W}_{i,k,:,:}^{(\ell+1)}
% \label{eq:eq3}
% \end{equation}

% The pruned feature map in the same position can be showed as below.

% \begin{equation}
% {\boldsymbol{\tilde{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k,:,:}^{(\ell)} \circledast \mathbf{W}_{i,k,:,:}^{(\ell+1)}
% \label{eq:eq}\nonumber
% \end{equation}

% And the compensated feature map in the same position can be showed as below.

% \begin{equation}
% {\tilde{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1}^{t}\mathbf{\tilde{A}}_{k,:,:}^{(\ell)}\circledast({\mathbf{W}}^{(\ell+1)} \times_{2} \boldsymbol{\mathcal{S}})_{i,k,:,:}
% \label{eq:eq4}
% \end{equation}

% By a few manipulation, we can make approximation matrix $\boldsymbol{\mathcal{S}}$ so that a pruned channel corresponding to a pruned filter in $l$-th layer is divided into preserved channels in each filters in $(l+1)$-th layer. Through this matrix, we can make compensated feature map ${\tilfde{\mathbf{Z}}_{i,:,:}^{{(l+1)}}}$ which is represented as below.

% \begin{equation}
% {{\tilde{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}} = \sum\limits_{k = 1, k \neq j}^{m} \mathbf{A}_{k,:,:}^{(\ell)} \circledast (\mathbf{W}_{i,k,:,:}^{(\ell+1)}+{s_{k}} \mathbf{W}_{i,j,:,:}^{(\ell+1)})
% \label{eq:eq}\nonumber
% \end{equation}

% Then, using Eq. (\ref{eq:eq3}). and Eq. (\ref{eq:eq4})., the reconstruction error after pruning and compensation can be represented as below.

% \begin{equation}
% {\mathbf{Z}_{i,:,:}^{{(\ell+1)}}}-{\mathbf{\tilde{Z}}_{i,:,:}^{{(l+1)}}}=(\mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)})\circledast\mathbf{W}_{i,j,:,:}^{(l+1)}
% \label{eq:eq5}
% \end{equation}

% And using Eq. (\ref{eq:eq5})., the whole reconstruction error of feature maps in $(\ell+1)$-th layer can be represented as below Eq. \ref{eq:eq6}).

% \begin{equation}
% \sum\limits_{{i} = 1}^{m^{\prime}}\|{\mathbf{Z}_{i,:,:}^{{(\ell+1)}}-\mathbf{\hat{Z}}_{i,:,:}^{{(\ell+1)}}}\|_1 = \sum\limits_{{i} = 1}^{m^{\prime}}\|(\mathbf{A}_{j,:,:}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(\ell)})\circledast\mathbf{W}_{i,j,:,:}^{(\ell+1)}\|_1
% \label{eq:eq6}
% \end{equation}


% \smalltitle{Without BN, ReLU}
% As shown in Eq. (\ref{eq:eq6})., we should find scalars $s_{k}$ such that $\mathbf{A}_{j,:,:}^{(\ell+1)} \approx \sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k,:,:}^{(l+1)}$ to minimize the reconstruction error. 

% \begin{equation}
% \mathbf{Z}_{j,:,:}^{(\ell)} =\sum\limits_{i = 1, i \neq j }^{m} {s}_{i} \times \mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{i,:,:,:}^{(l)} +  \mathbf{Z}^{(\ell-1)} \circledast \boldsymbol{\epsilon}
% \label{eq:eq7}
% \end{equation}

% \smalltitle{Considering BN} Now we should consider Batch Normalization to minimize Eq. (\ref{eq:goal2}). In this case, $\mathbf{A}^{(\ell)} = \N(\mathbf{Z}^{(\ell)})$, where $\N$ is Batch Normalization function and as a result (12) can be represented as below Eq.(14).

% \begin{eqnarray} \begin{split}\label{eq:eq8}
%      \|\mathbf{A}_{j}^{(\ell)}-\sum\limits_{k = 1, k \neq j}^{m}{s_{k}} \mathbf{A}_{k}^{(\ell)}\|_{1} = &~\| \N(\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{j}^{(l)} ) - \sum\limits_{k = 1, k \neq j }^{m} {s}_{k} \times \N (\mathbf{Z}^{(\ell-1)}  \circledast \mathbf{W}_{k}^{(l)} ) \|_{1}
% \end{split}
% \end{eqnarray}































% % In that case, reconstruction error formula Eq.(\ref{eq:eq5}) can be represented as theorem (\ref{theorem:theorem2})
% % If we compensate one filter with multiple filters, the reconstruction error formula can be obtained as below.
% To optimize the the approximation scale that minimize the reconstruction error, we decompose the how the reconstruction error consist of and discover that the reconstruction error is composed of three error terms,which are Sum of Squares Error(SSE), Batch Normalization Error(BE) and Activation Error(AE).

% \smalltitle{\textit{Theorem 1}} The reconstruction error is decomposed as below.
% \begin{eqnarray} \begin{split}\label{Theorem:Theorem1}
%         \boldsymbol{\|\mathcal{K}\|_1} & =  \|\boldsymbol{\alpha}_{j}^{{(l+1)}} - \sum\limits_{i = 0, i \neq j }^{m_i} {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}} \|_1 \\
%         & = \|\boldsymbol{\varepsilon} -\boldsymbol{\mathds{1}}\times\boldsymbol{\alpha}_{j}^{{(l+1)}} + \sum\limits_{i = 0, i \neq j }^{m_i}(\boldsymbol{\mathds{1}_{i}} \times {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}}) \|_1 \\
%         & \le  \|\boldsymbol{\varepsilon}\|_1 + \|\sum\limits_{i = 0, i \neq j }^{m_i}(\boldsymbol{\mathds{1}_{i}} \times {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}})  -\boldsymbol{\mathds{1}}\times\boldsymbol{\alpha}_{j}^{{(l+1)}}\|_1
% \end{split}
% \end{eqnarray}
% where, $\boldsymbol{\mathds{1}}$ is the indicator variable, $\boldsymbol{\varepsilon}$ = $\|\boldsymbol{\alpha}_{j}^{{(l+1)}} - \sum\limits_{i = 0, i \neq j }^{m_i} {\beta}_{i} \boldsymbol{{\alpha}}_{i}^{{(l+1)}} \|_1$. More detailed derivation above formula is in appendix. \kim{Is it better than the direc delta?}

% As we can see, Theorem (\ref{theorem:theorem2}) is generalized version of Theorem (\ref{theorem:theorem1}).
% We set a reasonable loss function as below that can overall control SSE and BE (and weakly AE through L2-regularization) Eq. \ref{eq:eq12} and optimizing this loss function, we can obtain nicely a closed form solution as Theorem \ref{theorem:theorem3}

% \begin{equation}
% loss = \| \boldsymbol{W}_{j,:,:,:}^{(\ell)} - \boldsymbol{\beta} \times \boldsymbol{W}_{i,:,:,:}^{(\ell)} \|_2 + \boldsymbol{\lambda_1} {\|\boldsymbol{\mathcal{K}}\|_2} + \boldsymbol{\lambda_1} {\|\boldsymbol{\beta}\|_2}
% \label{eq:eq12}
% \end{equation}

% \smalltitle{\textit{Theorem 3}} \kim{the unique closed form solution. we will use the property of positive definite matrix and weak vector calculus to prove that (in appendix).}
% \begin{eqnarray} \begin{split}\label{theorem:theorem3}
%     \mathcal{L}_{re} = 
% \end{split}
% \end{eqnarray}

% Using this closed form solution, we can compensate pruned filter in a real time. we call this compensation method LBYL(leave Before You Leave). LBYL can have advantage in the perspective of SSE. Furthermore, LBYL also relect other error components(BE,AE) so that pruned filter can be compensated more optimally.\kim{The whole procedure of LBYL is described in Algorithm 1.}



% As the pruned filter is represented by similar preserved filter, the activation maps generated by pruned filter can represent as shown in Eq. (\ref{eq:eq7}) because both pruned filter and preserved filter have same activation maps $\mathbf{Z}^{(\ell)}$

% \begin{equation}
% \boldsymbol{\hat{\alpha}}_{j,:,:}^{(l+1)} =\mathcal{S} \times \boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}}  + \boldsymbol{\epsilon}  \circledast \mathbf{Z}^{(\ell)} 
% \label{eq:eq7}
% \end{equation}

% However, \cite{NM} chooses a most similar the pruned filter with preserved filter based on $\boldsymbol{\mathcal{B}}$ which consider the batch normalization as shown Eq. (\ref{eq:eq8}) and then recompute scale $\mathcal{S}$ as adjusted scale $\mathcal{K}$. 

% \begin{equation}
% \boldsymbol{BN}(\boldsymbol{\hat{\alpha}}_{j,:,:}^{{(l+1)}}) =\mathcal{K} \times \boldsymbol{BN}(\boldsymbol{\hat{\alpha}}_{i,:,:}^{{(l+1)}})  + \boldsymbol{\mathcal{B}}
% \label{eq:eq8}
% \end{equation}
% where $\mathcal{K}$ = s$\frac{\gamma_{j}\sigma_{i}}{\gamma_{i}\sigma_{j}}$, $\boldsymbol{\mathcal{B}}$ = $\frac{\gamma_{j}}{\sigma_{j}}[s(-\frac{\sigma_{i}\beta_{i}}{\gamma_{i}} + \mu_{i}) - \mu_{j} ] + \beta_{j}$ are the adjusted scale and bias considering the batch normalization respectively, here s = $\frac{||\boldsymbol{W}_{j,:,:,:}^{(\ell)}||_2}{||\boldsymbol{W}_{i,:,:,:}^{(\ell)}||_2}$


% Finally, \cite{NM} consider the activation layer (\textit{e.g.,} ReLU) using the non-negative cosine similarity between the pruned filter and preserved filter. In other words, scale matrices $ {\boldsymbol\beta}^{(\ell)}$ in $l$-th layer is computed for all pairs of be 

% $\mathcal{K}$  has only non-negative entries with at most one strictly positive entry per column. Therefore, the pruned filter with negative similarity is not compensated.

% % limitations
% Therefore, there are limitations of one-to-one compensation. First of all, they should decide a similarity threshold about how similar pruned filter is. That is, if not exist a sufficiently similar filter, pruned filter is not compensated. Moreover, Even if there is a quiet similar filter about the pruned filter, its residual term  is not still zero because the scale is computed based on magnitude about the pruned filter and preserved filter. In other words, they only focus on how pruned filter is similar to preserved filter. 



==> backup/problem.tex <==
\section{Problem Formulation} \label{sec:probdef}

This section formally defines the problem of restoring a given pruned network with only using its original pretrained CNN in a way free of data and fine-tuning.



% Unlike many existing works utilize data for identifying unimportant filters as well as fine-tuning to this end, we cannot evaluate the filter importance by data-dependent values like activation maps (\textit{a.k.a.} channels) as our focus in this paper is not to use any training data. Thus, in our problem setting, we can only exploit the values of filters in the original network, and thereby have to make some changes in the remaining filters of the pruned network so that the network can return the output not too much different from the original one.

% No matter how much we carefully select unimportant filters to be pruned, some kinds of retraining process appears inevitable as done by the most existing works to this end. However, since our focus in this paper is not to use any training data, we cannot evaluate the importance of filters by data-dependent values like activation maps (\textit{a.k.a.} channels). 

% To this end, they not only use a careful criterion (\textit{e.g.}, L1-norm), but also fine-tune the network using the original data.
% Most of filter pruning methods try to select filters to be pruned prudently so that pruned network's output be similar to the original network's. To this end, they prune the unimportant filters and then fine-tune the pruned network with using the train data. 

% How can we restore the the pruned networks without any data? In other words, it implies that we cannot use any data-driven values(i.e., activation maps) and we can only exploit the values of original filters. In that case, the only thing we can do maybe changing the weights of remained filters appropriately not to amplify the difference between pruned and unpruned network's outputs through the information of original filters.

\begin{figure*}[t]
	\centering
    \subfloat[\label{fig:matrix:a}Pruning matrix]{\hspace{6mm}\includegraphics[width=0.4\columnwidth]{./figure/LBYL_figure_2_1.pdf}\hspace{6mm}} 
    \subfloat[\label{fig:matrix:b}Delivery matrix for LBYL]{\hspace{6mm}\includegraphics[width=0.4\columnwidth]{./figure/LBYL_figure_2_2.pdf}\hspace{6mm}}
    \subfloat[\label{fig:matrix:c}Delivery matrix for one-to-one]{\hspace{9mm}\includegraphics[width=0.4\columnwidth]{./figure/LBYL_figure_2_3.pdf}\hspace{9mm}} 
    \caption{Comparison between pruning matrix and delivery matrix, where the $4$-th and $6$-th filters are being pruned among $6$ original filters}
	\label{fig:matrix}
	\vspace{-2mm}
\end{figure*}


\subsection{Filter Pruning in a CNN}
Consider a given CNN to be pruned with $L$ layers, where each $\ell$-th layer starts with a convolution operation on its input channels, which are the output of the previous $(\ell-1)$-th layer $\mathbf{A}^{(\ell-1)}$, with the group of convolution filters $\mathbf{W}^{{(\ell)}}$ and thereby obtain the set of \textit{feature maps} $\mathbf{Z}^{(\ell)}$ as follows:
\begin{equation}
\boldsymbol{\mathbf{Z}}^{(\ell)} = {\mathbf{A}^{(\ell-1)} \circledast {\mathbf{W}}^{(\ell)}},
\nonumber
\end{equation}


%  \begin{equation}
% \label{deqn_ex1}
% x = \sum_{i=0}^{n} 2{i} Q.
% \end{equation}


where $\circledast$ represents the convolution operation. Then, this convolution process is normally followed by a batch normalization (BN) process and an activation function such as ReLU, and the $\ell$-th layer finally outputs an \textit{activation map} $\mathbf{A}^{(\ell)}$ to be sent to the $(\ell+1)$-th layer through this sequence of procedures as:
\begin{equation}
\mathbf{A}^{(\ell)} = \F(\N(\mathbf{Z}^{(\ell)})),
\nonumber
\end{equation}
where $\F(\cdot)$ is an activation function and $\N(\cdot)$ is a BN procedure.

Note that all of $\mathbf{W}^{(\ell)}$, $\mathbf{Z}^{(\ell)}$, and $\mathbf{A}^{(\ell)}$ are tensors such that: $\mathbf{W}^{(\ell)} \in \mathbb{R}^{m \times n \times k \times k}$ and $\mathbf{Z}^{(\ell)},\mathbf{A}^{(\ell)} \in \mathbb{R}^{m \times w \times h}$, where (1) $m$ is the number of filters, which also equals the number of output activation maps, (2) $n$ is the number of input activation maps resulting from the $(\ell-1)$-th layer, (3) $k \times k$ is the size of each filter, and (4) $w \times h$ is the size of each output channel for the $\ell$-th layer.

\smalltitle{Filter pruning as n-mode product}
When filter pruning is performed at the $\ell$-th layer, all three tensors above are consequently modified to their \textit{damaged} versions, namely $\mathbf{\Tilde{W}}^{(\ell)}$, $\mathbf{\Tilde{Z}}^{(\ell)}$, and $\mathbf{\Tilde{A}}^{(\ell)}$, respectively, in a way that: $\mathbf{\Tilde{W}}^{(\ell)} \in \mathbb{R}^{t \times n \times k \times k}$ and $\mathbf{\Tilde{Z}}^{(\ell)},\mathbf{\Tilde{A}}^{(\ell)} \in \mathbb{R}^{t \times w \times h}$, where $t$ is the number of remaining filters after pruning and therefore $t < m$. Mathematically, the tensor of remaining filters, \textit{i.e.}, $\mathbf{\Tilde{W}}^{(\ell)}$, is obtained by the \textit{$1$-mode product} \cite{DBLP:journals/siamrev/KoldaB09} of the tensor of the original filters $\mathbf{W}^{(\ell)}$ with a \textit{pruning matrix} $\boldsymbol{\S} \in \mathbb{R}^{m \times t}$ (see Figure \ref{fig:matrix:a})
as follows:
\begin{eqnarray}\begin{split}\label{eq:pruning}
\mathbf{\Tilde{W}}^{(\ell)} = {\mathbf{W}}^{(\ell)} \times_{1} {\boldsymbol{\S}}^{T},\text{where }\boldsymbol{\S}_{i,k} = 
  \begin{cases} 
   1~ \text{if } i = i'_k \\
   0~ \text{otherwise}
  \end{cases} \\
  \text{s.t. } i, i'_k \in [1, m] 
  \text{ and } k \in [1, t].
  \end{split}
\end{eqnarray}
  
By Eq. (\ref{eq:pruning}), each $i'_k$-th filter is not pruned and the other $(m-t)$ filters are completely removed from $\mathbf{W}^{(\ell)}$ to be $\mathbf{\Tilde{W}}^{(\ell)}$.

This reduction at the $\ell$-th layer causes another reduction for each filter of the $(\ell+1)$-th layer so that $\mathbf{W}^{(\ell+1)}$ is now modified to $\mathbf{\Tilde{W}}^{(\ell+1)} \in \mathbb{R}^{m' \times t \times k' \times k'}$, where $m'$ is the number of filters of size $k' \times k'$ in the $(\ell+1)$-th layer. Due to this series of information losses, the resulting feature map (\textit{i.e.}, $\mathbf{Z}^{(\ell+1)}$) would severely be damaged to be $\mathbf{\Tilde{Z}}^{(\ell+1)}$ as shown below:
\begin{equation}
{\mathbf{\Tilde{Z}}}^{{(\ell+1)}} = \mathbf{\Tilde{A}}^{(\ell)} \circledast {\mathbf{\Tilde{W}}}^{(\ell+1)}~~~\not\approx~~~\mathbf{Z}^{(\ell+1)}
\label{eq:eq}\nonumber
\end{equation}
The shape of $\mathbf{\Tilde{Z}}^{(\ell+1)}$ remains the same unless we also prune filters for the $(\ell+1)$-th layer. If we do so as well, the loss of information will be accumulated and further propagated to the next layers. Note that $\mathbf{\Tilde{W}}^{(\ell+1)}$ can also be represented by the \textit{$2$-mode product} \cite{DBLP:journals/siamrev/KoldaB09} of $\mathbf{W}^{(\ell+1)}$ with the transpose of the same matrix $\boldsymbol{\S}$ as:
\begin{equation} \label{eq:pruning2}
\mathbf{\Tilde{W}}^{(\ell+1)} = {\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\S}^T}
\end{equation}




\subsection{Problem of Restoring a Pruned Network without Data and Fine-Tuning}
As mentioned earlier, our goal is to restore a pruned and thus damaged CNN without using any data and re-training process, which implies the following two facts. First, we have to use a pruning criterion exploiting only the values of filters themselves such as L1-norm. In this sense, this paper does not focus on proposing a sophisticated pruning criterion but intends to recover a network somehow pruned by such a simple criterion. Secondly, since we cannot make appropriate changes in the remaining filters by fine-tuning, we should make the best use of the original network and identify how the information carried by a pruned filter can be delivered to the remaining filters.

% For brevity, we formulate our problem here with respect to a specific layer, say $\ell$, and then it can trivially be generalized for the entire network. 
\smalltitle{Delivery matrix}
In order to represent the information to be delivered to the preserved filters, let us first think of what the pruning matrix $\boldsymbol{\S}$ means. As defined in Eq. (\ref{eq:pruning}) and shown in Figure \ref{fig:matrix:a}, each row is either a zero vector (for filters being pruned) or a one-hot vector (for remaining filters), which is intended only to remove filters without delivering any information. Intuitively, we can transform this pruning matrix into a \textit{delivery matrix} that carries information for filters being pruned by replacing some meaningful values with some of the zero values therein. Once we find such an \textit{ideal} $\boldsymbol{\S^*}$, we can plug it into $\boldsymbol{\S}$ of Eq. (\ref{eq:pruning2}) to deliver missing information propagated from the $\ell$-th layer to the filters at the $(\ell+1)$-th layer, which will hopefully generate an approximation $\mathbf{\hat{Z}}^{(\ell+1)}$ close to the original feature map as follows:
\begin{equation} \label{eq:fmap_approx}
{\mathbf{\hat{Z}}}^{{(\ell+1)}} = {\mathbf{\Tilde{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\S^*}^T})}
~~~\approx~~~\mathbf{Z}^{(\ell+1)}
\end{equation}
Thus, using the delivery matrix $\boldsymbol{\mathcal{S^*}}$, the information loss caused by pruning at each layer is recovered at the feature map of the next layer.

\smalltitle{Problem statement}
Given a pretrained CNN, our problem aims to find the best delivery matrix $\boldsymbol{\mathcal{S^*}}$ for each layer without any data and training process such that the following \textit{reconstruction error} is minimized:
\begin{equation}
\sum\limits_{i = 1}^{m'}\|{{\mathbf{Z}}_{i}^{{(\ell+1)}}-{\hat{\mathbf{Z}}}_{i}^{{(\ell+1)}}}\|_1,
\label{eq:goal}
\end{equation}
where ${\mathbf{Z}}_i^{{(\ell+1)}}$ and ${\hat{\mathbf{Z}}}_i^{{(\ell+1)}}$ indicate the $i$-th original feature map and its corresponding approximation, respectively, out of $m'$ filters in the $(\ell+1)$-th layer. Note that what is challenging here is that we cannot obtain the activation maps in $\mathbf{A}^{(\ell)}$ and $\mathbf{\Tilde{A}}^{(\ell)}$ without data as they are data-dependent values.

% = \sum\limits_{i = 1}^{m'}\|{{\mathbf{Z}}_{i}^{{(\ell+1)}}-{\mathbf{\Tilde{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {\boldsymbol{\mathcal{S^*}^T}})}}\|_{1}


% Our goal is finding the approximation matrix $\boldsymbol{\mathcal{S}}$ to minimize the reconstruction error between the pruned model and the original model without any data, and effectively deliver missing information for pruned filters using this approximation matrix


% $\testit{s}$,which can be represented as below.

% \begin{equation}
% \boldsymbol{\mathcal{S}} =  \underset{{\boldsymbol{\mathcal{S}}}}{\mathrm{argmin}} \sum\limits_{{i} = 1}^{m_{\ell+1}} \|{{\mathbf{Z}}_{i,:,:}^{{(\ell+1)}}-{\hat{\mathbf{Z}}}_{i,:,:}^{{(\ell+1)}}}\|_{1} 
% \label{eq:eq1}
% \end{equation}



% Let us first recall that the ultimate goal of network pruning is to make the output of a pruned network as close as possible to that of its original network. Unlike many existing pruning methods, our focus is not to use any training data at all for the entire pruning and recovery process, and this implies the following two facts. First, we cannot evaluate the filter importance by data-dependent values like activation values or gradients, but have to use a pruning criterion exploiting only the values of filters themselves such as L1-norm. Furthermore, instead of fine-tuning with data, the only thing we can do for the pruned network is to make appropriate changes in the remaining filters by identifying some relationships between pruned filters and the other preserved ones without any support from data. Based on this intuition, this section mathematically and generally defines the problem of restoring a pruned neural network in a manner free of data and fine-tuning.


% Thus, we make approximation matrix $\testit{s}$ $\in$ $\mathbb{R}^{m_{\ell} \times t_{\ell}}$ with relationship between the pruned filter and preserved filters in $\ell$-th layer and then apply it to the original filters in $(\ell+1)$-th layer to compensate for pruned feature maps $\boldsymbol{\hat{\mathbf{Z}}}^{{(\ell+1)}}$ as shown below.
% (\textit{i.e.}, Let $\hat{\mathbf{W}}^{(\ell+1)}$ be ${\mathbf{W}}^{(\ell+1)}$ $\times_2$ ${{\textit{s}}} $, where $\times_2$ is 2-mode matrix product) 

% \begin{equation}
% \mathbf{Z}^{(\ell+1)} = {\mathbf{A}}^{(\ell)} \circledast {\mathbf{W}}^{(\ell+1)}
% \approx {\hat{\mathbf{A}}^{(\ell)} \circledast ({\mathbf{W}}^{(\ell+1)} \times_{2} {{s}}) = {\hat{\mathbf{Z}}}^{{(\ell+1)}}}
% \label{eq:eq}\nonumber
% \end{equation}




% For a Convolutional Neural Network (CNN) with $L$ layers, we denote $\mathcal{A}{^{(\ell-1)}}$ $\in$ $\mathbb{R}^{n_{\ell -1 } \times h_{\ell -1} \times w_{\ell -1}}$ is activation maps at $\ell-1$-th layer, where $n_{\ell -1}$, $h_{\ell -1}$ and $w_{\ell -1}$ are the number of channels, height and width in activation maps, respectively. and we denote $\mathbf{W}^{{(\ell )}}$ $\in$  $\mathbb{R}^{m_{\ell} \times n_{\ell -1}\times k \times k}$ is covolution filters in $\ell$-th layer,where $m_{\ell}$, $n_{\ell-1}$ and $k$ are the number of filters, number of channels and kernel size, respectively. Trough the convolution operation using activation map $\mathcal{A}{^{(\ell-1)}}$ and convolution filter $\mathbf{W}^{{(\ell)}}$ in $\ell$-th layer, the feature maps $\boldsymbol{\mathbf{Z}}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_{\ell} \times h_{\ell+1} \times w_{\ell+1}}$ is computed as shown as below.


% \begin{equation}
% \boldsymbol{\mathbf{Z}}^{(\ell)} = {\mathcal{A}^{(\ell-1)} \circledast {\mathbf{W}}^{(\ell)}}
% \label{eq:eq1}\nonumber
% \end{equation}
% where $\circledast$ is convolution operation.

% and the feature maps passed through the BN and ReLU layer are activation maps $\mathcal{A}{^{(\ell)}}$ $\in$ $\mathbb{R}^{m_{{\ell}} \times h_{\ell+1} \times w_{\ell+1}} $ in $\ell$-th layer as shown as below.

% \begin{equation}
% \mathcal{A}^{(\ell)} = \mathcal{F}(\mathbf{Z}^{(\ell)} \circledast {\mathbf{W}}^{(\ell)})
% \label{eq:eq2}\nonumber
% \end{equation}
% where $\mathcal{F}$ is the function that implement batch normalization and non-linear activation(\textit{e.g.}, ReLU).

% \smalltitle{Filter Pruning}
% If the filter pruning is performed in $\ell$-th layer, the shape of original filters $\mathbf{W}^{{(\ell)}}$ $\in$ $\mathbb{R}^{m_{\ell} \times n_{\ell-1}\times k \times k}$ is modified to ${\hat {\mathbf{W}}^{(\ell)}}$ $\in$ $\mathbb{R}^{t_{\ell} \times n_{\ell-1}\times k \times k}$, where $t_{\ell}$ $<$ $m_{\ell}$ by pruning criterion. Therefore, the pruned activation maps ${\hat {\mathcal{A}}}{^{({\ell+1})}}$ $\in$ $\mathbb{R}^{t_{{\ell}} \times h_{{\ell+2}} \times w_{{\ell+2}}}$ in (${\ell+1}$)-th layer is computed as below.

% \begin{equation}
% \mathbf{\hat{A}}^{(l+1)} = \mathcal{F}({\mathbf{A}^{(\ell)} \circledast {\mathbf{\hat{W}}}^{(\ell+1)}})
% \label{eq:eq3}\nonumber
% \end{equation}

% Moreover, corresponding channels of each filters in ($\ell +1$)-th layer are sequentially removed. As a result, shape of original filters $\mathbf{W}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times m_{\ell}\times k \times k}$ in ($\ell+1$)-th layer is changed to  ${\hat {\mathbf{W}}^{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times t_{\ell}\times k \times k}$. Although feature maps ${\hat{\mathbf{Z}}}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times h_{\ell+2} \times w_{\ell+2}}$ in ($\ell+1$)-th layer after pruning have same shape with original feature maps ${\mathbf{Z}}^{{(\ell+1)}}$ $\in$ $\mathbb{R}^{m_{\ell+1} \times h_{\ell+2} \times w_{\ell+2}}$, the pruned feature maps $\boldsymbol{\hat{\mathbf{Z}}}^{{(\ell+1)}}$ are damaged.

==> backup/related.tex <==
\section{Related Works} \label{sec:related}
Many filter pruning methods have been studied without considering such a case where we cannot use any data, whether real or synthetic, to restore a pruned network. They mostly go through an expensive retraining process either iteratively \cite{Soft,FPGM,Dynamic} or lastly as a fine-tuning phase \cite{GlobalRanking,Importance,NISP}. In this paper, we focus on the opposite case, which is more challenging in practice, where fine-tuning with any data is not available.

\smalltitle{Pruning with less fine-tuning} 
Most of the existing filter pruning methods have tried to avoid an expensive fine-tuning process by means of a carefully designed criterion for identifying unimportant filters such that the loss of information is minimized when they are pruned. To this end, they often make the best use of data-dependent values like channels and gradients that can be obtained by making inferences with some data. \cite{Thinet} propose a greedy algorithm that prunes the filters whose corresponding channels minimize the layer-wise reconstruction error. Similarly, \cite{Lasso} formulate this problem of channel selection as lasso regression and least square reconstruction. \cite{CoreSet_ICLR} introduce data-independent pruning criterion based on coreset together with an intermediate recovery method without training in order to reduce the overhead of fine-tuning. Despite their proposed methods on effective channel or neuron selection, a few epochs of fine-tuning process as well as some training data is inevitable for the pruned network to be sufficiently recovered. 


\smalltitle{Pruning with less fine-tuning and less data}
For the case of pruning with limited data, several methods \cite{CURL,Reborn} utilize knowledge distillation \cite{Knowledge_Distilation} not to use the entire original data in the recovery process. \cite{CURL} recently propose \textit{CURL} that globally prunes filters using a KL-divergence based criterion and perform knowledge distillation with a small dataset as a fine-tuning process. \cite{Reborn} tackle the similar problem and devise a way of transforming all the filters in a layer into compact ones, called \textit{reborn filters}, using only the limited data. These methods do not use the entire original data, but they still require some kinds of retraining process with a small amount of data. Meanwhile, there is a branch of data-free pruning methods \cite{Data-Free-NetworkPruning, DeepInversion} that still fine-tune the pruned model with synthetically generated data but not real data. In addition to the heavy fine-tuning process, these methods require another non-trivial training process to build a generative model for obtaining synthetic data.

\smalltitle{Pruning with no fine-tuning and no data} In the literature of filter pruning, there are only a couple of works \cite{NM, Data-free} that adopt the same problem setting as ours, that is, pruning filters without any data and fine-tuning. Both methods are based on the strong assumption that we can always find a pair of filters that are quite similar to each other and therefore a pruned filter can be compensated by its similar unpruned one. However, this assumption does not hold in modern convolutional neural networks (CNNs) having a number of filters in a fairly deep architecture. As even presented in \cite{NM}, the cosine similarity between each filter and its nearest one gets extremely low (\textit{e.g.}, around 0.2) in back layers to the point that it is better to do nothing for some pruned neurons that do not have sufficiently similar preserved neurons. In this paper, we remedy this problem by using as many preserved filters as possible to compensate for each pruned filter, and thereby propose a more robust method that successfully relaxes the assumption made by these existing works.

% \smalltitle{



% \lee{ \cite{RedPlus} focuses on reducing the number of computations by changing identical operations to identical memory access to a unique operation. That is, \cite{RedPlus} needs the hypothesis that memory access and allocation should run faster than mathematical operations, while our LBYL method do not need a specific hardware assumption. Therefore \cite{RedPlus} is orthogonal to our method. In this paper, we remedy problem of similarity based compensation \cite{NM, Data-free} by using as many preserved filters as possible to compensate for each pruned filter, and thereby propose a more robust method that successfully relaxes the assumption made by these existing works.}

